Learning Dynamics of Deep Linear Networks Beyond the Edge of Stability

Deep neural networks trained using gradient descent with a fixed learning rate $\eta$ often operate in the regime of "edge of stability" (EOS), where the largest eigenvalue of the Hessian equilibrates about the stability threshold $2/\eta$. In this work, we present a fine-grained analysis of the learning dynamics of (deep) linear networks (DLNs) within the deep matrix factorization loss beyond EOS. For DLNs, loss oscillations beyond EOS follow a period-doubling route to chaos. We theoretically analyze the regime of the 2-period orbit and show that the loss oscillations occur within a small subspace, with the dimension of the subspace precisely characterized by the learning rate. The crux of our analysis lies in showing that the symmetry-induced conservation law for gradient flow, defined as the balancing gap among the singular values across layers, breaks at EOS and decays monotonically to zero. Overall, our results contribute to explaining two key phenomena in deep networks: (i) shallow models and simple tasks do not always exhibit EOS; and (ii) oscillations occur within top features. We present experiments to support our theory, along with examples demonstrating how these phenomena occur in nonlinear networks and how they differ from those which have benign landscape such as in DLNs.

==> ICLR/text/deferred_proofs.tex <==

\section{Deferred Proofs}
\label{sec:proofs}

\subsection{Deferred Proofs for Oscillations}
\label{sec:proofs_oscillations}

\begin{manualpropositioninner}[Singular Vector Stationary Set]
Consider the deep matrix factorization loss in Equation~(\ref{eqn:deep_mf}). Let $\mbf{M}_\star = \mbf{U}_\star \mbf{\Sigma}_\star \mbf{V}_\star^\top$ and 
$\mbf{W}_\ell(t) = \mbf{U}_\ell(t) \mbf{\Sigma}_\ell(t) \mbf{V}_\ell^\top(t)$ denote the compact SVD for the target matrix and the $\ell$-th layer weight matrix at time $t$, respectively. For any time $t\geq 0$, if $\dot{\mbf{U}}_\ell(t) = \dot{\mbf{V}}_\ell(t) = 0$ for all $\ell \in [L]$, then the singular vector stationary points for each weight matrix are given by
\begin{align*}
\mathrm{SVS}(f(\mbf{\Theta})) = 
\begin{cases}
    (\mbf{U}_L, \mbf{V}_L) &= (\mbf{U}_\star, \mbf{Q}_L), \\
    (\mbf{U}_\ell, \mbf{V}_\ell) &= (\mbf{Q}_{\ell+1}, \mbf{Q}_\ell), \quad\forall \ell \in [2, L-1], \\
    (\mbf{U}_1, \mbf{V}_1) &= (\mbf{Q}_2, \mbf{V}_\star),
\end{cases}
\end{align*}
where \(\{\mbf{Q}_\ell\}_{\ell=2}^{L}\) can be any orthogonal matrices. \label{svs-set}
\end{manualpropositioninner}

\begin{proof}

Let us consider the dynamics of $\mbf{W}_\ell(t)$ in terms of its SVD with respect to time:
\begin{align}
\label{eqn:svd_rynamics}
    \dot{\mbf{W}}_\ell(t) &= \dot{\mbf{U}}_\ell(t) \mbf{\Sigma}_\ell(t) \mbf{V}_\ell^\top(t) + \mbf{U}_\ell(t) \dot{\mbf{\Sigma}}_\ell(t) \mbf{V}_\ell^\top(t) + \mbf{U}_\ell(t) \mbf{\Sigma}_\ell(t) \dot{\mbf{V}}_\ell^\top(t).
\end{align}
By left multiplying by \(\mbf{U}_\ell^\top(t)\) and right multiplying by \(\mbf{V}_\ell(t)\), we have
\begin{align}
    \mbf{U}_\ell^\top(t) \dot{\mbf{W}}_\ell(t) \mbf{V}_\ell(t) &= \mbf{U}_\ell^\top(t) \dot{\mbf{U}}_\ell(t) \mbf{\Sigma}_\ell(t) + \dot{\mbf{\Sigma}}_\ell(t) + \mbf{\Sigma}_\ell(t) \dot{\mbf{V}}_\ell^\top(t) \mbf{V}_\ell(t), 
\end{align}
where we used the fact that \(\mbf{U}_\ell(t)\) and \(\mbf{V}_\ell(t)\) have orthonormal columns. Now, note that we also have
\begin{align*}
    \mbf{U}_\ell^\top(t) \mbf{U}_\ell(t) = \mbf{I}_r \implies \dot{\mbf{U}}_\ell^\top(t) \mbf{U}_\ell(t) + \mbf{U}_\ell^\top(t) \dot{\mbf{U}}_\ell(t) = \mbf{0},
\end{align*}
which also holds for $\mbf{V}_\ell(t)$. This implies that $\dot{\mbf{U}}_\ell^\top(t) \mbf{U}_\ell(t)$ is a skew-symmetric matrix, and hence have zero diagonals. 
Since \(\mbf{\Sigma}_\ell(t)\) is diagonal, \(\mbf{U}_\ell^\top(t) \dot{\mbf{U}}_\ell(t) \mbf{\Sigma}_\ell(t)\) and \(\mbf{\Sigma}_\ell(t) \dot{\mbf{V}}_\ell^\top(t) \mbf{V}_\ell(t)\) have zero diagonals as well. On the other hand, since \(\dot{\mbf{\Sigma}}_\ell(t)\) is a diagonal matrix, we can write
\begin{align}
\label{eqn:diag_inv}
    \hat{\mbf{I}}_r \odot \left(\mbf{U}_\ell^\top(t) \dot{\mbf{W}}_\ell(t) \mbf{V}_\ell(t)\right) &= \mbf{U}_\ell^\top(t) \dot{\mbf{U}}_\ell(t) \mbf{\Sigma}_\ell(t) + \mbf{\Sigma}_\ell(t) \dot{\mbf{V}}_\ell^\top(t) \mbf{V}_\ell(t), 
\end{align}
where \(\odot\) stands for the Hadamard product and \(\hat{\mbf{I}}_r\) is a square matrix holding zeros on its diagonal and ones elsewhere. Taking transpose of Equation~(\ref{eqn:diag_inv}), while recalling that \(\mbf{U}_\ell^\top(t) \dot{\mbf{U}}_\ell(t)\) and \(\mbf{V}_\ell^\top(t) \dot{\mbf{V}}_\ell(t)\) are skew-symmetric, we have
\begin{align}
\label{eqn:diag_inv_transpose}
    \hat{\mbf{I}}_{r} \odot \left(\mbf{V}_\ell^\top(t) \dot{\mbf{W}}_\ell^\top(t) \mbf{U}_\ell(t)\right) &= -\mbf{\Sigma}_\ell(t) \mbf{U}_\ell^\top(t) \dot{\mbf{U}}_\ell(t) - \dot{\mbf{V}}_\ell^\top(t) \mbf{V}_\ell(t) \mbf{\Sigma}_\ell(t). 
\end{align}
Then, by right multiplying Equation~(\ref{eqn:diag_inv}) by \(\mbf{\Sigma}_\ell(t)\), left-multiply Equation~(\ref{eqn:diag_inv_transpose}) by \(\mbf{\Sigma}_\ell(t)\), and by adding the two terms, we get
\begin{align*}
    \hat{\mbf{I}}_{r} \odot \biggl(\mbf{U}_\ell^\top(t) \dot{\mbf{W}}_\ell(t) \mbf{V}_\ell(t) \mbf{\Sigma}_\ell(t) + \mbf{\Sigma}_\ell(t) \mbf{V}_\ell^\top(t) &\dot{\mbf{W}}_\ell^\top(t) \mbf{U}_\ell(t)\biggr) \\
    &= \mbf{U}_\ell^\top(t) \dot{\mbf{U}}_\ell(t) \mbf{\Sigma}_\ell^2(t) - \mbf{\Sigma}_\ell^2(t) \dot{\mbf{V}}_\ell^\top(t) \mbf{V}_\ell(t). 
\end{align*}
Since we assume that the singular values of $\mbf{M}_\star$ are distinct, the top-$r$ diagonal elements of \(\mbf{\Sigma}_{\ell}^2(t)\) are also distinct (i.e., $\Sigma^2_{r}(t) \neq \Sigma^2_{r'}(t) \text{ for } r \neq r'$). This implies that
\begin{align*}
    \mbf{U}_{\ell}^\top(t) \dot{\mbf{U}}_{\ell}(t) &= \mbf{H}(t) \odot \left[\mbf{U}_{\ell}^\top(t) \dot{\mbf{W}}_{\ell}(t) \mbf{V}_{\ell}(t) \mbf{\Sigma}_{\ell}(t) + \mbf{\Sigma}_{\ell}(t) \mbf{V}_{\ell}^\top(t) \dot{\mbf{W}}_{\ell}^\top(t) \mbf{U}_{\ell}(t)\right], 
\end{align*}

where the matrix \(\mbf{H}(t) \in \mathbb{R}^{d\times d}\) is defined by:
\begin{align}
    H_{r,r'}(t) := 
    \begin{cases}
    \left(\Sigma^2_{r'}(t) - \Sigma^2_r(t)\right)^{-1}, & r \neq r', \\
    0, & r = r'.
    \end{cases}
\end{align}

Then, multiplying from the left by \(\mbf{U}_{\ell}(t)\) yields
\begin{align}
    \mbf{P}_{\mbf{U}_{\ell}(t)} \dot{\mbf{U}}_{\ell}(t) &= \mbf{U}_{\ell}(t) \left(\mbf{H}(t) \odot \left[\mbf{U}_{\ell}^\top(t) \dot{\mbf{W}}_{\ell}(t) \mbf{V}_{\ell}(t) \mbf{\Sigma}_{\ell}(t) + \mbf{\Sigma}_{\ell}(t) \mbf{V}_{\ell}^\top(t) \dot{\mbf{W}}_{\ell}^\top(t) \mbf{U}_{\ell}(t)\right]\right), 
\end{align}
with \(\mbf{P}_{\mbf{U}_{\ell}(t)} := \mbf{U}_{\ell}(t) \mbf{U}_{\ell}^\top(t)\) being the projection onto the subspace spanned by the (orthonormal) columns of \(\mbf{U}_{\ell}(t)\). Denote by \(\mbf{P}_{\mbf{U}_{{\ell}\perp}(t)}\) the projection onto the orthogonal complement ( i.e., $\mbf{P}_{\mbf{U}_{\ell\perp}(t)} := \mbf{I}_r - \mbf{U}_{\ell}(t) \mbf{U}_{\ell}^\top(t)$). Apply \(\mbf{P}_{\mbf{U}_{\ell\perp}(t)}\) to both sides of Equation~(\ref{eqn:svd_rynamics}):
\begin{align}
    \mbf{P}_{\mbf{U}_{\ell\perp}(t)}\dot{\mbf{U}}_{\ell}(t)  = \mbf{P}_{\mbf{U}_{\ell\perp}(t)} \dot{\mbf{U}}_{\ell}(t) \mbf{\Sigma}_\ell(t) \mbf{V}_{\ell}^\top(t) &+ \mbf{P}_{\mbf{U}_{\ell\perp}(t)} \mbf{U}_\ell(t) \dot{\mbf{\Sigma}}_{\ell}(t) \mbf{V}_{\ell}^\top(t)\\ &+ \mbf{P}_{\mbf{U}_{\ell\perp}(t)} \mbf{U}_\ell(t) \mbf{\Sigma}_\ell(t) \dot{\mbf{V}}_{\ell}^\top(t). 
\end{align}

Note that \(\mbf{P}_{\mbf{U}_{\ell\perp}(t)} \mbf{U}_\ell(t) = 0\), and multiply from the right by \(\mbf{V}_\ell(t) \mbf{\Sigma}_{\ell}^{-1}(t)\) (the latter is well-defined since we have the compact SVD and the top-$r$ elements are non-zero):
\begin{align}
    \mbf{P}_{\mbf{U}_{\ell\perp}(t)} \dot{\mbf{U}}_\ell(t) &= \mbf{P}_{\mbf{U}_{\ell\perp}(t)} \dot{\mbf{W}}_\ell(t) \mbf{V}_\ell(t) \mbf{\Sigma}_\ell^{-1}(t) = (\mbf{I}_r - \mbf{U}_\ell(t)\mbf{U}^\top(t)) \dot{\mbf{W}}(t) \mbf{V}_\ell(t) \mbf{\Sigma}_\ell^{-1}(t). 
\end{align}
Then by adding the two equations above, we obtain an expression for \(\dot{\mbf{U}}(t)\):
\begin{align}
    \dot{\mbf{U}}_\ell(t) &= \mbf{P}_{\mbf{U}_\ell(t)} \dot{\mbf{U}}_\ell(t) + \mbf{P}_{\mbf{U}_{\ell\perp}(t)} \dot{\mbf{U}}_\ell(t) \nonumber \\
    &= \mbf{U}_\ell(t)\left(\mbf{H}(t) \odot \left[\mbf{U}_\ell^\top(t) \dot{\mbf{W}}_\ell(t) \mbf{V}_\ell(t) \mbf{\Sigma}_\ell(t) + \mbf{\Sigma}_\ell(t) \mbf{V}_\ell^\top(t) \dot{\mbf{W}}_\ell^\top(t) \mbf{U}_\ell(t)\right]\right) \nonumber \\
    &\quad + (\mbf{I}_r - \mbf{U}_\ell(t) \mbf{U}_\ell^\top(t)) \dot{\mbf{W}}(t) \mbf{V}_\ell(t) \mbf{\Sigma}_\ell^{-1}(t). 
\end{align}
We can similarly derive the dynamics for $\dot{\mbf{V}}_\ell(t)$ and $\dot{\mbf{\Sigma}}_\ell(t)$:
\begin{align}
\dot{\mbf{V}}_\ell(t) = \mbf{V}_\ell(t)\left(\mbf{H}(t) \odot \left[\mbf{\Sigma}_\ell(t) \mbf{U}^\top_\ell(t) \dot{\mbf{W}_{\ell}}(t) \mbf{V}_\ell(t) + \mbf{V}^\top_\ell(t) \dot{\mbf{W}_{\ell}}^\top(t) \mbf{U}_\ell(t) \mbf{\Sigma}_\ell(t)\right]\right) \\
+ \left(\mbf{I}_{r} - \mbf{V}_\ell(t)\mbf{V}^\top_\ell(t)\right) \dot{\mbf{W}_{\ell}}^\top(t) \mbf{U}_\ell(t) \mbf{\Sigma}_\ell^{-1}(t), \label{vdiff}
\end{align}
\begin{align*}
   \dot{\mbf{\Sigma}}_\ell(t) = \mbf{I}_r \odot \left[ \mbf{U}^\top_\ell(t) \dot{\mbf{W}}_\ell(t) \mbf{V}_\ell(t) \right].
\end{align*}

Now, we will left multiply $\dot{\mbf{U}}_\ell(t)$ and $\dot{\mbf{V}}_\ell(t)$ with $\mbf{U}_\ell^\top(t)$ and $\mbf{V}_\ell^\top(t)$, respectively, to obtain
\begin{align*}
    \mbf{U}^\top_\ell(t) \dot{\mbf{U}}_\ell(t) &= -\mbf{H}(t) \odot \left[\mbf{U}^\top_\ell(t)\nabla_{\mbf{W}_{\ell}} f(\mbf{\Theta}) \mbf{V}_\ell(t) \mbf{\Sigma}_\ell(t) + \mbf{\Sigma}_\ell(t) \mbf{V}^\top_\ell(t) \nabla_{\mbf{W}_{\ell}} f(\mbf{\Theta}) \mbf{U}_\ell(t)\right], \\
    \mbf{V}^\top_\ell(t) \dot{\mbf{V}}_\ell(t) &= -\mbf{H}(t) \odot \left[\mbf{\Sigma}_\ell(t) \mbf{U}^\top_\ell(t) \nabla_{\mbf{W}_{\ell}} f(\mbf{\Theta}) \mbf{V}_\ell(t) + \mbf{V}^\top_\ell(t) \nabla_{\mbf{W}_{\ell}} f(\mbf{\Theta}) \mbf{U}_\ell(t) \mbf{\Sigma}_\ell(t)\right],
\end{align*}
where we replaced $\dot{\mbf{W}}_\ell(t) \coloneqq -\nabla_{\mbf{W}_{\ell}} f(\mbf{\Theta})$, as $\dot{\mbf{W}}_\ell(t)$ is the gradient of $f(\mbf{\Theta})$ with respect to $\mbf{W}_\ell$ by definition. By rearranging and multiplying by $\mbf{\Sigma}_\ell(t)$, we have
\begin{align}
\label{eqn:diagonal_grad}
      \mbf{U}^\top_\ell(t) \dot{\mbf{U}}_\ell(t) \mbf{\Sigma}_\ell(t) -   \mbf{\Sigma}_\ell(t) \mbf{V}^T (t) \dot{\mbf{V}}_\ell(t) = -  \hat{\mbf{I}}_{r} \odot [\mbf{U}^\top_\ell(t) \nabla_{\mbf{W}_{\ell}} f(\mbf{\Theta}) \mbf{V}_\ell(t)].
\end{align}
Hence, when $\dot{\mbf{U}}_\ell(t)=0$ and $\dot{\mbf{V}}_\ell(t)=0$, it must be that the left-hand side is zero and so $\mbf{U}^\top_\ell(t) \nabla_{\mbf{W}_{\ell}} f(\mbf{\Theta}) \mbf{V}_\ell(t)$ is a diagonal matrix. 

Now, notice that for the given loss function $f(\mbf{\Theta})$, we have
\begin{align*}
   -\dot{\mbf{W}}_\ell(t) = \nabla_{\mbf{W}_{\ell}} f(\mbf{\Theta}(t)) = \mbf{W}^{\top}_{L:\ell+1}(t) \cdot \left(\mbf{W}_{L:1}(t) - \mbf{M}_\star \right) \cdot \mbf{W}^{\top}_{\ell-1:1}(t). 
\end{align*}
Then, from Equation~(\ref{eqn:diagonal_grad}), when the singular vectors are stationary, we have
\begin{align*}
    \mbf{U}_\ell^\top(t)\mbf{W}^{\top}_{L:\ell+1}(t) \cdot \left(\mbf{W}_{L:1}(t) - \mbf{M}_\star \right) \cdot \mbf{W}^{\top}_{\ell-1:1}(t)\mbf{V}_\ell(t)
\end{align*}
must be a diagonal matrix for all $\ell \in [L]$. The only solution to the above should be (since the intermediate singular vectors need to cancel to satisfy the diagonal condition), is the set
\begin{align*}
\mathrm{SVS}(f(\mbf{\Theta})) = 
\begin{cases}
    (\mbf{U}_L, \mbf{V}_L) &= (\mbf{U}_\star, \mbf{Q}_L), \\
    (\mbf{U}_\ell, \mbf{V}_\ell) &= (\mbf{Q}_{\ell+1}, \mbf{Q}_\ell), \quad\forall \ell \in [2, L-1], \\
    (\mbf{U}_1, \mbf{V}_1) &= (\mbf{Q}_2, \mbf{V}_\star),
\end{cases}
\end{align*}
where \(\{\mbf{Q}_\ell\}_{\ell=2}^{L}\) are any set of orthogonal matrices. Then, notice that when the singular vectors are stationary, the dynamics become isolated on the singular values: \begin{align*}
   \dot{\mbf{\Sigma}}_\ell(t) = \mbf{I}_r \odot \left[ \mbf{U}^\top_\ell(t) \dot{\mbf{W}}_\ell(t) \mbf{V}_\ell(t) \right],
\end{align*} 
since $\left[ \mbf{U}^\top_\ell(t) \dot{\mbf{W}}_\ell(t) \mbf{V}_\ell(t) \right]$ is diagonal. This completes the proof.


\end{proof}


\begin{manualtheoreminner}
[Stable Subspace Oscillations]
Let $\alpha' \coloneqq \left( \ln\left( \frac{2\sqrt{2}}{\eta \lambda_1} \right) \cdot \frac{ \sigma_{\star, 1}^{4/L}}{L^2 \cdot 2^{\frac{2L-3}{L}}} \right)^{1/4}$.
Consider running GD on the loss in~(\ref{eqn:deep_mf}) with initialization scale $0<\alpha < \alpha'$.
    If $\eta = \frac{2}{K}$ with $\lambda_i \leq K< \lambda_{i+1}$, then under strict balancing, $2$-period orbit oscillation occurs in the direction of $\Delta_i$, where $\lambda_i$ and $\Delta_i$ denote the $i$-th largest eigenvalue and eigenvector of the Hessian at the balanced minimum, respectively.
      \label{thm:stable_sub}
\end{manualtheoreminner}
\begin{proof}

Define $f_{\Delta_i}$ as the 1-D function at the cross section of the loss landscape and the line
following the direction of $\Delta_i$ passing the (balanced) minima. To prove the result, we will invoke Lemma~\ref{lemma:chen-bruna}, which states that two-period orbit oscillation occurs in the direction of $\Delta_i$ if the minima of $f_{\Delta_i}$ satisfies $f_{\Delta_i}^{(3)}>0$ and $3[f_{\Delta_i}^{(3)}]^2 - f_{\Delta_i}^{(2)}f_{\Delta_i}^{(4)} > 0$, for $\eta>\frac{2}{\lambda_{i}}$. Recall that the initialization condition is an artifact of Proposition~\ref{prop:balancing}, which allows us to consider the balanced minimum. 


First, we will derive the eigenvectors of the Hessian of the training loss at convergence (i.e., $\mbf{M}_\star = \mbf{W}_{L:1}$).
    To obtain the eigenvectors of the Hessian of parameters $(\mbf{W}_L, \ldots, \mbf{W}_2, \mbf{W}_1)$, consider a small perturbation of the parameters:
    \begin{align*}
        \mbf{\Theta} \coloneqq \left(\Delta \mbf{W}_\ell +  \mbf{W}_\ell \right)_{\ell=1}^L =  (\mbf{W}_L + \Delta \mbf{W}_L, \ldots, \mbf{W}_2+ \Delta \mbf{W}_2, \mbf{W}_1+ \Delta \mbf{W}_1).
    \end{align*}

    
    Given that $\mbf{W}_{L:1} = \mbf{M}_\star$, consider and evaluate the loss function at this minima: 
    \begin{align}
        \mathcal{L}(\mbf{\Theta}) = \frac{1}{2} \biggl\| &\sum_{\ell} \mbf{W}_{L:\ell+1} \Delta \mbf{W}_\ell \mbf{W}_{\ell-1:1} \\
        &+ \sum_{\ell<m} \mbf{W}_{L:\ell+1} \Delta \mbf{W}_\ell \mbf{W}_{\ell-1:m+1} \Delta \mbf{W}_{m} \mbf{W}_{m-1:1}   +   \ldots   +  \Delta \mbf{W}_{L:1}\biggr\|^2_{\mathsf{F}}.
    \end{align}
    By expanding each of the terms and splitting by the orders of $\Delta \mbf{W}_\ell$ (perturbation), we get that the second-order term is equivalent to
    \begin{align*}
        \Theta&\left(\sum_{\ell=1}^L\|\Delta \mbf{W}_\ell\|^2\right): \,\, \frac{1}{2} \biggl\| \sum_{\ell} \mbf{W}_{L:\ell+1} \Delta \mbf{W}_\ell \mbf{W}_{\ell-1:1} \biggr\|^2_{\mathsf{F}} \\
        \Theta&\left(\sum_{\ell=1}^L\|\Delta \mbf{W}_\ell\|^3\right): \,\, \mathrm{tr}\left[\left(\sum_{\ell} \mbf{W}_{L:\ell+1} \Delta \mbf{W}_\ell \mbf{W}_{\ell-1:1} \right)^\top \left( \sum_{\ell<m} \mbf{W}_{L:\ell+1} \Delta \mbf{W}_\ell \mbf{W}_{\ell-1:m+1} \Delta \mbf{W}_{m} \mbf{W}_{m-1:1} \right)\right] \\
        \Theta&\left(\sum_{\ell=1}^L\|\Delta \mbf{W}_\ell\|^4\right): \,\, \frac{1}{2} \| \sum_{\ell<m} \mbf{W}_{L:\ell+1} \Delta \mbf{W}_\ell \mbf{W}_{\ell-1:m+1} \Delta \mbf{W}_{m} \mbf{W}_{m-1:1}\|^2_{\mathsf{F}}\\
        &+ \mathrm{tr}\left[\sum_{l} \left(\mbf{W}_{L:\ell+1}\Delta \mbf{W}_\ell \mbf{W}_{\ell-1:1} \right)^\top \left(\sum_{l<m<p} \mbf{W}_{L:\ell+1} \Delta \mbf{W}_\ell \mbf{W}_{\ell-1:m+1} \Delta \mbf{W}_{m} \mbf{W}_{m-1:p+1} \Delta \mbf{W}_{p} \mbf{W}_{p-1:1} \right)\right]
    \end{align*}

The direction of the steepest change in the loss at the minima correspond to the largest eigenvector direction of the Hessian. Since higher order terms such as $ \Theta\left(\sum_{\ell=1}^L\|\Delta \mbf{W}_\ell\|^3\right)$ are insignifcant compared to the second order terms $  \Theta\left(\sum_{\ell=1}^L\|\Delta \mbf{W}_\ell\|^2\right)$, finding the direction that maximizes the second order term leads to finding the eigenvector of the Hessian.
    Then, the eigenvector corresponding to the maximum eigenvalue of  $\nabla^2 \mathcal{L}$ is the solution of 
    \begin{align}
        \Delta_{1} \coloneqq \mathrm{vec}(\Delta \mbf{W}_L, \ldots \Delta \mbf{W}_1) = \underset{\|\Delta \mbf{W}_L\|^2_{\mathsf{F}} + \ldots + \|\Delta \mbf{W}_1\|^2_{\mathsf{F}} = 1}{\mathrm{arg max}} \, f\left(\Delta \mbf{W}_L, \ldots, \Delta \mbf{W}_1 \right),\label{max-eig}
    \end{align}
    where 
    \begin{align}
        f(\Delta \mbf{W}_L, \ldots, \Delta \mbf{W}_1) \coloneqq \frac{1}{2} \|\Delta \mbf{W}_L \mbf{W}_{L-1:1} + \ldots + \mbf{W}_{L:3}\Delta \mbf{W}_2 \mbf{W}_{1} + \mbf{W}_{L:2} \Delta \mbf{W}_1\|^2_{\mathsf{F}}.
    \end{align}

While the solution of Equation~(\ref{max-eig}) gives the maximum eigenvector direction of the Hessian, $\Delta_{1}$, the other eigenvectors can be found by solving
\begin{align}
    \Delta_{r} \coloneqq  \underset{
    \substack{
    \|\Delta \mbf{W}_L\|^2_{\mathsf{F}} + \ldots + \|\Delta \mbf{W}_1\|^2_{\mathsf{F}} = 1, \\
    \Delta_{r}\perp \Delta_{r-1},.., \Delta_{r}\perp \Delta_{1}
    }
    }{\mathrm{argmax}} \, f\left(\Delta \mbf{W}_L, \ldots, \Delta \mbf{W}_1 \right).\label{other-eig}
\end{align}

    By expanding $f(\cdot)$, %subject to the constraint ${\|\Delta \mbf{W}_L\|^2_{\mathsf{F}}} + \ldots + \|\Delta \mbf{W}_1\|^2_{\mathsf{F}} = 1$ ,
    we have that % we don't expand subject to a constraint
    \begin{align}
        f(\Delta \mbf{W}_L, &\ldots, \Delta \mbf{W}_1) = \|\Delta\mbf{W}_L \mbf{W}_{L-1:1}\|^2_{\mathsf{F}} +\ldots+ \|\mbf{W}_{L:3}\Delta \mbf{W}_2 \mbf{W}_{1}\|^2_{\mathsf{F}}  + \|\mbf{W}_{L:2} \Delta \mbf{W}_1\|^2_{\mathsf{F}} \notag \\
        &+ \mathrm{tr}\left[\left(\Delta\mbf{W}_L \mbf{W}_{L-1:1} \right)^\top \left(\mbf{W}_{L:3}\Delta \mbf{W}_2 \mbf{W}_{1} + \ldots +\mbf{W}_{L:2} \Delta \mbf{W}_1 \right)\right] + \ldots + \notag \\
        &\mathrm{tr}\left[\left(\mbf{W}_{L:2} \Delta \mbf{W}_1\right)^\top \left(\mbf{W}_{L:3}\Delta \mbf{W}_2 \mbf{W}_{1} + \ldots +\mbf{W}_{L:3}\Delta \mbf{W}_2 \mbf{W}_{1} \right)\right].     \label{expansion}
    \end{align}

We can solve Equation~(\ref{max-eig}) by maximizing each of the terms, which can be done in two steps:
\begin{enumerate}[label=(\roman*)]
\item 
Each Frobenius term in the expansion is maximized when the left singular vector of $\Delta \mbf{W}_{\ell}$ aligns with $\mbf{W}_{L:\ell+1}$ and the right singular vector aligns with $\mbf{W}_{\ell-1:1}$. This is a result of Von Neumann's trace inequality~\citep{mirsky1975trace}. Similarly, each term in the trace is maximized when the singular vector of the perturbations align with the products. 
\item Due to the alignment, Equation~(\ref{max-eig}) can be written in just the singular values. Let $\Delta s_{\ell, i}$ denote the $i$-th singular value of the perturbation matrix $\Delta\mbf{W}_\ell$. Recall that all of the singular values of $\mbf{M}_\star$ are distinct (i.e., $\sigma_{\star, 1} > \ldots>\sigma_{\star, r}$). Hence, it is easy to see that
Equation~(\ref{max-eig}) is maximized when $\Delta s_{\ell,i} = 0$ (i.e, all the weight goes to $\Delta s_{\ell,1}$). Thus, each perturbation matrix must be rank-$1$.
\end{enumerate}
Now since each perturbation is rank-$1$, we can write each perturbation as 
    \begin{align}
        \Delta\mbf{W}_{\ell} = \Delta s_{\ell} \Delta \mbf{u}_{\ell} \Delta\mbf{v}_\ell^\top, \quad \forall \ell \in [L],
    \end{align}
    % Then, notice that since the top-$r$ singular values of $\mbf{M}_\star$ are unique (i.e., $\sigma_{\star, 1} > \ldots > \sigma_{\star, r}$), the singular values of each $\mbf{W}_{\ell}$ are also unique, and hence the solution for each $\Delta\mbf{W}_{\ell}$ will be rank-$1$. We can express each solution as \
    for $\Delta s_{\ell} > 0$ and orthonormal vectors $\Delta \mbf{u}_{\ell} \in \mbb{R}^d$ and  $\Delta \mbf{v}_{\ell} \in \mbb{R}^d$ with $\sum_{\ell=1}^L \Delta s^2_{\ell} = 1$.
    Plugging this in each term, we obtain:
   \begin{align*}
        \|\mbf{W}_{L:\ell+1} \Delta_1 \mbf{W}_{\ell} \mbf{W}_{\ell-1:1}\|_2^2 = \Delta_1 s_\ell^2\cdot \biggl\|\underbrace{\mbf{V}_\star \mbf{\sigma}^{\frac{L-\ell}{L}}_\star \mbf{V}^\top_\star \Delta \mbf{u}_\ell}_{\eqqcolon \mbf{a}}\underbrace{ \Delta \mbf{v}_\ell^\top \mbf{V}_\star \mbf{\sigma}^{\frac{\ell-1}{L}}_\star \mbf{V}^\top_\star}_{\eqqcolon \mbf{b}^\top}\biggr\|_2^2.
    \end{align*}

    Since alignment maximizes this expression as discussed in first point, we have:
        % We first derive the leading eigenvector of the Hessian, denoted by $\Delta_1$. This makes repeated use of Von-Neumann trace inequality~, in that $\Delta \mbf{W}_\ell$ will have their singular vectors align.
    

    % To maximize $f(\cdot)$, we can find $\Delta \mbf{W}_\ell$ that maximizes each term in its expansion. Consider the Frobenius norm terms (e.g., $\|\mbf{W}_{L:\ell+1} \Delta \mbf{W}_{\ell} \mbf{W}_{\ell-1:1}\|^2_{\mathsf{F}}$). Since each $\Delta\mbf{W}_\ell$ solution is rank-$1$, it follows that each one of the matrices within the norm must also be at most rank-$1$. Then, we have
    % \begin{align*}
    %     \|\mbf{W}_{L:\ell+1} \Delta_1 \mbf{W}_{\ell} \mbf{W}_{\ell-1:1}\|^2_{\mathsf{F}} = \|\mbf{W}_{L:\ell+1} \Delta_1 \mbf{W}_{\ell} \mbf{W}_{\ell-1:1}\|^2_{2} &\leq \|\mbf{W}_{L:\ell+1}\|_2^2 \cdot \|\Delta_1 \mbf{W}_{\ell}\|_2^2 \cdot \|\mbf{W}_{\ell-1:1}\|_2^2 \\
    %     &= \Delta_1 s_{\ell}^{2} \cdot \sigma_{\star, 1}^{2 - \frac{2}{L}}.
    % \end{align*}
    % To obtain this upper bound, consider the following:
    % \begin{align*}
    %     \|\mbf{W}_{L:\ell+1} \Delta_1 \mbf{W}_{\ell} \mbf{W}_{\ell-1:1}\|_2^2 = \Delta_1 s_\ell^2\cdot \biggl\|\underbrace{\mbf{V}_\star \mbf{\sigma}^{\frac{L-\ell}{L}}_\star \mbf{V}^\top_\star\mbf{u}_\ell}_{\eqqcolon \mbf{a}}\underbrace{\mbf{v}_\ell^\top \mbf{V}_\star \mbf{\sigma}^{\frac{\ell-1}{L}}_\star \mbf{V}^\top_\star}_{\eqqcolon \mbf{b}^\top}\biggr\|_2^2.
    % \end{align*}
     $\mbf{u}_\ell =\mbf{v}_\ell = \mbf{v}_{\star, 1}$ for all $\ell \in [2, L-1]$, then
    \begin{align*}
        \mbf{a} = \sigma_{\star, 1}^{\frac{L-\ell}{L}}\mbf{v}_{\star, 1} \quad \text{and} \quad \mbf{b}^\top = \sigma_{\star, 1}^{\frac{\ell - 1}{L}}\mbf{v}_{\star, 1}^\top \implies \mbf{ab}^\top = \sigma_{\star, 1}^{1 - \frac{1}{L}} \cdot \mbf{v}_{\star, 1}\mbf{v}_{\star, 1}^\top.
    \end{align*}
    The very same argument can be made for the trace terms.
    Hence, in order to maximize $f(\cdot)$, we must have
    \begin{align*}
        \mbf{v}_L &= \mbf{v}_{\star, 1}, \quad \text{and} \quad \mbf{u}_1 = \mbf{v}_{\star, 1}, \\
        \mbf{u}_\ell &= \mbf{v}_\ell = \mbf{v}_{\star, 1}, \quad \forall \ell \in [2, L-1].
    \end{align*}
    To determine $\mbf{u}_L$ and $\mbf{v}_1$, we can look at one of the trace terms:
    \begin{align*}
    \mathrm{tr}\left[\left(\Delta_1\mbf{W}_L \mbf{W}_{L-1:1} \right)^\top \left(\mbf{W}_{L:3}\Delta_1 \mbf{W}_2 \mbf{W}_{1} + \ldots +\mbf{W}_{L:2} \Delta_1 \mbf{W}_1 \right)\right] \leq \left(\frac{L-1}{L} \right)\cdot\sigma_{\star, 1}^{2 - \frac{2}{L}}.
    \end{align*}
    To reach the upper bound, we require $\mbf{u}_L = \mbf{u}_{\star, 1}$ and $\mbf{v}_1 = \mbf{v}_{\star, 1}$. Finally, as the for each index, the singular values are balanced, we will have  $\Delta_1 s_{\ell} = \frac{1}{\sqrt{L}}$ for all $\ell \in [L]$ to satisfy the constraint. Finally, we get that the leading eigenvector is
    \begin{align*}
        \Delta_1 \coloneqq \mathrm{vec}\left(\frac{1}{\sqrt{L}}\mbf{u}_1 \mbf{v}_1^\top, \frac{1}{\sqrt{L}}\mbf{v}_1 \mbf{v}_1^\top, \ldots, \frac{1}{\sqrt{L}}\mbf{v}_1 \mbf{v}_1^\top \right).
    \end{align*}
    Notice that we can also verify that $f(\Delta_1) = L\sigma_{\star, 1}^{2- \frac{2}{L}}$, which is the leading eigenvalue (or sharpness) derived in Lemma~\ref{lemma:hessian_eigvals}.  

    To derive the remaining eigenvectors, we need to find all of the vectors in which $\Delta_i^\top \Delta_j = 0$ for $i\neq j$, where
    \begin{align*}
        \Delta_i = \mathrm{vec}(\Delta_i \mbf{W}_L, \ldots \Delta_i \mbf{W}_1),
    \end{align*}
    and $f(\Delta_i) = \lambda_i$, where $\lambda_i$ is the $i$-th largest eigenvalue. By repeating the same process as above, we find that the eigenvector-eigenvalue pair as follows:
    \begin{align*}
        \Delta_1 &= \mathrm{vec}\left(\frac{1}{\sqrt{L}}\mbf{u}_1 \mbf{v}_1^\top, \frac{1}{\sqrt{L}}\mbf{v}_1 \mbf{v}_1^\top, \ldots, \frac{1}{\sqrt{L}}\mbf{v}_1 \mbf{v}_1^\top \right) , \quad\lambda_{1} =  L\sigma_{\star, 1}^{2- \frac{2}{L}} \\
        \Delta_2 &= \mathrm{vec}\left(\frac{1}{\sqrt{L}}\mbf{u}_1 \mbf{v}_2^\top, \frac{1}{\sqrt{L}}\mbf{v}_1 \mbf{v}_2^\top, \ldots, \frac{1}{\sqrt{L}}\mbf{v}_1 \mbf{v}_2^\top \right), \quad\lambda_{2} =  \left(\sum_{i=0}^{L-1} \sigma_{\star, 1}^{1-\frac{1}{L}-\frac{1}{L}i} \cdot \sigma_{\star, 2}^{\frac{1}{L}i} \right) \\
        \Delta_3 &= \mathrm{vec}\left(\frac{1}{\sqrt{L}}\mbf{u}_2 \mbf{v}_1^\top, \frac{1}{\sqrt{L}}\mbf{v}_2 \mbf{v}_1^\top, \ldots, \frac{1}{\sqrt{L}}\mbf{v}_2 \mbf{v}_1^\top \right), \quad\lambda_{3} =  \left(\sum_{i=0}^{L-1} \sigma_{\star, 1}^{1-\frac{1}{L}-\frac{1}{L}i} \cdot \sigma_{\star, 2}^{\frac{1}{L}i} \right) \\
        \quad\quad\quad&\vdots \\
         \Delta_d &= \mathrm{vec}\left(\frac{1}{\sqrt{L}}\mbf{u}_2 \mbf{v}_2^\top, \frac{1}{\sqrt{L}}\mbf{v}_2 \mbf{v}_2^\top, \ldots, \frac{1}{\sqrt{L}}\mbf{v}_2 \mbf{v}_2^\top \right), \quad\lambda_{d} =  L\sigma_{\star, 2}^{2- \frac{2}{L}} \\     
        \quad\quad\quad&\vdots \\
        \Delta_{dr+r} &= \mathrm{vec}\left(\frac{1}{\sqrt{L}}\mbf{u}_d \mbf{v}_r^\top, \frac{1}{\sqrt{L}}\mbf{v}_d \mbf{v}_r^\top, \ldots, \frac{1}{\sqrt{L}}\mbf{v}_d \mbf{v}_r^\top \right),
    \end{align*}
    which gives a total of $dr + r$ eigenvectors.

    Second, equipped with the eigenvectors, let us consider the 1-D function $f_{\Delta_i}$ generated by the cross-section of the loss landscape and each eigenvector $\Delta_i$ passing the minima:
    \begin{align*}
        f_{\Delta_i}(\mu) &= \mathcal{L}(\mbf{W}_L + \mu\Delta \mbf{W}_L, \ldots, \mbf{W}_2+ \mu\Delta \mbf{W}_2, \mbf{W}_1+ \mu\Delta \mbf{W}_1), \\
        &= \mu^2\cdot \frac{1}{2} \|\Delta \mbf{W}_L \mbf{W}_{L-1:1} + \ldots + \mbf{W}_{L:3}\Delta \mbf{W}_2 \mbf{W}_{1} + \mbf{W}_{L:2} \Delta \mbf{W}_1\|^2_{\mathsf{F}}\\
        \quad&+\mu^3 \cdot \sum_{\ell=1, \ell< m}^L\mathrm{tr}\left[\left(\mbf{W}_{L:\ell+1}\Delta \mbf{W}_\ell \mbf{W}_{\ell-1:1} \right)^\top \left( \mbf{W}_{L:\ell+1} \Delta \mbf{W}_\ell \mbf{W}_{\ell-1:m+1} \Delta \mbf{W}_{m} \mbf{W}_{m-1:1} \right)\right] \\
        \quad&+\mu^4\cdot \frac{1}{2} \left\|  \left( \sum_{\ell<m} \mbf{W}_{L:\ell+1} \Delta \mbf{W}_\ell \mbf{W}_{\ell-1:m+1} \Delta \mbf{W}_{m} \mbf{W}_{m-1:1} \right) \right\|^2_{\mathsf{F}}\\
        &+ \mu^4 \cdot\sum_{\ell<m<p} ^L \mathrm{tr}\left[\left(\mbf{W}_{L:\ell+1}\Delta \mbf{W}_\ell \mbf{W}_{\ell-1:1} \right)^\top  \left(\mbf{W}_{L:\ell+1} \Delta \mbf{W}_\ell \mbf{W}_{\ell-1:m+1} \Delta \mbf{W}_{m} \mbf{W}_{m-1:p+1} \Delta \mbf{W}_{p} \mbf{W}_{p-1:1} \right)\right].
    \end{align*}
    Then, the several order derivatives of $f_{\Delta_i}(\mu)$ at $\mu = 0$ can be obtained from Taylor expansion as
    \begin{align*}
        f_{\Delta_i}^{(2)}(0) &= \|\Delta_i \mbf{W}_L \mbf{W}_{L-1:1} + \ldots + \mbf{W}_{L:3}\Delta_i \mbf{W}_2 \mbf{W}_{1} + \mbf{W}_{L:2} \Delta_i \mbf{W}_1\|^2_{\mathsf{F}} = \lambda^2_{i}\\
        f_{\Delta_i}^{(3)}(0) &= 6\sum_{\ell=1}^L\mathrm{tr}\left[\left(\mbf{W}_{L:\ell+1}\Delta_i \mbf{W}_\ell \mbf{W}_{\ell-1:1} \right)^\top \left(\mbf{W}_{L:\ell+2}\Delta_i \mbf{W}_{\ell+1} \mbf{W}_\ell\Delta_i\mbf{W}_{\ell-1} \mbf{W}_{\ell-2:1} \right)\right] \\
        & = 6 \biggl\| \sum_{\ell} \mbf{W}_{L:\ell+1}\Delta_i \mbf{W}_\ell \mbf{W}_{\ell-1:1} \biggr\|_{\mathsf{F}}\cdot \biggl\| \left( \sum_{\ell<m} \mbf{W}_{L:\ell+1} \Delta \mbf{W}_\ell \mbf{W}_{\ell-1:m+1} \Delta \mbf{W}_{m} \mbf{W}_{m-1:1} \right) \biggr\|_{\mathsf{F}}\\
        & \coloneqq 6  \lambda_{i}\cdot\beta_{i} \\
        f_{\Delta_i}^{(4)}(0) &= 12\|\Delta_i \mbf{W}_L \Delta_i\mbf{W}_{L-1}\mbf{W}_{L-2:1} + \ldots + \mbf{W}_{L:4}\Delta_i \mbf{W}_3 \mbf{W}_{2}\Delta_i\mbf{W}_1 + \mbf{W}_{L:3}\Delta_i\mbf{W}_2 \Delta_i \mbf{W}_1\|^2_{\mathsf{F}} \\
        &+ 24\sum_{\ell=1}^L \mathrm{tr}\left[\left(\mbf{W}_{L:\ell+1}\Delta_i \mbf{W}_\ell \mbf{W}_{\ell-1:1} \right)^\top \left(\sum_{l<m<p} \mbf{W}_{L:\ell+1} \Delta \mbf{W}_\ell \mbf{W}_{\ell-1:m+1} \Delta \mbf{W}_{m} \mbf{W}_{m-1:p+1} \Delta \mbf{W}_{p} \mbf{W}_{p-1:1} \right)\right] \\
        &\coloneqq 12\beta^2_{i} + 24\lambda_{i}\cdot\delta_{i},
    \end{align*}
  
    % \begin{align*}
    %     3[f_{\Delta_i}^{(3)}]^2 - f_{\Delta_i}^{(2)}f_{\Delta_i}^{(4)} &= 108\beta\|\Delta_i \mbf{W}_L \mbf{W}_{L-1:1} + \ldots + \mbf{W}_{L:3}\Delta_i \mbf{W}_2 \mbf{W}_{1} + \mbf{W}_{L:2} \Delta_i \mbf{W}_1\|^2_{\mathsf{F}} \\
    %     &- 12\beta\|\Delta_i \mbf{W}_L \mbf{W}_{L-1:1} + \ldots + \mbf{W}_{L:3}\Delta_i \mbf{W}_2 \mbf{W}_{1} + \mbf{W}_{L:2} \Delta_i \mbf{W}_1\|^2_{\mathsf{F}} \\
    %     &- 24\gamma\|\Delta_i \mbf{W}_L \mbf{W}_{L-1:1} + \ldots + \mbf{W}_{L:3}\Delta_i \mbf{W}_2 \mbf{W}_{1} + \mbf{W}_{L:2} \Delta_i \mbf{W}_1\|^2_{\mathsf{F}} \\
    %     &= 96\beta\|\Delta_i \mbf{W}_L \mbf{W}_{L-1:1} + \ldots + \mbf{W}_{L:3}\Delta_i \mbf{W}_2 \mbf{W}_{1} + \mbf{W}_{L:2} \Delta_i \mbf{W}_1\|^2_{\mathsf{F}} \\
    %     &- 24\gamma\|\Delta_i \mbf{W}_L \mbf{W}_{L-1:1} + \ldots + \mbf{W}_{L:3}\Delta_i \mbf{W}_2 \mbf{W}_{1} + \mbf{W}_{L:2} \Delta_i \mbf{W}_1\|^2_{\mathsf{F}}.
    % \end{align*}

    where we defined 
    \begin{align*}
        & \lambda_{i} = \biggl\| \sum_{\ell} \mbf{W}_{L:\ell+1} \Delta_{i} \mbf{W}_\ell \mbf{W}_{\ell-1:1}  \biggr\|_{\mathsf{F}} \quad \tag{Total $L\choose 1$ terms}\\
        & \beta_{i} =\biggl\| \left( \sum_{\ell<m} \mbf{W}_{L:\ell+1} \Delta \mbf{W}_\ell \mbf{W}_{\ell-1:m+1} \Delta \mbf{W}_{m} \mbf{W}_{m-1:1} \right)\biggr\|_{\mathsf{F}} \quad \tag{Total $L\choose 2$ terms}\\
        & \delta_{i} = \biggl\| \left(\sum_{l<m<p} \mbf{W}_{L:\ell+1} \Delta \mbf{W}_\ell \mbf{W}_{\ell-1:m+1} \Delta \mbf{W}_{m} \mbf{W}_{m-1:p+1} \Delta \mbf{W}_{p} \mbf{W}_{p-1:1} \right) \biggr\|_{\mathsf{F}}, \quad \tag{Total $L\choose 3$ terms}
    \end{align*}
and used the fact that $\mathrm{tr}(\mbf{A}^\top \mbf{B}) = \| \mbf{A} \|_{\mathsf{F}}\cdot \| \mbf{B}\|_{\mathsf{F}}$ under singular vector alignment.

Then, since $\beta_{i} $ has $L\choose 2$ terms inside the sum, when the Frobenium term is expanded, it will have $\frac{{L\choose 2}\left({L\choose 2}+1\right)}{2}$ number of terms. 
Under alignment and balancedness, $\beta^{2}_{i} = \Delta s^2_{\ell} \sigma^{2-\frac{4}{L}}_{i}  \times \frac{{L\choose 2}\left({L\choose 2}+1\right)}{2}$ and $\lambda_{i} \delta_{i} =  \Delta s^2_{\ell} \sigma^{2-\frac{4}{L}}_{i}  \times {L\choose 3} L$. Thus, we have the expression
\begin{align*}
   2\beta^{2}_{i} - \lambda_{i} \delta_{i} &= \Delta s^2_{\ell} \sigma^{2-\frac{4}{L}}_{i} \left( 2 \frac{\binom{L}{2}\left(\binom{L}{2} + 1\right)}{2} -  \binom{L}{3} L \right) \\
   &= \Delta s^2_{\ell} \sigma^{2-\frac{4}{L}}_{i}  \binom{L}{3} L \times \left( \frac{3\left(\frac{L(L-1)}{2}+1\right)}{L(L-2)} -1 \right) \\
   & =  \Delta s^2_{\ell} \sigma^{2-\frac{4}{L}}_{i} \frac{2 \binom{L}{3} L }{L(L-2)} \times \left( (L-1)^2  + 5\right) > 0,\\
\end{align*}
for any depth $L>2$. Finally, the condition of stable oscillation of 1-D function is
\begin{align*}
       &  3[f_{\Delta_i}^{(3)}]^2 - f_{\Delta_i}^{(2)}f_{\Delta_i}^{(4)} =   108 \lambda^2_{i}\beta^{2}_{i} -  ( \lambda^{2}_{i})( 12\beta^{2}_{i} + 24(2\lambda_{i})(\delta_{i})) = 48 \lambda^{2}_{i} ( 2\beta^{2}_{i} - \lambda_{i} \delta_{i}  ) > 0,
\end{align*}
which we have proven to be positive for any depth $L>2$, for all the eigenvector directions corresponding to the non-zero eigenvalues. This completes the proof. 
    % Then, notice that from the first part of the proof,
    % \begin{align*}
    %     \|\Delta_i \mbf{W}_L \mbf{W}_{L-1:1} + \ldots + \mbf{W}_{L:3}\Delta_i \mbf{W}_2 \mbf{W}_{1} + \mbf{W}_{L:2} \Delta_i \mbf{W}_1\|^2_{\mathsf{F}} = 2\lambda_i > 0,
    % \end{align*}
    
\end{proof}



\begin{manualtheoreminner}[Rank-$p$ Periodic Subspace Oscillations]

Let $\mbf{M}_\star = \mbf{U}_\star \mbf{\Sigma}_\star \mbf{V}_\star^\top$ denote the SVD of the target matrix and define $S_p\coloneqq L \sigma^{2-\frac{2}{L}}_{\star,p}$ and $K'_p \coloneqq \mathrm{max} \left\{ S_{p+1},\frac{S_p}{2\sqrt{2}}\right\}$.
If we run GD on the deep matrix factorization loss with initialization scale $\alpha < \alpha'$ from Theorem~\ref{thm:stable_oscillations} and learning rate $\eta = \frac{2}{K}$, where $K'_p < K< S_p$, then under strict balancing, the top-$p$ singular values of the end-to-end DLN oscillates in a $2$-period orbit ($j \in \{1,2\}$) around the balanced minimum and admits the following decomposition:
\begin{align}
    \mbf{W}_{L:1} = \underbrace{\sum_{i=1}^p\rho_{i, j}^L \cdot \mbf{u}_{\star, i}\mbf{v}_{\star, i}^{\top} }_{\text{oscillation subspace}}+ \underbrace{\sum_{k=p+1}^d \sigma_{\star, k}\cdot \mbf{u}_{\star, k}\mbf{v}_{\star, k}^{\top}}_{\text{stationary subspace}}, \quad j \in \{1,2\}, \quad \forall\ell \in [L-1],
\end{align}
where $\rho_{i, 1} \in \left(0, \sigma_{\star, i}^{1/L}\right)$ and $\rho_{i, 2} \in \left(\sigma_{\star, i}^{1/L}, (2\sigma_{\star, i})^{1/L}\right)$ are the two real roots of the polynomial $g(\rho_i)=0$ and
\begin{align*}
    g(\rho_i) = \rho_i^L\cdot\frac{1+\left(1 + \eta L(\sigma_{\star, i} - \rho_i^L)\cdot \rho_i^{L-2} \right)^{2L-1}}{1+\left(1 + \eta L(\sigma_{\star, i} - \rho_i^L)\cdot \rho_i^{L-2} \right)^{L-1}} - \sigma_{\star, i}.
\end{align*}
\label{main:thm}
\end{manualtheoreminner}

\begin{proof}

To prove the result, we will consider the GD step on the $i$-th singular value and show that the $2$-period orbit condition holds given the learning rate $\eta = \frac{2}{K}$.
For ease of exposition, let us denote the $i$-th singular value of each $\mbf{W}_\ell$ as $\sigma_{i} \coloneqq \sigma_{\ell, i}$. Under balancing, consider the two-step GD update on the first singular value:
\begin{align*}
    \sigma_i(t+1) &= \sigma_i(t) + \eta L \cdot \left(\sigma_{\star, i} - \sigma_i^L(t)\right)\cdot \sigma^{L-1}_{i}(t) \\
      \sigma_i(t) = \sigma_i(t+2) &= \sigma_i(t+1) + \eta L \cdot \left(\sigma_{\star, i} - \sigma_i^L(t+1)\right)\cdot \sigma^{L-1}_{i}(t+1). \tag{By 2-period orbit}
\end{align*}
Define $z \coloneqq \left(1 + \eta L \cdot \left(\sigma_{\star, i} - \sigma_i^L(t)\right)\cdot \sigma^{L-2}_{i}(t) \right)$ and by plugging in $\sigma_i(t+1)$ for $\sigma_i(t)$, we have
\begin{align*}
    \sigma_i(t) &= \sigma_i(t) z + \eta L \cdot \left(\sigma_{\star, i} - \sigma_i^L(t)z^L \right) \cdot \sigma_i^{L-1}(t)z^{L-1} \\
    \implies 1 &= z + \eta L \cdot \left(\sigma_{\star, i} - \sigma_i^L(t)z^L \right) \cdot \sigma_i^{L-2}(t)z^{L-1} \\
    \implies 1 &= \left(1 + \eta L \cdot \left(\sigma_{\star, i} - \sigma_i^L(t)\right)\cdot \sigma^{L-2}_{i}(t) \right) + \eta L \cdot \left(\sigma_{\star, i} - \sigma_i^L(t)z^L \right) \cdot \sigma_i^{L-2}(t)z^{L-1} \\
    \implies 0 &= \left(\sigma_{\star, i} - \sigma_i^L(t)\right) + \left(\sigma_{\star, i} - \sigma_i^L(t)z^L \right) \cdot z^{L-1}
\end{align*}
Simplifying this expression further, we have
\begin{align*}
    &0 = \sigma_{\star, i} - \sigma_i^L(t) + \sigma_{\star, i} z^{L-1} - \sigma_i^L(t) z^{2L-1} \\
    \implies &\sigma_i^L(t) + \sigma_i^L(t) z^{2L-1} =  \sigma_{\star, i} + \sigma_{\star, i} z^{L-1} \\
    \implies &\sigma_i^L(t)\cdot\left(1 + z^{2L - 1} \right) = \sigma_{\star, i}\cdot\left(1 + z^{L - 1} \right) \\
    \implies &\sigma_i^L(t)\frac{\left(1 + z^{2L - 1} \right)}{\left(1 + z^{L - 1} \right)} = \sigma_{\star, i},
\end{align*}
and by defining $\rho_i \coloneqq \sigma_i(t)$, we obtain the polynomial
\begin{align*}
    \sigma_{\star, i} = \rho_i^L\frac{1+z^{2L-1}}{1+z^{L-1}}, \quad \text{where  } \, z \coloneqq \left(1 + \eta L(\sigma_{\star, i} - \rho_i^L)\cdot \rho_i^{L-2} \right).
\end{align*}
Next, we show the existence of (real) roots within the ranges for $\rho_{i,1}$ and $\rho_{i, 2}$. We note that these roots only exist within the EOS regime.
First, consider $\rho_{i, 1} \in \left(0, \sigma_{\star, i}^{1/L} \right)$. We will show that for two values within this range, there is a sign change for all $L \geq 2$. More specifically, we show that there exists $\rho_i \in \left(0, \sigma_{\star, i}^{1/L} \right)$ such that
\begin{align*}
     \rho_i^L\frac{1+z^{2L-1}}{1+z^{L-1}} - \sigma_{\star, i} > 0 \quad \text{and} \quad \rho_i^L\frac{1+z^{2L-1}}{1+z^{L-1}} - \sigma_{\star, i} < 0.
\end{align*}
For the positive case, consider $\rho_i = (\frac{1}{2}\sigma_{\star, i})^{1/ L}$. We need to show that 
\begin{align*}
    \frac{1+z^{2L-1}}{1+z^{L-1}}  = \frac{1 + \left(1+\eta L\cdot\left(\frac{\sigma_{\star, i}}{2}\right)\frac{\sigma_{\star, i}^{1-\frac{2}{L}}}{2^{1 - \frac{2}{L}}}\right)^{2L-1}}{1 + \left(1+\eta L\cdot\left(\frac{\sigma_{\star, i}}{2}\right)\frac{\sigma_{\star, i}^{1-\frac{2}{L}}}{2^{1 - \frac{2}{L}}}\right)^{L-1}} > 2.
\end{align*}
To do this, we will plug in the smallest possible value of $\eta = \frac{2}{L\sigma_{\star, i}^{2 - \frac{2}{L}}}$ to show that the fraction is still greater than $2$, which gives us
\begin{align}
\label{eqn:first_range_pos}
    u(L) \coloneqq \frac{1 + \left(1+\frac{1}{ 2^{1 - \frac{2}{L}}} \right)^{2L-1}}{1 + \left(1+\frac{1}{ 2^{1 - \frac{2}{L}}} \right)^{L-1}},
\end{align}
which is an increasing function of $L$ for all $L\geq 2$. Since $u(2) > 2$, Equation~(\ref{eqn:first_range_pos}) must always be greater than $2$. For the negative case, we can simply consider $\rho_i = 0$.
Hence, since the polynomial is continuous, by the Intermediate Value Theorem (IVT), there must exist a root within the range $\rho_i \in \left(0, \sigma_{\star, i}^{1/L} \right)$.


Next, consider the range $\rho_{i, 2} \in \left(\sigma_{\star, i}^{1/L}, (2\sigma_{\star, i})^{1/L}\right)$. Similarly, we will show sign changes for two values in $\rho_{i, 2}$.
For the positive case, consider $\rho_i = \left(\frac{3}{2} \sigma_{\star, i}\right)^{1/L}$. For $\eta$, we can plug in the smallest possible value within the range to show that this value of $\rho_i$  provides a positive quantity. Specifically, we need to show that
\begin{align*}
    \frac{1+z^{2L-1}}{1+z^{L-1}} > \frac{2}{3} \implies \frac{1+\left(1+\frac{2}{\sigma_{\star, i}^{2- \frac{2}{L}}}\cdot(\sigma_{\star, i} - \frac{3}{2}\sigma_{\star, i})\cdot \left(\frac{3}{2}\sigma_{\star, i}\right)^{1 - \frac{2}{L}} \right)^{2L-1}}{1+\left(1+\frac{2}{\sigma_{\star, i}^{2- \frac{2}{L}}}\cdot(\sigma_{\star, i} - \frac{3}{2}\sigma_{\star, i})\cdot \left(\frac{3}{2}\sigma_{\star, i}\right)^{1 - \frac{2}{L}} \right)^{L-1}} > \frac{2}{3}.
\end{align*}
We can simplify the fraction as follows:
\begin{align*}
    \frac{1+\left(1+\frac{2}{\sigma_{\star, 1}^{2- \frac{2}{L}}}\cdot(\sigma_{\star, 1} - \frac{3}{2}\sigma_{\star, 1})\cdot \left(\frac{3}{2}\sigma_{\star, 1}\right)^{1 - \frac{2}{L}} \right)^{2L-1}}{1+\left(1+\frac{2}{\sigma_{\star, 1}^{2- \frac{2}{L}}}\cdot(\sigma_{\star, 1} - \frac{3}{2}\sigma_{\star, 1})\cdot \left(\frac{3}{2}\sigma_{\star, 1}\right)^{1 - \frac{2}{L}} \right)^{L-1}} = 
    \frac{1+\left(1-(\frac{3}{2})^{1 - \frac{2}{L}} \right)^{2L-1}}{1+\left(1-(\frac{3}{2})^{1 - \frac{2}{L}} \right)^{L-1}}.
\end{align*}
Then, since we are subtracting by $(\frac{3}{2})^{1 - \frac{2}{L}}$, we can plug in its largest value for $L\geq 2$, which is $3/2$. This gives us 
\begin{align*}
    \frac{1+\left(-0.5\right)^{2L-1}}{1+\left(-0.5 \right)^{L-1}} > \frac{2}{3},
\end{align*}
as for odd values of $L$, the function increases to $1$ starting from $L=2$, and decreases to $1$ for even $L$. 
To check negativity, let us define
\begin{align*}
    h(\rho) \coloneqq \frac{f(\rho)}{g(\rho)} \coloneqq \frac{\rho^L \left(1 + z^{2L-1} \right)}{1 + z^{L-1}}.
\end{align*}
We will show that $h'\left(\sigma_{\star, i}^{1/L} \right) < 0$:
\begin{align*}
h'\left(\sigma_{\star, i}^{1/L} \right) &= \frac{f'\left(\sigma_{\star, i}^{1/L} \right)g\left(\sigma_{\star, i}^{1/L} \right) - f\left(\sigma_{\star, i}^{1/L} \right)g'\left(\sigma_{\star, i}^{1/L} \right)}{g^2\left(\sigma_{\star, i}^{1/L} \right)} \\
&= \frac{f'\left(\sigma_{\star, i}^{1/L} \right) - \sigma_{\star, i}\cdot g'\left(\sigma_{\star, i}^{1/L} \right)}{2} \\
&= \frac{L\sigma_{\star, i}^{1 - \frac{1}{L}} - \sigma_{\star, i}(2L-1)\left(\eta L^2 \sigma_{\star, i}^{2 -\frac{3}{L}} \right) - \sigma_{\star, i}(L-1)\left(\eta L^2 \sigma_{\star, i}^{2 -\frac{3}{L}} \right) }{2} \\
&= \frac{L\sigma_{\star, i}^{1 - \frac{1}{L}} - (3L-2)\left(\eta L^2 \sigma_{\star, i}^{3 -\frac{3}{L}} \right) }{2} < 0,
\end{align*}
as otherwise we need $\eta \leq \frac{\sigma_{\star, i}^{2/L - 2}}{3L^2 - 2L}$, which is out of the range of interest. Since $h'(\rho)< 0$, it follows that there exists a $\delta > 0$ such that $h(\rho) > h(x)$ for all $x$ such that $\rho < x < \rho+\delta$. Lastly, since $h(\rho) - \sigma_{\star, i} = 0$ for $\rho = \sigma_{\star, i}^{1/L}$, it follows that $h(\rho) - \sigma_{\star, i}$ must be negative at $\rho + \delta$.
Similarly, by IVT, there must exist a root within the range 
$\rho_{i,2} \in \left(\sigma_{\star, i}^{1/L}, (2\sigma_{\star, i})^{1/L}\right)$. This proves that the $i$-th singular value undergoes a two-period orbit with the roots $\rho_{i, 1}$ and $\rho_{i, 2}$. Then, notice that if the learning rate is large enough to induce oscillations in the $i$-th singular value, then it is also large enough to have oscillations in all singular values from $1$ to the $(i-1)$-th singular value (assuming that it is not large enough for divergence). Finally, at the (balanced) minimum, we can express the dynamics as 
\begin{align}
    \mbf{W}_{L:1} = \underbrace{\sum_{i=1}^p\rho_{i, j}^L \cdot \mbf{u}_{\star, i}\mbf{v}_{\star, i}^{\top} }_{\text{oscillation subspace}}+ \underbrace{\sum_{k=p+1}^d \sigma_{\star, k}\cdot \mbf{u}_{\star, k}\mbf{v}_{\star, k}^{\top}}_{\text{stationary subspace}}, \quad j \in \{1,2\}, \quad \forall\ell \in [L-1].
\end{align}
This completes the proof.


\end{proof}







\begin{manuallemmainner}[Balancing]
  Let $\sigma_{\star, i}$ and $\sigma_{\ell, i}(t)$ denote the $i$-th singular value of $\mbf{M}_\star \in \mbb{R}^{d\times d}$ and $\mbf{W}_\ell(t)$, respectively and define $S_i \coloneqq L \sigma^{2-\frac{2}{L}}_{\star,i}$.
    Consider GD on the $i$-th index of the simplified loss in~(\ref{eqn:simplified_loss}) with the unbalanced initialization and learning rate $\frac{2}{S_i} < \eta < \frac{2\sqrt{2}}{S_i}$. If the initialization scale $\alpha$ satisfies
    $0 < \alpha < \left( \ln\left( \frac{2\sqrt{2}}{\eta S_i} \right) \cdot \frac{ \sigma_{\star, i}^{4/L}}{L^2 \cdot 2^{\frac{2L-3}{L}}} \right)^{1/4}$, then there exists a constant $c \in (0, 1]$ such that for all $\ell \in [L-1]$, we have $\left| \sigma^2_{L, i}(t+1) - \sigma^2_{\ell, i}(t+1)\right| < c\cdot \left| \sigma^2_{L, i}(t) - \sigma^2_{\ell, i}(t)\right|$.
\end{manuallemmainner}

\begin{proof}



To prove the result, we adopt the analysis from~\cite{kreisler2023gradient}, where they use the notion of gradient flow solution (GFS) sharpness defined below:
\begin{definition}[GFS Sharpness]
    The GFS sharpness denoted by $\psi(x)$ is the sharpness achieved by the global minima which lies in the same GF trajectory of $x$ (i.e., $\|\nabla^2 L(z)\|$ such that $L(z)=0$ and $z = GF(x)$, where $GF(\cdot)$ denotes the gradient flow solution).
\end{definition}

\noindent Then, let us consider the $i$-th index of the simplified loss in~(\ref{eqn:simplified_loss}):
\begin{align*}
    \frac{1}{2} \left(\prod_{\ell=1}^L \sigma_{\ell, i} - \sigma_{\star, i}  \right)^2 \eqqcolon \frac{1}{2} \left(\prod_{\ell=1}^L \sigma_{\ell} - \sigma_{\star}  \right)^2  ,
\end{align*}
and omit the dependency on $i$ for ease of exposition. Our goal is to show that the $L$-th singular value $\sigma_L$ initialized to zero become increasingly balanced to $\sigma_\ell$ which are initialized to $\alpha$.
%So, first we show that in a singular value scalar loss, for a learning rate $\eta > \frac{2}{S_{i}}$, oscillations occur provably for any initialization range $0<\alpha$. We do this in the following steps: 1) show that the sharpness around the global minima is the least when iterates are balanced, 2) By using the descent lemma, if $\eta>\frac{2}{S_{i}}$, then oscillations start occuring at the balanced point, 3) By lemma-1, if oscillations can occur at balanced point, then oscillation can occur anywhere around the global minima. So, $\eta>\frac{2}{S_{i}}$ is a sufficient condition to show oscillation. \footnote{Oscillations can also start occuring for some $\eta<\frac{2}{S_{i}}$ but will eventually subside once it reaches close to balanced minima. }
To that end, let us define the balancing dynamics between $\sigma_i$ and $\sigma_j$ as $b_{i,j}^{(t+1)} \coloneqq \left(\sigma_i^{(t+1)}\right)^2 - \left(\sigma_j^{(t+1)}\right)^2$ and $\pi^{(t)} \coloneqq \prod_{\ell=1}^L \sigma_{\ell}(t)$ for the product of singular values at iteration $t$.
We can simplify the balancing dynamics as follows:
% \begin{align*}
%     \pi^{(t+1)} = \prod_{i=1}^{L} \sigma_{i}^{(t+1)} 
%     &= \prod_{i=1}^{D} \left(\sigma_i^{(t)} - \eta \left(\pi^{(t)} - 1 \right)\frac{\pi^{(t)}}{\sigma_i^{(t)}} \right) \\
%     &= \pi^{(t)} \prod_{i=1}^{L} \left(1 - \eta \left(\pi^{(t)} - 1 \right) \frac{\pi^{(t)}}{\left(\sigma_i^{(t)}\right)^2}\right) \\
%     &= \pi^{(t)} + \sum_{m=1}^{L} \eta^m (1 - \pi^{(t)})^m \pi^{(t)} \sigma_m(\sigma^{(t)}).
% \end{align*}

% Defining  to be the balance,
% The dynamic of the balances then becomes:
\begin{align*}
    b_{i,j}^{(t+1)} &= \left(\sigma_i^{(t+1)}\right)^2 - \left(\sigma_j^{(t+1)}\right)^2 \\
    &= \left(\sigma_i^{(t)} - \eta\left(\pi^{(t)} - \sigma_{\star}\right)\frac{\pi^{(t)}}{\sigma_i^{(t)}}\right)^2 - \left(\sigma_j^{(t)} - \eta\left(\pi^{(t)} - \sigma_{\star}\right)\frac{\pi^{(t)}}{\sigma_j^{(t)}}\right)^2 \\
    &= \left(\sigma_i^{(t)}\right)^2 - \left(\sigma_j^{(t)}\right)^2 + \eta^2 \left(\pi^{(t)} - \sigma_{\star}\right)^2 \left(\frac{\left(\pi^{(t)}\right)^2}{\left(\sigma_i^{(t)}\right)^2} - \frac{\left(\pi^{(t)}\right)^2}{\left(\sigma_j^{(t)}\right)^2}\right) \\
    &= \left(\left(\sigma_i^{(t)}\right)^2 - \left(\sigma_j^{(t)}\right)^2 \right) \left( 1 - \eta^2 (\pi^{(t)} - \sigma_{\star})^2 \frac{\left(\pi^{(t)}\right)^2}{\left(\sigma_i^{(t)}\right)^2 \left(\sigma_j^{(t)}\right)^2} \right) \\
    &= b_{i,j}^{(t)} \left( 1 - \eta^2 (\pi^{(t)} - \sigma_{\star})^2 \frac{\left(\pi^{(t)}\right)^2}{\left(\sigma_i^{(t)}\right)^2 \left(\sigma_j^{(t)}\right)^2} \right).
\end{align*}
Then, in order to show that $ \left|b_{i,j}^{(t+1)}\right| < c\left|b_{i,j}^{(t)}\right|$ for some $0<c \leq 1$, we need to prove that
\begin{align*}
    \left | 1 - \eta^2 (\pi^{(t)} -\sigma_{\star} )^2 \frac{\left(\pi^{(t)}\right)^2}{\left(\sigma_i^{(t)}\right)^2 \left(\sigma_j^{(t)}\right)^2} \right| < c,
\end{align*}
 for all iterations $t$. Note that for our case, it is sufficient to show the result for $i=L$ and $j=\ell$ for any $\ell \neq L$.
 %Now we introduce  a definition called gradient flow solution sharpness (GFS sharpness) before we proceed.
We complete this using the following two steps:
\begin{enumerate}[label=(\roman*)]
    \item We show that for all scalars $\sigma$ in the trajectory, if $\psi(\sigma)< \frac{2\sqrt{1+c}}{\eta}$ and $\sigma > 0$, then it holds that $\sum_{i=1}^{\min\{2,L-1\}} \frac{\eta^2 (\pi(\sigma) - \sigma_{\star} )^2 \pi^2(\sigma)}{\sigma_{L-i}^2 \sigma_{L}^2} \leq 1+c$, where $\pi(\sigma)$ denotes the product given the trajectory of all $\sigma_i$. This case is analyzed when  \(\pi(\sigma) \in [0,\sigma_{\star} )\) where $0<c<1$ and when $\pi(\sigma) > \sigma_{\star}$ where $c=1$.
    \item If $\sum_{i=1}^{\min\{2,L-1\}} \frac{\eta^2 (\pi(\sigma) - \sigma_{\star} )^2 \pi^2(\sigma)}{\sigma_{L-i}^2 \sigma_{L}^2} \leq 1+c$, then iterates become more balanced, i.e,  $|b_{i,j}^{(t+1)}| <c |b_{i,j}^{(t)}|$.
\end{enumerate}

\noindent We prove (i) in Lemma \ref{GFS-1} and (ii) in Lemma \ref{GFS-2}. Both of the proofs are originally from \cite{kreisler2023gradient}, which we adapted using our notation for ease of the reader. Then, in Lemma~\ref{GFS-3}, we show that for each $\sigma_\star$, as long as the initialization scale satisfies
\begin{align*}
    \alpha < \left( \ln\left( \frac{2\sqrt{2}}{\eta L \sigma_{\star}^{2 - \frac{2}{L}}} \right) \cdot \frac{ \sigma_{\star}^{\frac{4}{L}}}{L^2 \cdot 2^{\frac{2L-3}{L}}} \right)^{\frac{1}{4}} ,
\end{align*}
then it holds that the GFS sharpness satisfies $\psi(\sigma) < \frac{2{\sqrt{2}}}{\eta}$, which is the necessary condition for balancing. Then, to satisfy this condition for all singular values $\sigma_{\star, i}$ for all $i \in [r]$, we need
\begin{align}
\label{eqn:balance_condition}
    \alpha < \left( \ln\left( \frac{2\sqrt{2}}{\eta L \sigma_{\star, 1}^{2 - \frac{2}{L}}} \right) \cdot \frac{ \sigma_{\star, 1}^{\frac{4}{L}}}{L^2 \cdot 2^{\frac{2L-3}{L}}} \right)^{\frac{1}{4}}  \implies \eta < \frac{2\sqrt{2}}{L \sigma_{\star, 1}^{2 - \frac{2}{L}}},
\end{align}
 for the validity of the initialization scale. Thus, as long as the conditions in Equation~(\ref{eqn:balance_condition}) hold, we will have balancing. This completes the proof. 
\end{proof}



\begin{manuallemmainner}
[Hessian Eigenvalues at Balanced Minimum]
     Consider running GD on the deep matrix factorization loss $f(\mbf{\Theta})$ defined in Equation~(\ref{eqn:deep_mf}). The set of all non-zero eigenvalues of the training loss Hessian at the balanced minimum is given by
    \begin{align*}
       \lambda_{\mbf{\Theta}} = \underbrace{\left\{L \sigma_{\star, i}^{2 - \frac{2}{L}}, \sigma_{\star, i}^{2 - \frac{2}{L}}\right\}_{i=1}^r }_{\text{self-interaction}} \, \bigcup \, \underbrace{\left\{\sum_{\ell=0}^{L-1} \left(\sigma_{\star, i}^{1-\frac{1}{L} - \frac{1}{L}\ell} \cdot \sigma_{\star, j}^{\frac{1}{L}\ell}\right)^2\right\}_{i\neq j}^{r}}_{\text{interaction with other singular values}} \,\bigcup \, \underbrace{\left\{\sum_{\ell=0}^{L-1} \left(\sigma_{\star, k}^{1-\frac{1}{L} - \frac{1}{L}\ell} \cdot \alpha^{\ell}\right)^2\right\}_{k = 1}^{r}}_{\text{interaction with initialization}} 
    \end{align*}
    where $\sigma_{\star, i}$ is the $i$-th singular value of the target matrix $\mbf{M}_\star \in \mbb{R}^{d\times d}$,  $\alpha \in \mbb{R}$ is the initialization scale, $L$ is the depth of the network, and the second element of the set under ``self-interaction'' has a multiplicity of $d-r$.
\end{manuallemmainner}

\begin{proof}
By Proposition~\ref{prop:one_zero_svs_set}, notice that we can re-write the loss in Equation~(\ref{eqn:deep_mf}) as 
    \begin{align*}
        \frac{1}{2} \left\|\mbf{W}_{L:1} - \mbf{M}_\star\right\|^2_{\mathsf{F}} = \frac{1}{2} \|\mbf{\Sigma}_{L:1} - \mbf{\Sigma}_\star\|^2_{\mathsf{F}},
    \end{align*}
    where $\mbf{\Sigma}_{L:1}$ are the singular values of $\mbf{W}_{L:1}$. We will first show that the eigenvalues of the Hessian with respect to the weight matrices $\mbf{W}_\ell$ are equivalent to those of the Hessian taken with respect to its singular values $\mbf{\Sigma}_\ell$.
    To this end, consider the vectorized form of the loss:
    \begin{align*}
        f(\mbf{\Theta}) \coloneqq \frac{1}{2}\|\mbf{W}_{L:1} - \mbf{M}_\star\|^2_{\mathsf{F}} = \frac{1}{2}\|  \text{vec}(\mbf{W}_{L:1}) - \text{vec}(\mbf{M}_\star)\|^2_2.
    \end{align*}
    Then, each block of the Hessian $ \nabla_{\mbf{\Theta}}^2 f(\mbf{\Theta}) \in \mbb{R}^{d^2 L \times d^2 L}$ with respect to the vectorized parameters is given as
    \begin{align*}
    \left[\nabla_{\mbf{\Theta}}^2 f(\mbf{\Theta})\right]_{m, \ell} = \nabla_{\text{vec}(\mbf{W}_{m})} \nabla^\top_{\text{vec}(\mbf{W}_{\ell})} f(\mbf{\Theta}) \in \mbb{R}^{d^2 \times d^2}.
    \end{align*}
    %Here, notice that 
%Note that each of the Hessian wrt product combinatinos $\nabla_{\text{vec}(\mbf{W_{l}})} \nabla_{\text{vec}(\mbf{W}_{m})^\top} f(\mbf{\Theta})  \in \mathbf{R}^{n^2 \times n^2} $ which makes  $  \nabla_{\mbf{\Theta}}^2 f(\mbf{\Theta}) \in \mathbf{R}^{n^2 L \times n^2 L}$.
By the vectorization trick, each vectorized layer matrix has an SVD of the form $\text{vec}(\mbf{W}_{\ell}) = \text{vec} (\mbf{U}_{\ell} \mbf{\Sigma}_{\ell} \mbf{ V}^\top_{\ell}) = (\mbf{V}_{\ell} \otimes \mbf{U}_{\ell}) \cdot \text{vec}(\mbf{\Sigma}_{\ell})$.
Then, notice that we have
\begin{align*}
    \nabla_{\text{vec}(\mbf{W}_{\ell})} f(\mbf{\Theta}(t)) = (\mbf{ V}_{\ell} \otimes \mbf{U}_{\ell})  \cdot \nabla_{\text{vec}(\mbf{ \Sigma}_{\ell})}f(\mbf{\Theta}(t)),
\end{align*}
which gives us that 
each block of the Hessian is given by  
%Similarly, calculating the $ml$ block product matrix of the Hessian, we have:
\begin{align*}
    \left[\nabla_{\mbf{\Theta}}^2 f(\mbf{\Theta})\right]_{m, \ell} &= \nabla_{\text{vec}(\mbf{W}_{m})} \nabla^\top_{\text{vec}(\mbf{W}_{\ell})} f(\mbf{\Theta})\\
  &=  (\mbf{V}_{m} \otimes \mbf{U}_{m})\cdot \underbrace{\nabla_{\text{vec}(\mbf{\Sigma}_{m})}   \nabla^\top_{\text{vec}(\mbf{\Sigma}_{\ell})} f(\mbf{\Theta})}_{\eqqcolon \mbf{H}_{m, \ell}}\cdot (\mbf{V}_{\ell} \otimes \mbf{U}_\ell)^\top.
\end{align*}
Then, since the Kronecker product of two orthogonal matrices is also an orthogonal matrix by Lemma~\ref{lemma:kronecker_ortho}, we can write the overall Hessian matrix as  
    \begin{align*}
        \widetilde{\mbf{H}} =
        \begin{bmatrix}
            \mbf{R}_1\mbf{H}_{1, 1}\mbf{R}_1 & \mbf{R}_1\mbf{H}_{1, 2}\mbf{R}_2 & \ldots & \mbf{R}_1\mbf{H}_{1, L}\mbf{R}_L \\
            \mbf{R}_2\mbf{H}_{2, 1}\mbf{R}_1& \mbf{R}_2 \mbf{H}_{2, 2}\mbf{R}_2 & \ldots & \mbf{R}_2\mbf{H}_{2, L} \mbf{R}_L\\
            \vdots & \vdots & \ddots & \vdots \\
             \mbf{R}_L\mbf{H}_{L, 1}\mbf{R}_1 & \mbf{R}_L\mbf{H}_{L, 2}\mbf{R}_2 & \ldots & \mbf{R}_L\mbf{H}_{L, L}\mbf{R}_L
        \end{bmatrix},
    \end{align*}
 for orthogonal matrices $\{\mbf{R}_\ell\}_{\ell=1}^L$. Then, by Lemma~\ref{lem:relationship_lemma}, the eigenvalues of $\widetilde{\mbf{H}}$ are the same as those of $\mbf{H}$, where $\mbf{H} \in \mbb{R}^{d^2 L \times d^2 L}$ is the Hessian matrix with respect to the vectorized $\mbf{\Sigma}_\ell$:
\begin{align*}
    \mbf{H} = \begin{bmatrix}
            \mbf{H}_{1,1} & \mbf{H}_{1, 2} & \hdots &\mbf{H}_{L, 1}\\
            \mbf{H}_{2,1} & \mbf{H}_{2,2} & \hdots & \mbf{H}_{L, 2} \\
            \vdots & \vdots & \ddots & \vdots \\
            \mbf{H}_{1, L} & \mbf{H}_{2, L} & \hdots &\mbf{H}_{L, L}
        \end{bmatrix}.
\end{align*}
   Now, we can consider the following vectorized loss:
    \begin{align*}
        f(\mbf{\Theta}) = \frac{1}{2} \|\mbf{\Sigma}_{L:1} - \mbf{\Sigma}_\star\|_\mathsf{F}^2 &= \frac{1}{2} \left\|\mathrm{vec}\left(\mbf{\Sigma}_{L:1} - \mbf{\Sigma}_\star\right)\right\|_2^2 \\&= \frac{1}{2} \| \underbrace{\left(\mbf{\Sigma}^\top_{\ell-1:1} \otimes \mbf{\Sigma}_{L:\ell+1} \right)}_{\eqqcolon \mbf{A}_{\ell}}\cdot\mathrm{vec}(\mbf{\Sigma}_{\ell}) - \mathrm{vec}(\mbf{\Sigma}_\star) \|_2^2. 
    \end{align*}
    Then, the gradient with respect to $\mathrm{vec}(\mbf{\Sigma}_{\ell})$ is given by
    \begin{align*}
        \nabla_{\mathrm{vec}(\mbf{\Sigma}_{\ell})} f(\mbf{\Theta}) = \mbf{A}_{\ell}^\top \left( \mbf{A}_{\ell}\cdot \mathrm{vec}(\mbf{\Sigma}_{\ell}) - \mathrm{vec}(\mbf{\Sigma}_\star)\right).
    \end{align*}
   
    Then, for $m=\ell$, we have
    \begin{align*}
        \mbf{H}_{\ell, \ell} = \nabla^2_{\mathrm{vec}(\mbf{\Sigma}_{\ell})} f(\mbf{\Theta}) &= \mbf{A}_{\ell}^{\top}\mbf{A}_{\ell}. 
    \end{align*}
For $m\neq \ell$, we have
\begin{align*}
   & \mbf{H}_{m, \ell} = \nabla_{\mathrm{vec}(\mbf{\Sigma}_{m})}  \nabla_{\mathrm{vec}(\mbf{\Sigma}_{\ell})} f(\mbf{\Theta}) =  \nabla_{\mathrm{vec}(\mbf{\Sigma}_{m})} \left[\mbf{A}_{\ell}^\top (\mbf{A}_{\ell} \mathrm{vec}(\mbf{\Sigma}_{\ell}) - \mathrm{vec}(\mbf{M}^{\star})) \right] \\
   & = \nabla_{\mathrm{vec}(\mbf{\Sigma}_{m})} \mbf{A}_{\ell}^\top \cdot \underbrace{(\mbf{A}_\ell \mathrm{vec}(\mbf{\Sigma}_{\ell}) - \mathrm{vec}(\mbf{M}^{\star}))}_{=0 \text{ 
 at convergence}} + \mbf{A}_{\ell}^{\top} \cdot  \nabla_{\mathrm{vec}(\mbf{\Sigma}_{m})} (\mbf{A}_{\ell} \mathrm{vec}(\mbf{\Sigma}_{\ell}) - \mathrm{vec}(\mbf{M}^{\star})) \\
   & = \mbf{A}_{\ell}^\top \mbf{A}_{m},
\end{align*}
where we have used the product rule along with the fact that $\mbf{A}_{\ell} \mathrm{vec}(\mbf{\Sigma}_{\ell}) = \mbf{A}_m \mathrm{vec}(\mbf{\Sigma}_{m})$.

Overall, the Hessian at convergence for GD is given by
\begin{align*}
    \mbf{H} =
    \begin{bmatrix}
        \mbf{A}_{1}^\top \mbf{A}_{1} & \mbf{A}_{1}^\top \mbf{A}_{2} & \ldots & \mbf{A}_{1}^\top \mbf{A}_{L} \\
        \mbf{A}_{2}^\top \mbf{A}_{1} & \mbf{A}_{2}^\top \mbf{A}_{2} & \ldots & \mbf{A}_{2}^\top \mbf{A}_{L} \\
        \vdots & \vdots & \ddots & \vdots \\
        \mbf{A}_{L}^\top \mbf{A}_{1} & \mbf{A}_{L}^\top \mbf{A}_{2} & \ldots & \mbf{A}_{L}^\top \mbf{A}_{L}
    \end{bmatrix}
\end{align*}
Now, we can derive an explicit expression for each $\mbf{A}_{m, \ell}$ by considering the implicit balancing effect of GD in Proposition~\ref{prop:balancing}. Under balancing and Proposition~\ref{prop:one_zero_svs_set}, we have that at convergence,
    \begin{align*}
        \mbf{\Sigma}_{L:1} = \mbf{\Sigma}_\star \implies \mbf{\Sigma}_{\ell} = \begin{bmatrix}
            \mbf{\Sigma}^{1/L}_{\star, r} & \mbf{0} \\
            \mbf{0} & \alpha \cdot \mbf{I}_{d-r}
        \end{bmatrix}, \quad \forall \ell \in [L-1], \quad \text{and} \,\,\, \mbf{\Sigma}_L = \mbf{\Sigma}^{1/L}_{\star}.
    \end{align*}
    Thus, we have
    \begin{align*}
        \mbf{H}_{m, \ell} = \begin{cases}
            \mbf{\Sigma}_{\ell}^{2(\ell -1)} \otimes \mbf{\Sigma}_{\star}^{\frac{2(L-\ell)}{L}} \quad& \text{for } \,m=\ell, \\
            \mbf{\Sigma}_\ell^{m+\ell - 2} \otimes \mbf{\Sigma}_{\star}^{2L -m-\ell} \quad& \text{for }\, m\neq\ell. \\
        \end{cases}
    \end{align*}
        Now, we are left with computing the eigenvalues of $\mbf{H} \in \mbb{R}^{d^2 L \times d^2 L}$. To do this, let us block diagonalize $\mbf{H}$ into $\mbf{H} = \mbf{PCP}^\top$, where $\mbf{P}$ is a permutation matrix and 
    \begin{align*}
        \mbf{C} = 
        \begin{bmatrix}
            \mbf{C}_{1} & & \\
            & \ddots & \\
            &&\mbf{C}_{d^2}
        \end{bmatrix} \in \mbb{R}^{d^2 L \times d^2 L},
    \end{align*}
    where each $(i,j)$-th entry of $\mbf{C}_k \in \mbb{R}^{L \times L}$ is the $k$-th diagonal element of $\mbf{H}_{i, j}$. Since $\mbf{C}$ and $\mbf{H}$ are similar matrices, they have the same eigenvalues.
    Then, since $\mbf{C}$ is a block diagonal matrix, its eigenvalues (and hence the eigenvalues of $\mbf{H}$) are the union of each of the eigenvalues of its blocks. 

    By observing the structure of $\mbf{H}_{m, \ell}$, notice that each $\mbf{C}_k$ is a rank-$1$ matrix. Hence, when considering the top-$r$ diagonal elements of $\mbf{H}_{m, \ell}$ corresponding to each Kronecker product to construct $\mbf{C}_k$, each $\mbf{C}_k$ can be written as an outer product $\mbf{uu}^{\top}$, where $\mbf{u} \in \mbb{R}^L$ is
    \begin{align}
        \mbf{u}^{\top} = \begin{bmatrix}
            \sigma_{\star, i}^{1 - \frac{1}{L}} \sigma_{\star, j}^{0} & \sigma_{\star, i}^{1 - \frac{2}{L}} \sigma_{\star, j}^{\frac{1}{L}} & \sigma_{\star, i}^{1 - \frac{3}{L}} \sigma_{\star, j}^{\frac{2}{L}} & \ldots & \sigma_{\star, i}^{0} \sigma_{\star, j}^{1 - \frac{1}{L}} 
        \end{bmatrix}^{\top}.
    \end{align}
    Then, the non-zero eigenvalue of this rank-$1$ matrix is simply $\|\mbf{u}\|_2^2$, which simplifies to 
    \begin{align*}
        \|\mbf{u}\|_2^2 = \sum_{\ell=0}^{L-1} \left(\sigma_{\star, i}^{1-\frac{1}{L} - \frac{1}{L}\ell} \cdot \sigma_{\star, j}^{\frac{1}{L}\ell}\right)^2.
    \end{align*}
    Next, we can consider the remaining $d-r$ components of each Kronecker product of $\mbf{H}_{m, \ell}$. Notice that for $m = \ell = L$, we have
    \begin{align*}
        \mbf{H}_{L, L} = \begin{bmatrix}
            \sigma_{\star, 1}^{\frac{2(L-1)}{L}} \cdot \mbf{I}_d & & & \\
            & \ddots & & \\
            & & \sigma_{\star, r}^{\frac{2(L-1)}{L}} \cdot \mbf{I}_d  & \\
            & & & \alpha^{2(L-1)}\mbf{I}_{d-r} \otimes \mbf{I}_d
        \end{bmatrix}. 
    \end{align*}
    This amounts to a matrix $\mbf{C}_k$ with a single element  $\sigma_{\star, i}^{\frac{2(L-1)}{L}}$ and $0$ elsewhere. This gives an eigenvalue $\sigma_{\star, i}^{\frac{2(L-1)}{L}}$  for all $i \in [r]$, with multiplicity $d-r$. 

    Lastly, we can consider the diagonal components of $\mbf{H}_{m, \ell}$ that is a function of the initialization scale $\alpha$. For this case, each $\mbf{C}_k$ can be written as an outer product $\mbf{vv}^{\top}$, where 
    \begin{align}
        \mbf{v}^{\top} = \begin{bmatrix}
            \sigma_{\star, i}^{1 - \frac{1}{L}} \alpha^{0} & \sigma_{\star, i}^{1 - \frac{2}{L}} \alpha& \sigma_{\star, i}^{1 - \frac{3}{L}} \alpha^{2} & \ldots & \sigma_{\star, i}^{0} \alpha^{L-1}
        \end{bmatrix}^{\top}.
    \end{align}
    Similarly, the non-zero eigenvalue is simply $\|\mbf{v}\|_2^2$, which corresponds to
    \begin{align*}
        \|\mbf{v}\|_2^2 = \sum_{\ell=0}^{L-1} \left(\sigma_{\star, k}^{1-\frac{1}{L} - \frac{1}{L}\ell} \cdot \alpha^{\ell}\right)^2.
    \end{align*}
    This completes the proof.
\end{proof}



\begin{manuallemmainner}
\label{GFS-1}
    If the GFS sharpness $\psi(\sigma) \leq \frac{2\sqrt{1+c}}{\eta}$ and $\sigma > 0$, then  $\sum_{i=1}^{\min\{2,L-1\}} \frac{\eta^2 (\pi(\sigma)-\sigma_{\star})^2 \pi^2(\sigma)}{\sigma_{[L-i]}^2 \sigma_{[D]}^2} \leq (1+c)$ for some $0<c\leq1$.
\end{manuallemmainner}

\begin{proof}

We will consider two cases: (i) $\pi(\sigma) \in [0, \sigma_\star)$ and (ii) $\pi(\sigma) > \sigma_\star$ \footnote{We ignore the case $\pi^{(t)} =\sigma_{\star}$ when we get $b_{i,j}^{(t+1)} = b_{i,j}^{(t)}$. Since the occurence $\pi^{(t)} =\sigma_{\star}$ holds with a probability of zero. } .\\

\noindent \textbf{Case 1:} Let \(\sigma \in \mathbb{R}^D\) and consider the case where \(\pi(\sigma) \in [0,\sigma_{\star} )\). Then, we have
\[
\sum_{i=1}^{\min\{2,L-1\}} \frac{\eta^2 (\pi(\sigma) - \sigma_{\star} )^2 \pi^2(\sigma)}{\sigma_{L-i}^2 \sigma_{L}^2 } 
\leq \frac{\eta^2 \pi^2(\sigma)}{\sigma_{L-i}^2 \sigma_{L}^2}.
\]
Our goal is to show that if \(\psi(\sigma) \leq \frac{2\sqrt{1+c}}{\eta}\) for some $0<c<1$ then, 
\[
\sum_{i=1}^{\min\{2,L-1\}} \frac{\eta^2 (\pi(\sigma) - 1)^2 \pi^2(\sigma)}{\sigma_{L-i}^2 \sigma_{L}^2}  \leq \frac{\eta^2 \pi^2(\sigma)}{\sigma_{L-i}^2 \sigma_{L}^2}\leq 1+c.
\]

Since the GFS sharpness is constant for all the weights on the gradient flow (GF) trajectory by definition, we can focus on the singular values (or weights) at the global minima.
Consider $z = \mathrm{GF}(\sigma)$, the GF solution of $\sigma$. In Lemma \ref{gf-unbalanced}, we proved that GF preserves unbalancedness, such that $\sigma^2_{l} - \sigma^2_{m} = z^2_{l} - z^2_{m}$ for all layers. Hence, it is sufficient to show that $\sum_{i=1}^{\min\{2,L-1\}} \frac{\eta^2 \pi(z)^2}{z_{L-i}^2 z_{L}^2} \leq 1+c$ in order to ensure $\sum_{i=1}^{\min\{2,L-1\}} \frac{\eta^2 \pi^2(\sigma)}{\sigma_{L-i}^2 \sigma_{L}^2} \leq 1+c$. Note that $\pi(z)=\sigma_{\star}$, since it lies on the global minima. Then,
\begin{align}
    \sum_{i=1}^{\min\{2,L-1\}} \frac{\eta^2 \pi^2(z)}{z^{2}_{L-i} z^2_{L}} 
= \sum_{i=1}^{\min\{2,L-1\}} \frac{\eta^2 \sigma^2_{\star}}{z^{2}_{L-i} z^2_{L}}.
\end{align}
From Lemma~\ref{1d-sharp}, we know that the sharpness at the global minima is given as
\begin{align}
\label{eqn:helper1}
\psi(\sigma)=\left\| \nabla^2 L(z) \right\| = \sum_{i=1}^{L} \frac{ \sigma^2_{\star}}{z_i^2}.
\end{align}
This immediately implies that \(\frac{\sigma^2_{\star}}{z^2_{L}} \leq \psi(\sigma)\) and equivalently, \(\exists \alpha \in [0,1]\) such that $\frac{\sigma^2_{\star}}{z^2_{L}} = \alpha \psi(\sigma)$.
Therefore, we have
\begin{align}
\label{eqn:helper2}
    \sum_{i=1}^{\min\{2,L-1\}} \frac{\sigma^2_{\star}}{z^2_{L-i}} \leq (1 - \alpha) \psi(\sigma).
\end{align}
Substituting Equations~(\ref{eqn:helper1}) and~(\ref{eqn:helper2}) into the expression we aim to bound, we obtain

\[
\sum_{i=1}^{\min\{2,L-1\}} \frac{\eta^2 (\pi(\sigma) - \sigma^2_{\star})^2 \pi^2(\sigma)}{\sigma_{L-i}^2 \sigma_{L}^2}
= \sum_{i=1}^{\min\{2,L-1\}} \frac{\eta^2 \sigma^2_{\star}}{z^{2}_{L-i} z^2_{L}} 
\leq \eta^2 \alpha (1 - \alpha) \psi^2(\sigma) \leq \frac{\eta^2}{4} \psi^2(\sigma) \leq 1+c,
\]
where we used the fact that the maximum of $\alpha(1-\alpha) $ is $\frac{1}{4}$ when \(\alpha = \frac{1}{2}\) and \(\psi(\sigma) \leq \frac{2\sqrt{1+c}}{\eta}\).
Thus, if \(\psi(\sigma) \leq \frac{2\sqrt{1+c}}{\eta}\), then for every weight $\sigma$ lying on its GF trajectory, we have
\begin{align*}
    \sum_{i=1}^{\min\{2,L-1\}} \frac{\eta^2 (\pi(\sigma) - \sigma_{\star})^2 \pi^2(\sigma)}{\sigma_{L-i}^2 \sigma_{L}^2} \leq 1+c.
\end{align*}


\noindent \textbf{Case 2:} Consider the case in which $\pi(\sigma) > \sigma_{\star}$. We already have that $\sigma>0$ throughout the trajectory (refer to Lemma 3.11 in \cite{kreisler2023gradient}) and so  $\pi(\sigma)>0$. So, the GD update from $\sigma_{i}$ will also stay positive
\begin{align*}
    \sigma_{i}-\eta (\pi(\sigma) - \sigma_{\star})\pi(\sigma) \frac{1}{\sigma_{i}} >0.
\end{align*}
From this, we get 
\begin{align*}
  2 >  \frac{\eta (\pi(\sigma) - \sigma_{\star})\pi(\sigma)}{\sigma^2_{i}}>0,
\end{align*}
This implies $\sum_{i=1}^{\min\{2,L-1\}} \frac{\eta^2 (\pi(\sigma) - \sigma_{\star})^2 \pi^2(\sigma)}{\sigma_{L-i}^2 \sigma_{L}^2} \leq (1+c)$ with $c=1$. This completes the proof.
\end{proof}




\begin{manuallemmainner}
\label{GFS-2}
    If $\sum_{i=1}^{\min\{2,L-1\}} \frac{\eta^2 (\pi(\sigma) - \sigma_{\star})^2 \pi^2(\sigma)}{\sigma_{L-i}^2 \sigma_{L}^2} \leq 1+c$ for $i,j \in [L]$ for some $0<c\leq1$, then $ \left|b_{i,j}^{(t+1)}\right| < c \left|b_{i,j}^{(t)}\right|$.
\end{manuallemmainner}

\begin{proof}

Recall that the condition for balancing was given by
\begin{align}
\label{balance}
 b_{i,j}^{(t+1)}  = b_{i,j}^{(t)} \left( 1 - \eta^2 (\pi^{(t)} - \sigma_{\star})^2 \frac{\pi^{(t)2}}{\left(\sigma_i^{(t)}\right)^2 \left(\sigma_j^{(t)}\right)^2} \right).
\end{align}
WLOG, suppose that the $\sigma$ are sorted such that $\sigma_1 \geq \sigma_2 \geq \ldots \geq \sigma_L$. We know that  $$\sum_{i=1}^{\min\{2,L-1\}} \frac{\eta^2 (\pi(\sigma) - \sigma_{\star})^2 \pi^2(\sigma)}{\sigma_{L-i}^2 \sigma_{L}^2} \leq 1+c,$$ 
which implies 
\begin{align}
        \frac{\eta^2 (\pi(\sigma) - \sigma_{\star})^2 \pi^2(\sigma)}{\sigma_{L-1}^2 \sigma_{L}^2} < 1+c \quad \text{and} \quad 
        \frac{\eta^2 (\pi(\sigma) - \sigma_{\star})^2 \pi^2(\sigma)}{\sigma_{i}^2 \sigma_{j}^2} < \frac{1+c}{2},
\end{align}
for all $i \in [L]$, $j \in [L-2] $ and $ i < j$. Notice that the latter inequality comes from the fact that 
\begin{align*}
    \frac{\eta^2 (\pi(\sigma) - \sigma_{\star})^2 \pi^2(\sigma)}{\sigma_{L-2}^2 \sigma_{L}^2} + \frac{\eta^2 (\pi(\sigma) - \sigma_{\star})^2 \pi^2(\sigma)}{\sigma_{L-2}^2 \sigma_{L}^2} &< \frac{\eta^2 (\pi(\sigma) - \sigma_{\star})^2 \pi^2(\sigma)}{\sigma_{L-1}^2 \sigma_{L}^2} + \frac{\eta^2 (\pi(\sigma) - \sigma_{\star})^2 \pi^2(\sigma)}{\sigma_{L-2}^2 \sigma_{L}^2} \\
    &< 1+c,
\end{align*}
which implies that
\begin{align*}
    2\frac{\eta^2 (\pi(\sigma) - \sigma_{\star})^2 \pi^2(\sigma)}{\sigma_{L-2}^2 \sigma_{L}^2} < 1+c \implies \frac{\eta^2 (\pi(\sigma) - \sigma_{\star})^2 \pi^2(\sigma)}{\sigma_{L-2}^2 \sigma_{L}^2} < \frac{1+c}{2},
\end{align*}
and since $\sigma$ are sorted, it holds for all other $\sigma$.
Therefore from Equation~(\ref{balance}), we have for all $i \in [L-2]$,
\begin{align}
    b^{(t+1)}_{i,i+1} < c b^{(t)}_{i,i+1} \quad \text{and}\quad b^{(t+1)}_{L-2,L} < c b^{(t)}_{L-2,L}
    \quad \text{and} \quad -c b^{(t)}_{L-1,L}  <b^{(t+1)}_{L-1,L} < c b^{(t)}_{L-1,L} .
\end{align}
%Now, we prove balancing considering two cases where $b^{(t+1)}_{L-1,L} \geq 0 $ and $b^{(t+1)}_{L-1,L} \leq 0 $. 
%First, consider the case $b^{(t+1)}_{L-1,L} \geq 0 $ then using the fact for all $i \in [L-2]$,
%$b^{(t+1)}_{i,i+1} <  b^{(t)}_{i,i+1}$, $b^{(t+1)}_{i,i+1} <  b^{(t)}_{i,i+1}$.
Then, notice that since we initialized all of the singular values $\sigma_\ell$ for $\ell \in [L-1]$ to be the same, they follow the same dynamics. Since we already showed that $|b^{(t+1)}_{L-1,L}| < c |b^{(t)}_{L-1,L}|$, it must follow that
\begin{align*}
    \left|b_{i,j}^{(t+1)}\right| < c \left|b_{i,j}^{(t)}\right| \quad \text{for } \, i,j \in [L].
\end{align*}
This completes the proof.

%Hence we prove balancing for all $i,j \in [L]$, we have $ b_{i,j}^{(t+1)} \leq b_{i,j}^{(t)}$. 


%Now considering the case $b^{(t+1)}_{L-1,L} \leq 0 $, we will only obtain till $i \in [L-3]$, that $b^{(t+1)}_{i,i+1} <  b^{(t)}_{i,i+1}$ and $b^{(t+1)}_{L-2,L} <  b^{(t)}_{L-2,L} $
%Now considering the case $b^{(t+1)}_{L-1,L} \leq 0 $, we will only obtain till $i \in [L-3]$, that $b^{(t+1)}_{i,i+1} <  b^{(t)}_{i,i+1}$ and $b^{(t+1)}_{L-1,L} <  b^{(t)}_{L-1,L} $. This completes the proof. 
\end{proof}




\begin{manuallemmainner}
\label{GFS-3}
    Consider running GD with learning rate $\eta$ in Equation~(\ref{eqn:gd}) on the scalar loss 
    \begin{align*} 
        \mathcal{L}(\{\sigma_i\}_{i=1}^d)
 = \frac{1}{2} \left( \prod_{i=1}^L \sigma_{i} - \sigma_{\star} \right)^2,
    \end{align*} 
    with initialization
    $\sigma_{L}(0) = 0$ and $\sigma_{\ell}(0) = \alpha$ for all $\ell \in [L-1]$.
    If $\alpha < \left( \ln\left( \frac{2\sqrt{2}}{\eta L \sigma_{\star}^{2 - \frac{2}{L}}} \right) \cdot \frac{ \sigma_{\star}^{\frac{4}{L}}}{L^2 \cdot 2^{\frac{2L-3}{L}}} \right)^{\frac{1}{4}}$, then
    the GFS sharpness $\psi(\sigma) \leq \frac{2\sqrt{1+c}}{\eta}$ for some $0<c<1$.
\end{manuallemmainner} 


\begin{proof}
    %We prove that the initialization set $\sigma_{L}(0) = 0$ and $\sigma_{\ell}(0) = \alpha$ for all $\ell \in [L-1]$ has a GFS sharpness $\psi(\sigma) \leq \frac{2\sqrt{2}}{\eta}$ if $\alpha \leq \log(\frac{2\sqrt{2}}{\eta}) $. This means that starting from this initialization the solution that GF finds will have sharpness less than $\frac{2\sqrt{2}}{\eta}$. For this initialization set, gradient descent with step-size $\eta$ will always balance in the next iterate. 

    %Note that at initialization $(L-1)$ iterates are equal. So, throughout the GD trajectory they are always equal, i.e, $\sigma_{L-1}(t) = \sigma_{L-2}(t)= \ldots= \sigma_{1}(t) \eqqcolon y$ for all t. Further by lemma \ref{balance}, $\sigma^{2}_{L}(t)-\sigma^{2}_{l}(t)=-\alpha^2$ for all $t$. 
    Since the singular values $\sigma_\ell$ for all $\ell \in [L-1]$ are initialized to $\alpha$, note that they all follow the same dynamics. Then, let us define 
    \begin{align*}
        y \coloneqq \sigma_1 = \ldots = \sigma_{L-1} \quad \text{and} \quad x \coloneqq \sigma_L.
    \end{align*}
    The gradient flow (GF) solution is the intersection between
    \begin{align*}
       xy^{L-1}=\sigma_{\star} \quad \text{and} \quad x^{2} - y^{2}= -\alpha^2,
    \end{align*}
    where the first condition comes from convergence and the second comes from the conservation flow law of GF which we prove in Lemma \ref{gf-unbalanced}.  
    Then, if we can find a solution at the intersection such that
    \begin{align}
    \label{constraint-set}
        (\hat{x}(\alpha),\hat{y}(\alpha)) = \begin{cases}
            xy^{L-1}=\sigma_{\star} \\
            x^{2} - y^{2}= -\alpha^2,
        \end{cases} 
    \end{align}
    solely in terms of $\alpha$, then we can plug in $(\hat{x}(\alpha),\hat{y}(\alpha))$ into the GFS\footnote{Note that throughout the proof $(\hat{x}(\alpha),\hat{y}(\alpha))$ denotes the gradient flow solution as function of $\alpha$. It does
not refer to the GF trajectory.} from Lemma \ref{1d-sharp}
    \begin{align*}
        \psi(\hat{x}(\alpha),\hat{y}(\alpha)) 
 = \psi(\sigma) = \sum_{i=1}^{L} \frac{\sigma^2_{\star}}{\sigma^2_{i}} = \sigma^2_{\star}\left(\frac{1}{\hat{x}(\alpha)^2} + \frac{L-1}{\hat{y}(\alpha)^2}\right) < \frac{2\sqrt{2}}{\eta}
    \end{align*}
and solve to find an upper bound on $\alpha$. The strict inequality ensures that we can find a $c$ in $c \in [0,1)$ such that $ \psi(\alpha) <\frac{2\sqrt{1+c}}{\eta} $. However, the intersection $(\hat{x}(\alpha),\hat{y}(\alpha))$ is a $2L$-th order polynomial in $\hat{y}(\alpha)$ which does not have a straightforward closed-form solution solely in terms of $\alpha$. Hence, we aim to find the upper bound on $\alpha$ by using a calculus of variations. By plugging in $x$, the solution $\hat{y}(\alpha)$ satisfies
\begin{align*}
    y^{2L} - \alpha^2 y^{2L-2} =  \sigma^2_{\star}.
\end{align*}
Then, by differentiating the relation with respect to $\alpha$, we obtain the following variational relation:
\begin{align}
   & 2L y^{2L-1}dy - \alpha^2 2 (L-1) y^{2L-3}dy - 2\alpha y^{2L-2} d\alpha = 0 \notag  \\ 
   & \implies y^{2L-3} (y^2 L - \alpha^2 (L-1)) dy = \alpha y^{2(L-1)} d\alpha \notag \\ \
   & \implies dy = \frac{y \alpha}{ (y^2 L -\alpha^2 (L-1))} d\alpha,
\end{align}
where we used the fact that $y^{2L-2} > 0 $ from Lemma~\ref{GFS-1} in the last line. Then, in order to have $\frac{dy}{d \alpha}>0$, we need $y > \sqrt{\frac{L-1}{L}} \alpha$, which is always true since $y > \alpha$ from initialization. Then, since $\alpha \to 0$, 
$\lim_{\alpha \rightarrow 0} \hat{y}(\alpha) = \sigma^{\frac{1}{L}}_{\star}$ and $\lim_{\alpha \rightarrow 0} \hat{x}(\alpha) = \sigma^{\frac{1}{L}}_{\star}$, as it corresponds to exact balancing. Hence, $\frac{dy}{d \alpha}>0$ implies as $\alpha$ increases from $0$, $\hat{y}(\alpha)$ would increase from $\sigma^{\frac{1}{L}}_{\star}$ and $\hat{y}(\alpha)$ is an increasing function of $\alpha$.
%Note that $\lim_{\alpha \rightarrow 0} \hat{y}(\alpha) = \sigma^{\frac{1}{L}}_{\star}$ and $\lim_{\alpha \rightarrow 0} \hat{x}(\alpha) = \sigma^{\frac{1}{L}}_{\star}$ , since $\alpha \rightarrow 0$ correspond to exact balancing. 
%So, $\frac{dy}{d \alpha}>0$ implies $y > \sqrt{\frac{L-1}{L}} \alpha$, which is always true since $y> \alpha$ as it is the intialization. So, $\frac{dy}{d \alpha}>0$, implies as $\alpha$ increases from $0$, $\hat{y}(\alpha)$ would increase from $\sigma^{\frac{1}{L}}_{\star}$. 
%So, $\hat{y}(\alpha)$ is an increasing function of $\alpha$. 
Similarly, the intersection at the global minima would satisfy the following relation for $ \hat{x}(\alpha)$:
\begin{align}
    & x^{(2+ \frac{2}{L-1})} + x^{\frac{2}{(L-1)}} \alpha^2 = \sigma^{\frac{2}{L-1}}_{\star} \notag \\ 
    & \implies \left(2+\frac{2}{L-1} \right) x^{1+ \frac{2}{L-1}}dx + \left(\frac{2}{L-1}\right)\alpha^2 x^{\frac{2}{L-1}-1} dx  + x^{\frac{2}{L-1}}(2\alpha d\alpha) = 0 \notag \\
    & \implies dx = \frac{-\alpha}{\left(\frac{L}{L-1}x + \frac{\alpha^2}{L-1}\frac{1}{x}\right)} d\alpha.
\end{align}

Note that since $x>0$, we will always have $\frac{dx}{d\alpha}<0$. Then, since $\lim_{\alpha \rightarrow 0} \hat{x}(\alpha) = \sigma^{\frac{1}{L}}_{\star}$,  $\frac{dx}{d\alpha}<0$ implies that as $\alpha$ increases, $\hat{x}(\alpha)$ would decrease from $\sigma^{\frac{1}{L}}_{\star}$.
Now, with the variational relations  $\frac{d\hat{x}}{d\alpha}$ and  $\frac{d \hat{y}}{d\alpha}$ in place, we aim to find $\frac{d \psi}{d \alpha}$:
\begin{align*}
   &  \Psi(\alpha) \coloneqq  \psi(\hat{x}(\alpha),\hat{y}(\alpha)) =  \sigma_{\star}^2 \left(\frac{1}{\hat{x}(\alpha)^2} + \frac{L-1}{\hat{y}(\alpha)^2} \right)  \\ 
   & \implies d \Psi = \sigma^2_{\star} \left(-\frac{2 }{\hat{x}^3} d\hat{x} - \frac{2 (L-1) }{\hat{y}^3}d\hat{y} \right)  \\ 
   & \implies d \Psi = \frac{1}{\hat{x}^3} \left[\frac{2 \alpha \sigma^2_{\star}}{\left(\frac{L}{L-1}\right)\hat{x} +\left(\frac{\alpha^2}{L-1}\right)\frac{1}{\hat{x}} } \right] d\alpha 
   - \left[\frac{(L-1)}{\hat{y}^3} \frac{2 \alpha \hat{y} \sigma^2_{\star}}{(\hat{y}^2L - \alpha^2 (L-1))} \right] d \alpha \\
   & \implies d \Psi = \left [\frac{1}{\hat{x}^4 + \frac{\alpha^2}{L}\hat{x}^2 } - \frac{1}{(\hat{y}^4 - \alpha^2 \hat{y}^2\frac{(L-1)}{L})} \right] 2 \frac{(L-1)\sigma^2_{\star}}{L} \alpha d \alpha \\
   & \implies d \Psi  = G(\alpha) d\alpha,
\end{align*}
where we defined $G(\alpha) \coloneqq \left [\frac{1}{\hat{x}^4 + \frac{\alpha^2}{L}\hat{x}^2 } - \frac{1}{(\hat{y}^4 - \alpha^2 \hat{y}^2\frac{(L-1)}{L})} \right] 2 \frac{(L-1)\sigma^2_{\star}}{L} \alpha$ and used the notation $\hat{x} = \hat{x}(\alpha)$ and $\hat{y} = \hat{y}(\alpha)$ for simplicity. \\

\noindent Next, we will show the three following steps:
\begin{enumerate}[label=(\roman*)]
    \item Prove that $G(\alpha) > 0$ for all $\alpha > 0$ to show that the sharpness $\Psi(\alpha)$ is an increasing function of $\alpha$.
    \item Solve the differential $d\Psi$ to find the relationship between $d\Psi$ and $\Psi(\alpha)$.
    \item Find an upper bound on a part of $\frac{d\Psi}{\Psi(\alpha)}$ found in Step 2.
\end{enumerate}
\  These series of steps comes from the fact that the intersection does not have a closed-form solution. The goal is to find a function in which we can upper bound $\frac{d\Psi}{\Psi(\alpha)}$ with a function with a closed-form solution to find a bound on $\alpha$ such that the sharpness $\psi(\alpha) < \frac{2\sqrt{2}}{\eta}$. \\

% \ag{There are a few steps to go from here. }

% \begin{enumerate}
%     \item Show that  $ G(\hat{x}(\alpha),\hat{y}(\alpha),\alpha)$ is always positive, meaning sharpness increases as $\alpha$ increases. This is true since we already proved balanced iterates have the least sharpness. 
%     \item Find an upper bound on $ G(\hat{x}(\alpha),\hat{y}(\alpha),\alpha)$ (say $H(\alpha)$), so that the PDE $d \Psi  = H(\alpha) d\alpha$ has a known closed form solution (since we know initial condition). 
%     \item By continuity, the solution of PDE $d \Psi  = H(\alpha) d\alpha$ will always be above the curve $d \Psi  = G(\hat{x}(\alpha),\hat{y}(\alpha),\alpha) d\alpha$. 
%     \item Since both are increasing function and $d \Psi  = H(\alpha) d\alpha$ is an upper bound on $d \Psi  = G(\hat{x}(\alpha),\hat{y}(\alpha),\alpha) d\alpha$, the initialization condition found by solving $d \Psi  = H(\alpha) d\alpha$ would be also true for the original PDE. 
% \end{enumerate}

\noindent \textbf{Step 1}: \underline{Prove $ G(\alpha)>0 $ to show sharpness $ \Psi(\alpha)$ is an increasing function of $\alpha$}. \\

\noindent There have been several lines of work such as those by \cite{kreisler2023gradient} and \cite{marion2024deep} which showed that GD would decrease the sharpness of the solution. The more balanced the solution (which corresponds to smaller $\alpha$), the smaller the sharpness. We prove this again here:
\begin{align*}
    G(\alpha) > 0 
    & \implies \hat{y}^4 - \alpha^2 \hat{y}^2\frac{(L-1)}{L} > \hat{x}^4 + \frac{\alpha^2}{L}\hat{x}^2 \\
    & \implies (\hat{y}^4  - \hat{x}^4) > \alpha^2 \left(\frac{1}{L}\hat{x}^2 + \hat{y}^2\frac{(L-1)}{L}\right) \\
    &  \implies \underbrace{(\hat{y}^2  - \hat{x}^2)}_{=\alpha^2}(\hat{y}^2  + \hat{x}^2) > \alpha^2 \left(\frac{1}{L}\hat{x}^2 + \hat{y}^2\frac{(L-1)}{L}\right) \\
    & \implies  \hat{x}^2 (1- \frac{1}{L}) + \hat{y}^2\frac{1}{L} >0,
\end{align*}
where the last inequality always holds since we have $L>2$. This proves that $\Psi$ is an increasing function of $\alpha$ since for  $d \Psi  = G(\alpha) d\alpha$, as it always holds that $ G(\alpha) >0$ for any $L>2$ and $\alpha > 0$. \\

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{figures/objective_vs_a_L_variation.png}
    \caption{Sharpness $\Psi(\alpha)$ as a function of initialization $\alpha$. The theoretical approximation bound $ \Psi = \Psi_{0} \exp\left( \frac{  L^2\cdot 2^{\frac{2(L-1)}{L}}}{2\sigma_{\star}^{\frac{4}{L}}} \alpha^4 \right)$ serves as proxy upper bound to this increasing function.}
    \label{fig:sharp-init}
\end{figure}


\noindent \textbf{Step 2}: \underline{Solve the differential to establish the relation between $\Psi(\alpha)$ and $\alpha$}. \\

\noindent Rewriting the expression for sharpness and establishing an equation we have
\begin{align}
    \Psi(\alpha) = \sigma_{\star}^2 \left(\frac{1}{\hat{x}(\alpha)^2} + \frac{L-1}{\hat{y}(\alpha)^2} \right) 
    & \implies  \Psi(\alpha) = \sigma_{\star}^2 \left(\frac{\hat{y}^2 + (L-1)\hat{x}^2}{\hat{x}^2\hat{y}^2} \right)\\ 
    & \implies \frac{\hat{y}^2}{L} + \left(1-\frac{1}{L} \right) \hat{x}^2 = \frac{\Psi(\alpha) \hat{x}^2 \hat{y}^2}{L \sigma_{\star}^2}. \label{mid-eq}
\end{align}
Now, we revisit the original differential between $\Psi(\alpha)$ and $\alpha$:
\begin{align}
   &  d \Psi  = \left [\frac{1}{(\hat{x}^4 + \frac{\alpha^2}{L}\hat{x}^2 )} - \frac{1}{(\hat{y}^4 - \alpha^2 \hat{y}^2\frac{(L-1)}{L})} \right] 2 \frac{(L-1)\sigma^2_{\star}}{L} \alpha d\alpha \notag \\
   & \implies d \Psi = \frac{\hat{y}^4 - \hat{x}^4 -\alpha^2 (\frac{\hat{x}^2}{L} + (1-\frac{1}{L}\hat{y}^2 )) }{(\hat{x}^4 + \frac{\alpha^2}{L}\hat{x}^2 )(\hat{y}^4 - \alpha^2 \hat{y}^2\frac{(L-1)}{L}) } 2 \left(1-\frac{1}{L} \right) \sigma^2_{\star} \alpha d \alpha \notag \\
   &  \implies   d \Psi =   \frac{\alpha^2  \left( \frac{\hat{y}^2}{L} + (1-\frac{1}{L})\hat{x}^2\right) }{(\hat{x}^4 + \frac{\alpha^2}{L}\hat{x}^2 )(\hat{y}^4 - \alpha^2 \hat{y}^2\frac{(L-1)}{L}) } 2 \left(1-\frac{1}{L}\right) \sigma^2_{\star} \alpha d \alpha    \label{mid-eq2}   
\end{align}
Using the expression for $  \frac{\hat{y}^2}{L} + (1-\frac{1}{L})\hat{x}^2$ derived in Equation~(\ref{mid-eq}) and plugging it into Equation~(\ref{mid-eq2}), we obtain
\begin{align}
    &    d \Psi = \frac{\alpha^2 \left( \frac{\Psi(\alpha) \hat{x}^2 \hat{y}^2}{L \sigma_{\star}^2} \right)}{(\hat{x}^4 + \frac{\alpha^2}{L}\hat{x}^2)(\hat{y}^4 - \alpha^2 \hat{y}^2 \frac{(L-1)}{L})} 2 \left(1-\frac{1}{L}\right) \sigma_{\star}^2 \alpha \, d \alpha \notag \\
    & \implies \frac{d \Psi }{\Psi(\alpha)} =   \frac{2}{(\hat{x}^2 + \frac{\alpha^2}{L})(\hat{y}^2 - \alpha^2\frac{(L-1)}{L})}    \left(\frac{1}{L} - \frac{1}{L^2} \right)\alpha^{3} d \alpha \notag  \\ 
    & \implies \frac{d \Psi }{\Psi(\alpha)} =   \frac{2}{(\hat{x}^2 + \frac{\alpha^2}{L} )^2 }    \left(\frac{1}{L} - \frac{1}{L^2} \right)\alpha^{3} d \alpha  \\
    & \implies \frac{d \Psi }{\Psi(\alpha)} = P(\alpha) \alpha^3 d\alpha, \\
\end{align}
where we have defined $P(\alpha) \coloneqq \frac{2}{(\hat{x}^2 + \frac{\alpha^2}{L} )^2 }    \left(\frac{1}{L} - \frac{1}{L^2} \right)$.

\noindent Solving the differential $ \frac{d \Psi }{\Psi(\alpha)} = P(\alpha) \alpha^{3}d\alpha$ in exact closed-form is difficult since $\hat{x}$ is also an function of $\alpha$. However, in Step 1, we proved that $\Psi(\alpha)$ is an increasing function of $\alpha$, and so instead of solving exactly, we can find a differential equation $ \frac{d \Psi }{\Psi(\alpha)} = F(\alpha) \alpha^{3} d\alpha$ with $F(\alpha)> P(\alpha) $ such that $F(\alpha)$ is more increasing, and use it to solve the PDE instead.
Though, note that the initialization limit on $\alpha$ that would be found after solving the surrogate PDE $ \frac{d \Psi }{\Psi(\alpha)} = F(\alpha)\alpha^{3} d\alpha$ would be smaller than the $\alpha$ if it was found using the original PDE $ \frac{d \Psi }{\Psi(\alpha)} = P(\alpha)\alpha^{3} d\alpha$. \\ 

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{figures/objective_vs_a_variation.png}
    \caption{$P(\alpha)$ for GF has a unique maxima at $\alpha = \frac{\sigma_{*}^{\frac{1}{L}}}{\left(\frac{1}{\sqrt{L(L-2)}} \left(1+\frac{1}{L(L-2)}\right)^{\frac{L-1}{2}}\right)^{\frac{1}{L}}}$ for $L>2$.}
    \label{fig:P_obj}
\end{figure}


\noindent \textbf{Step 3}: \underline{Finding an upper bound function and solving for initialization}. \\
\noindent Note that the original coefficient in $ \frac{d \Psi }{\Psi(\alpha)} = P(\alpha)\alpha^{3} d\alpha$ is of the form
\begin{align}
    P(\alpha)  = \frac{2}{(\hat{x}^2 + \frac{\alpha^2}{L})^2 }    \left(\frac{1}{L} - \frac{1}{L^2}\right) \label{ref-dif}
\end{align}
Let us consider the two corner cases for $\alpha$. We showed before that $\lim_{\alpha \rightarrow 0} \hat{x}(\alpha) = \sigma^{\frac{1}{L}}_{\star}$, so \[
\lim_{\alpha \rightarrow 0} P(\alpha) = \frac{2 \left(\frac{1}{L} - \frac{1}{L^2}\right)}{\sigma_{\star}^{\frac{4}{L}} }
\]
As $\alpha \rightarrow \infty $, we have $\lim_{\alpha \rightarrow \infty} P(\alpha) \rightarrow 0 $ since $\lim_{\alpha \rightarrow \infty} \hat{x} = 0$. Furthermore, we have 

\begin{align*}
 &   P'(\alpha) = \frac{-4}{(\hat{x}^2 + \frac{\alpha^2}{L})^3 }    \left(\frac{1}{L} - \frac{1}{L^2}\right)(2\hat{x} \frac{d \hat{x}}{d \alpha} + \frac{2 \alpha}{L} ) \\
 & = \frac{-4 \left(\frac{1}{L} - \frac{1}{L^2}\right)}{(\hat{x}^2 + \frac{\alpha^2}{L})^3 }    \left(2\hat{x} ( \frac{-\alpha}{\left(\frac{L}{L-1}\hat{x} + \frac{\alpha^2}{L-1}\frac{1}{\hat{x}}\right)}) + \frac{2 \alpha}{L} \right ) \\
 & = \frac{8 \alpha \left(\frac{1}{L} - \frac{1}{L^2}\right)}{(\hat{x}^2 + \frac{\alpha^2}{L})^3 }  \left( \frac{L-1}{L+ \frac{\alpha^2}{\hat{x}^2}} - \frac{1}{L}\right)
\end{align*}
For $L=2$, we always have $P'(\alpha)<0$. Hence, choosing $F(\alpha) = \lim_{\alpha \rightarrow 0} P(\alpha) = \frac{2 \left(\frac{1}{L} - \frac{1}{L^2}\right)}{\sigma_{\star}^{\frac{4}{L}} } $, will serve as the correct upper bound. 

Then, let us consider $L>2$. We can see that $\alpha$ at which $\hat{x}(\alpha)= \frac{\alpha}{\sqrt{L(L-2)}} $ is the critical point of $P(\alpha)$. Further, we note that when $\hat{x}(\alpha)< \frac{\alpha}{\sqrt{L(L-2)}} $, $P'(\alpha)<0 $ meaning $P(\alpha)$ is decreasing. Since $\hat{x}(\alpha)$ is itself decreasing in $\alpha$, this states there for any $\alpha>\alpha_{crit}$, $P(\alpha)$ is decreasing. $\alpha_{crit}$ is the solution of $\hat{x}(\alpha)= \frac{\alpha}{\sqrt{L(L-2)}}$. 


For any $\alpha<\alpha_{crit}$, $ P'(\alpha) > 0$, so $P(\alpha)$ is increasing. So, $P(\alpha_{crit})$ corresponds to the maximum of $P$ in $\alpha$. Choosing $F(\alpha) = P(\alpha_{crit}) $, a constant allows us to find an upper bound function for the function in Equation~(\ref{ref-dif}). Furthermore, note that since $\frac{d \hat{x}}{d \alpha} <0$ and $\hat{x}>0$, $\alpha>0$, there must be only one critical point of $P(\alpha)$ which is at $\alpha_{crit}$. 

Hence, we have $\hat{x}(\alpha_{crit}) = \frac{\alpha_{crit}}{\sqrt{L(L-2)}}$. From Equation~(\ref{constraint-set}), we also get $\hat{y} = \alpha_{crit} \sqrt{1+\frac{1}{L(L-2)}}$ and 
\begin{align*}
    & \left(\frac{\alpha_{\text{crit}}}{\sqrt{L(L-2)}}\right) \left( \alpha_{\text{crit}} \sqrt{1+\frac{1}{L(L-2)}}\right)^{L-1} = \sigma_{*} \\ 
    & \implies \alpha_{\text{crit}}  = \frac{\sigma_{*}^{\frac{1}{L}}}{\left(\frac{1}{\sqrt{L(L-2)}} \left(1+\frac{1}{L(L-2)}\right)^{\frac{L-1}{2}}\right)^{\frac{1}{L}}} \\
\end{align*}

Using $\alpha_{\text{crit}}$, we obtain the maximum of $P(\alpha)$ to be 

\begin{align*}
& P(\alpha_{crit}) =  \frac{2}{(\hat{x}(\alpha_{crit})^2 + \frac{\alpha_{crit}^2}{L})^2 }    \left(\frac{1}{L} - \frac{1}{L^2}\right) \\
& = \frac{2}{ \left(\alpha^2_{crit} (\frac{1}{L(L-2)} +\frac{1}{L}) \right)^2 }    \left(\frac{1}{L} - \frac{1}{L^2}\right)  \\
& = \frac{2}{\sigma^{\frac{4}{L}}_{*}} g(L)
\end{align*}
where $g(L)= \frac{(\frac{1}{L} - \frac{1}{L^2}) [ \frac{1}{\sqrt{L(L-2)}} \left(1+\frac{1}{L(L-2)}\right)^{\frac{L-1}{2}}]^{\frac{4}{L}}}{(\frac{1}{L(L-2)} +\frac{1}{L})^2} $.

Now, chosing $F(\alpha)= P(\alpha_{crit})$, we integrate the upper bound function as 

\begin{align*}
    & \int \frac{d \Psi}{\Psi} = \frac{2 g(L)}{\sigma_{\star}^{\frac{4}{L}}} \int \alpha^3 \, d\alpha \\
    & \implies \mathrm{ln}(\frac{\Psi}{\Psi_{0}}) = \frac{ g(L)}{2\sigma_{\star}^{\frac{4}{L}}} (\alpha^4) \\ 
    & \implies \Psi = \Psi_{0} \exp\left( \frac{ g(L)}{2\sigma_{\star}^{\frac{4}{L}}} \alpha^4 \right)\\
\end{align*}

where $\Psi_{0}= \lim_{\alpha \rightarrow 0}\Psi = L\sigma^{2-\frac{2}{L}}_{\star} $. 
We verify this upper bound empirically from Figure \ref{fig:sharp-init}, where we see a near exponential growth in sharpness as function of $\alpha$. 

Now, note that the function $\Psi = \Psi_{0} \exp\left( \frac{ g(L)}{2\sigma_{\star}^{\frac{4}{L}}} \alpha^4 \right)$ acts an upper bound to the original sharpness function of $\alpha$ and both are increasing in $\alpha$ (Step 1). So, solving for an initialization $\alpha$-upper limit with  $\Psi = \frac{2\sqrt{2}}{\eta}$ would mean that the original sharpness with this initialization would be less than $\frac{2\sqrt{1+c}}{\eta}$ for some $0<c<1$.  Hence, $\alpha$ is restricted to
\begin{align*}
    \alpha < \left( \ln\left( \frac{\frac{2\sqrt{2}}{\eta}}{L \sigma_{\star}^{2 - \frac{2}{L}}} \right) \cdot \frac{2 \sigma_{\star}^{\frac{4}{L}}}{g(L)} \right)^{\frac{1}{4}}.
\end{align*}
We can simplify the bound further by finding an upper bound on $g(L)$ \footnote{This includes the case for $L=2$ since $(\frac{1}{L}- \frac{1}{L^2}) < L^2\cdot 2^{\frac{2(L-1)}{L}}$ for $L=2$.}:
\begin{align*}
    g(L) \leq \frac{\left(\left(1 + \frac{1}{L(L-2)}\right)^{\frac{L-1}{2}}\right)^{\frac{4}{L}}}{\left(\frac{1}{L(L-2)}+\frac{1}{L}\right)^2} \leq L^2 \cdot \left(\left(1 + \frac{1}{L(L-2)}\right)^{\frac{L-1}{2}}\right)^{\frac{4}{L}} \leq L^2\cdot 2^{\frac{2(L-1)}{L}}.
\end{align*}
Then, we get obtain a lower bound on $\alpha$:
\begin{align*}
    \alpha < \left( \ln\left( \frac{2\sqrt{2}}{\eta L \sigma_{\star}^{2 - \frac{2}{L}}} \right) \cdot \frac{2 \sigma_{\star}^{\frac{4}{L}}}{L^2 \cdot 2^{\frac{2(L-1)}{L}}} \right)^{\frac{1}{4}} = \left( \ln\left( \frac{2\sqrt{2}}{\eta L \sigma_{\star}^{2 - \frac{2}{L}}} \right) \cdot \frac{ \sigma_{\star}^{\frac{4}{L}}}{L^2 \cdot 2^{\frac{2L-3}{L}}} \right)^{\frac{1}{4}} 
\end{align*}
 Hence, as long as $\alpha$ satisfies this upper bound, we will have balancing. This completes the proof.
 % And as $\alpha \rightarrow \infty$, we will have $\hat{x}(\alpha) \rightarrow 0$, since we proved that  $\hat{x}(\alpha)$ is a decreasing function of $\alpha$ but the product $\hat{x}^2(\alpha)\alpha^2$ is finite, so $\lim_{\alpha \rightarrow \infty}P(\alpha) < \infty$.  So, we chose $F(\alpha) = \sup_{0< \alpha<\infty} P(\alpha)$ and use it to solve the PDE.

% We find the critical points of $ g(\alpha) = (\hat{x}(\alpha)^2 + \frac{\alpha^2}{L} )^2$ to analyze the behavior of $P(\alpha)$. 

% \begin{align*}
%    & \frac{\partial g}{\partial \alpha} = 2 (\hat{x}^2 + \frac{\alpha^2}{L} )(2\hat{x} \frac{\partial x}{\partial \alpha} +\frac{2 \alpha }{L} )  \\
%    & = 2 (\hat{x}^2 + \frac{\alpha^2}{L} )(2\hat{x} \frac{-\alpha}{[\frac{L}{L-1}\hat{x} + \frac{\alpha^2}{L-1}\frac{1}{\hat{x}}]} +\frac{2 \alpha }{L} ) \\
%    & = -4 \alpha  (\hat{x}^2 + \frac{\alpha^2}{L} )(\frac{L-1}{L+\frac{\alpha^2}{\hat{x}^2}} -\frac{1}{L})
% \end{align*}


% The critical points of $\frac{\partial g}{\partial \alpha}$ are solved as:
% % Using the expression for $\frac{\partial \hat{x}}{\partial \alpha}$ and solving for $\hat{x}$, we obtain
% \begin{align*}
%     \hat{x}^2 = \frac{\alpha^2}{L(L-1)-L}
% \end{align*} which gives $P(\alpha)$ at critical point to be :

% \begin{align*}
%     P(\alpha) = \frac{2}{\alpha^4 (\frac{1}{L(L-1)-L} + \frac{1}{L} )^2}\left(\frac{1}{L} - \frac{1}{L^2}\right)
% \end{align*}
% We note that this expression is larger than both $\lim_{\alpha \rightarrow \infty} P(\alpha)$ and $\lim_{\alpha \rightarrow 0}  P(\alpha)$, since we have $\sigma_{\star} > \alpha^{L} (\frac{1}{L(L-1)-L} + \frac{1}{L})^2 $.

% So, we will use $F(\alpha) = \frac{2}{\alpha^4 (\frac{1}{L(L-1)-L} + \frac{1}{L} )^2}\left(\frac{1}{L} - \frac{1}{L^2}\right) $ and integrate both sides as follows:

% \begin{align*}
%   &  \int \frac{d \Psi}{\Psi(\alpha)} = \frac{2}{ \left( \frac{1}{L(L-1)-1} + \frac{1}{L} \right)^2}\left(\frac{1}{L} - \frac{1}{L^2}\right) \int  \frac{d \alpha}{\alpha}  \\
%   & 
% \end{align*}

\end{proof}

\begin{manuallemmainner}
\label{gf-unbalanced}
    Consider the minimizing the loss         \begin{align*} 
        \mathcal{L}\left(\{\sigma_\ell\}_{\ell=1}^L\right)
 = \frac{1}{2} \left( \prod_{\ell=1}^L \sigma_{\ell} - \sigma_{\star} \right)^2,
    \end{align*}  
    using gradient flow. Then, the balancedness between two singular values defined by $\sigma^2_{ \ell} (t) - \sigma^2_{m} (t)$ for all $m, \ell \in [L]$ is constant for all $t$.
\end{manuallemmainner}

\begin{proof}
Notice that the result holds specifically for gradient flow and not descent. The dynamics of each scalar factor for gradient flow can be written as
    \begin{align*}
        \dot{\sigma}_{\ell}(t) = - \left(\prod_{\ell=1}^L \sigma_{ \ell} (t) - \sigma_{\star} \right)\cdot \prod_{i\neq \ell}^L \sigma_{i}(t)
    \end{align*}
Then, the time derivative of balancing is given as
\begin{align*}
  & \frac{\partial}{\partial t} (\sigma^2_{ \ell} (t) - \sigma^2_{m} (t)) = \sigma_{ \ell} (t)\dot{\sigma}_{\ell}(t)  - \sigma_{m} (t)\dot{\sigma}_{m}(t)  \\
  & = - \sigma_{ \ell} (t)\left(\prod_{\ell=1}^L \sigma_{ \ell} (t) - \sigma_{\star} \right)\cdot \prod_{i\neq \ell}^L \sigma_{i}(t) + \sigma_{m} (t)\left(\prod_{m=1}^L \sigma_{ \ell} (t) - \sigma_{\star} \right)\cdot \prod_{j\neq m}^L \sigma_{j}(t). \\
  & = 0.
\end{align*}
Hence, the quantity $\sigma^2_{ \ell} (t) - \sigma^2_{m} (t) $ remains constant for all time $t$, hence preserving unbalancedness. 
\end{proof}

\begin{manuallemmainner}
\label{1d-sharp}
    Consider the scalar loss     \begin{align*} 
        \mathcal{L}(\{\sigma_i\}_{i=1}^d)
 = \frac{1}{2} \left( \prod_{i=1}^L \sigma_{i} - \sigma_{\star} \right)^2,
    \end{align*}
    The sharpness at the global minima is given as $\| \nabla^2 \mathcal{L} \|_{2} = \sum_{i=1}^{L} \frac{\sigma^2_{\star}}{\sigma^2_{i}}$.
\end{manuallemmainner}

\begin{proof}
The gradient is given by
\begin{align*}
    \nabla_{\sigma_{i}}  \mathcal{L} = \left(\prod_{\ell=1}^L \sigma_{ \ell} (t) - \sigma_{\star} \right) \prod_{j\neq i}^L \sigma_{j}(t).
\end{align*}
Then, 
\begin{align*}
     \nabla_{\sigma_{j}}  \nabla_{\sigma_{i}}  \mathcal{L} =  \prod_{\ell\neq i}^L \sigma_{\ell}(t)  \prod_{\ell\neq j}^L \sigma_{\ell}(t) + \left(\prod_{\ell=1}^L \sigma_{ \ell} (t) - \sigma_{\star} \right)  \prod_{\ell\neq j, \ell \neq i}^L \sigma_{\ell}(t)
\end{align*}
 Let $\pi(t)=  \prod_{i=1}^L \sigma_{i}(t)$. Then, at the global minima, we have
\begin{align*}
     \nabla_{\sigma_{j}}  \nabla_{\sigma_{i}}  \mathcal{L} =  \frac{\pi^2}{\sigma_{i} \sigma_{j}} = \frac{\sigma_{\star}^2}{\sigma_{i} \sigma_{j}}
\end{align*}
Thus, the sharpness of the largest eigenvalue is given as $ \| \nabla^2 \mathcal{L} \|_{2} = \sum_{i=1}^{L} \frac{\sigma^2_{\star}}{\sigma^2_{i}}$. 
\end{proof}

\begin{manuallemmainner}
\label{lemma:flattest}
Consider the loss \begin{align*} 
        \mathcal{L}\left(\{\sigma_i\}_{i=1}^L\right)
 = \frac{1}{2} \left( \prod_{i=1}^L \sigma_{i} - \sigma_{\star} \right)^2.
    \end{align*} 
The balanced minimum $\sigma_i = \sigma_\star^{1/L}$ has the smallest sharpness amongst all global minima with a value of $\|\nabla^2 \mathcal{L}\|_2 = L\sigma_\star^{2-2/L}$.
\end{manuallemmainner}
\begin{proof}
    By Lemma~\ref{1d-sharp}, recall that the sharpness at the global minima is given in the form
    \begin{align*}
        \|\nabla^2 \mathcal{L}\|_2 = \sum_{i=1}^L \frac{\sigma_\star^2}{\sigma_i^2}.
    \end{align*}
    To show that the balanced minimum is the flattest (i.e., it has the smallest sharpness amongst all global minima), we will show that KKT stationarity condition of the constrained objective
    \begin{align*}
        \underset{\{\sigma_i\}_{i=1}^L }{\mathrm{min}} \,  \sum_{i=1}^L \frac{\sigma_\star^2}{\sigma_i^2} \quad\,\mathrm{s.t.} \,\, \prod_{i=1}^L \sigma_i = \sigma_\star,
    \end{align*}
    are only met at the balanced minimum, 
    which gives us the sharpness value $\| \nabla^2 \mathcal{L} \|_{2} = L\sigma_\star^{2-2/L}$.
    The Lagrangian is given by
    \begin{align*}
        L(\sigma_1, \ldots, \sigma_L, \mu) = \sum_{i=1}^L \frac{\sigma_\star^2}{\sigma_i^2} + \mu\left( \prod_{i=1}^L \sigma_i - \sigma_\star \right).
    \end{align*}
Then, the stationary point conditions of the Langrangian is given by 
    \begin{align}
    \label{eqn:station1}
        \frac{\partial L}{\partial \sigma_i} &= -\frac{2\sigma_\star^2}{\sigma_i^3} + \mu \prod_{j\neq i} \sigma_j = 0, \\
    \label{eqn:station2}
    \frac{\partial L}{\partial \mu} &= \prod_{i=1}^L \sigma_i - \sigma_\star = 0.
    \end{align}
    From Equation~(\ref{eqn:station1}), the solution of the stationary point gives
    \begin{align*}
        \frac{2\sigma_\star^2}{\sigma_i^3} = \mu \prod_{j\neq i} \sigma_j \implies \mu =  \frac{2\sigma_\star^2}{\sigma_i^3 \prod_{j\neq i} \sigma_j} = \frac{2\sigma_\star^2}{\sigma_i^2 \sigma_\star} = \frac{2\sigma_\star}{\sigma_i^2}.
    \end{align*}
    This also indicates that at the stationary point, $\sigma_{i} = \sqrt{\frac{2\sigma_\star}{\mu}}$ for all $i \in [L]$, which means that the condition is \emph{only} satisfied at the balanced minimum, i.e, $\sigma_{i} = \sigma_\star^{1/L}$. Furthermore, notice that
    \begin{align*}
        \nabla^2 f(\sigma_i) = 6 \sigma_\star^2 \cdot \diag\left(\frac{1}{\sigma^4_{i}}\right) \succ \mathbf{0},
    \end{align*}
    where $f(\sigma_i) = \sum_{i=1}^L \frac{\sigma_\star^2}{\sigma_i^2}$, indicating that $f$ only has a minimum. Notice that Equation~(\ref{eqn:station2}) holds immediately. Thus, the balanced minimum has the smallest shaprness (flattest), which plugging into $f$ gives a sharpness of $\|\nabla^2 \mathcal{L}\|_2 = L\sigma_\star^{2-2/L}$. 

    
    % Then, plugging in the balanced minimum and $\mu^*$ into Equation~(\ref{eqn:station1}), we have
    % \begin{align*}
    %     -\frac{2\sigma_\star^2}{\sigma_\star^{3/L}} + \frac{2\sigma_\star}{\sigma_\star^{2/L}} \cdot \left(\sigma_\star^{1/L}\right)^{L-1} = -2\sigma_\star^{\frac{2L-3}{L}} + 2\sigma_\star^{\frac{2L-3}{L}} = 0.
    % \end{align*}
    % Notice that Equation~(\ref{eqn:station2}) holds immediately. Thus, the balanced minimum $\sigma_i = \sigma_\star^{1/L}$ satisfies both the stationary point conditions, which completes the proof.
\end{proof}








\begin{comment}

As  $\mbf{s}^\star \in \mbb{R}^{d}$ is a $r$-sparse vector, we denote the support set $I$ as the indices set where  $\mbf{s}^\star$ is non-zero. Let $I^{C}$ denote the complement set. Let us denote each diagonal vector layer $\mbf{s}_l =  \text{vec}\left( \{ s_{l,i} \}_{i=1}^{d} \right)$.  We specify vector $\mbf{q}_{i} = \text{vec}\left( \{ s_{l,i} \}_{l=1}^{L} \right)$, which is a vector containing the $i^{th}$ index for all layers $l-1,.,L$. 

With these notation, we can equivalently write the loss of diagonal linear network as $\mathcal{L}(\mbf{s}) =  \sum_{i=1}^d L(\mbf{q}_{i})  = \frac{1}{2} \sum_{i} (s_{1,i}s_{2,i}..s_{L,i} - s_{\star,i} )^2$. 

 The loss of diagonal linear networks can be decomposed in the sum of each scalar losses on each index   , where $\mathbf{s}_{l} = \text{vec}\left( \{ s_{l,i} \}_{i=1}^{d} \right)$ and $L(\mbf{q}_{i}) = (s_{1,i}s_{2,i}..s_{L,i} - s_{\star,i} )^2  $. So the Hessian of the end to end loss can be written as:

 \begin{align*}
    \nabla^2 \mathcal{L}(\mbf{s}) = \begin{bmatrix}
        \nabla^2 \mathcal{L}(\mbf{q}_{1})& & \\
        & \ddots & \\
        & & \nabla^2 \mathcal{L}(\mbf{q}_{d})
    \end{bmatrix}
 \end{align*}

where $\nabla^2 \mathcal{L}(\mbf{q}_{i})$ denote the Hessian of the loss $L(\mbf{q}_{i}) = (s_{1,i}s_{2,i}..s_{L,i} - s_{\star,i} )^2  $ and we have that $\nabla_{(\mbf{q}_{i})} \nabla_{(\mbf{q}_{j})} \mathcal{L} = \mbf{0}$ since the loss is separable. 

Due to the balancednes ( $\alpha< \log({\frac{2\sqrt{2}}{h}})$), we will have $\mbf{q}_{i} =  s^{\frac{1}{L}}_{\star,i} \mbf{1}_{L}$ if $i \in I$ and otherwise $\mbf{q}_{i} =   \text{vec}\left( \alpha, \alpha, ..,\alpha, 0  \right)$ if $i \in I^{C}$. 

With this each diagonal block of the Hessian is calculated as follows:
$ \nabla^2 \mathcal{L}(\mbf{q}_{i}) =  s^{2(1 - \frac{1}{L})}_{\star,i} \mbf{1}_{L} \mbf{1}_{L}^T $ if $ i \in I$.




If $ i\in I^{C}$,  $ \nabla^2 \mathcal{L}(\mbf{q}_{i}) = \begin{bmatrix}
            0 & \hdots & 0 & \alpha^{2(L-1)} \\
            \vdots & \ddots & \vdots & \vdots \\
            0 & \hdots & 0 & \alpha^{2(L-1)} \\
            \alpha^{2(L-1)} & \hdots & \alpha^{2(L-1)} & \alpha^{2(L-1)}
        \end{bmatrix} $.
        
The top $r$ (corresponding to the $r$-support set) eigenvectors of $\nabla^2 \mathcal{L}(\mbf{s})$ and eigenvalue pairs are then given as 

\begin{align*}
    \Delta_1 &= \mathrm{vec}\left( \frac{1}{\sqrt{L}} \mathbf{1}_{L}, \mathbf{0}, \dots, \mathbf{0} \right), \quad \lambda_{1} = L s_{\star,1}^{2 - \frac{2}{L}} \\
    \Delta_2 &= \mathrm{vec}\left( \mathbf{0}, \frac{1}{\sqrt{L}} \mathbf{1}_{L}, \dots, \mathbf{0} \right), \quad \lambda_{2} = L s_{\star,2}^{2 - \frac{2}{L}} \\
    \quad\quad\quad&\vdots \\
    \Delta_r &= \mathrm{vec}\left( \mathbf{0}, \dots, \frac{1}{\sqrt{L}} \mathbf{1}_{L}, \dots, \mathbf{0} \right), \quad \lambda_{r} = L s_{\star,r}^{2 - \frac{2}{L}} \\
\end{align*}

Followed by eigenvector-eigenvalue pair for the support set complement where $\mathbf{e}_{r+j} $ is the eigenvector of the matrix $\begin{bmatrix}
            0 & \hdots & 0 & \alpha^{2(L-1)} \\
            \vdots & \ddots & \vdots & \vdots \\
            0 & \hdots & 0 & \alpha^{2(L-1)} \\
            \alpha^{2(L-1)} & \hdots & \alpha^{2(L-1)} & \alpha^{2(L-1)}
        \end{bmatrix} $
:
\begin{align*}
    \Delta_{r+j} &= \mathrm{vec}\left( \mathbf{0}, \dots, \mathbf{e}_{r+j}, \dots, \mathbf{0} \right) , \quad \lambda_{r+j} = \frac{-\alpha^{2(L-1)} \pm \sqrt{(4L-3)\cdot \alpha^{4(L-1)^2}}}{-2}
\end{align*}


\begin{align*}
     \Delta_{r+j} = \mathrm{vec}\left( \mathbf{0}, \dots, \mbf{e}_{r+j},\dots, \mathbf{0} \right)
\end{align*}
In each 1D eigenvector direction, we can analyze the loss and verify if it satisifies the stable condition or not. 
Infact, in each eigen-vector cross-section, the 1D loss is exactly $L(\mbf{q}_{i}) =(s_{1,i}s_{2,i}..s_{L,i} - s_{\star,i} )^2  $. Due to balancing the 1D loss boils down to a multilayer scalar loss $L(x) = (x^{L} - s_{\star,i})^2$. Using Corollary-5 in \cite{chen2023edge} or restated lemma \ref{lemma:chen-bruna} on the 1D scalar function $L(x) = (x^{L} - s_{\star,i})^2$ , we prove that this 1D loss is amenable to stable oscillation when learning rate $ \eta >\frac{2}{\lambda_{i}} $. To prove the uniqueness and existence of two period orbit fixed point for $ \eta >\frac{2}{\lambda_{i}} $, we show that the polynomial obtained by solving two step fixed point has a real root. This is the same loss we analyzed in Theorem \ref{thm:stable_oscillations}, where we showed that the oscillations are real root of the polynomial

\begin{align*}
    \sigma_{\star, 1} = \rho^L\frac{1+z^{2L-1}}{1+z^{L-1}}, \quad \text{where  } \, z \coloneqq \left(1 + \eta L(\sigma_{\star, 1} - \rho^L)\cdot \rho^{L-2} \right).
\end{align*}


$\rho_1 \in \left(0, \sigma_{\star, 1}^{1/L}\right)$ and $\rho_2 \in \left(\sigma_{\star, 1}^{1/L}, (2\sigma_{\star, 1})^{1/L}\right)$ are the two real roots of the polynomial which exists and are unique.

So, whenever the learning rate $\eta$ lies between $[\frac{2}{\lambda_{i}},\frac{2}{\lambda_{i+1}}]$, we will have oscilaltions in all the eigenvector directions 
\end{proof}
\end{comment}



\begin{comment}

\section{Auxiliary Results}


\begin{customlemma}{4}\label{lem:relationship_lemma} 
    Let $\mbf{U}, \mbf{V}, [\mbf{\sigma}_{l}]_{l=2}^L \in \mathbb{R}^{n\times n}$ be $L$ orthogonal matrices and $\mbf{H}_{i, j} \in \mathbb{R}^{n^2 \times n^2}$ be diagonal matrices. Consider the two following block matrices:
    \begin{align*}
       & \widetilde{\mbf{H}} = \begin{bmatrix}
            \mbf{H}_{1,1} & \mbf{H}_{1, 2} & \hdots &\mbf{H}_{L, 1}\\
            \mbf{H}_{2,1} & \mbf{H}_{2,2} & \hdots & \mbf{H}_{L, 2} \\
            \vdots & \vdots & \ddots & \vdots \\
            \mbf{H}_{1, L} & \mbf{H}_{2, L} & \hdots &\mbf{H}_{L, L}
        \end{bmatrix} \quad\quad\quad \\
      &  \mbf{W} = \begin{bmatrix}
                 (\mbf{\sigma}_{L} \otimes \mbf{U})\mbf{H}_{1,1}(\mbf{\sigma}_{L} \otimes \mbf{U})^{\top} & (\mbf{\sigma}_{L} \otimes \mbf{U}) \mbf{H}_{1, 2}(\mbf{\sigma}_{L-1} \otimes \mbf{\sigma}_{L})^{\top} & \hdots &  (\mbf{\sigma}_{L} \otimes \mbf{U}) \mbf{H}_{1, L}  (\mbf{V}  \otimes \mbf{\sigma}_{2})^{\top}\\
            (\mbf{\sigma}_{L-1} \otimes \mbf{\sigma}_{L}) \mbf{H}_{2,1}(\mbf{\sigma}_{L} \otimes \mbf{U})^{\top} & (\mbf{\sigma}_{L-1} \otimes \mbf{\sigma}_{L}) \mbf{H}_{2,2} (\mbf{\sigma}_{L-1} \otimes \mbf{\sigma}_{L})^{\top} & \hdots & (\mbf{\sigma}_{L-1} \otimes \mbf{\sigma}_{L}) \mbf{H}_{2, L}  (\mbf{V}  \otimes \mbf{\sigma}_{2})^{\top}\\
            \vdots & \vdots & \ddots & \vdots \\
                (\mbf{V}  \otimes \mbf{\sigma}_{2}) \mbf{H}_{L, 1}(\mbf{\sigma}_{L} \otimes \mbf{U})^{\top} &   (\mbf{V}  \otimes \mbf{\sigma}_{2}) \mbf{H}_{L, 2}(\mbf{\sigma}_{L-1} \otimes \mbf{\sigma}_{L})^{\top}  & \hdots &  (\mbf{V}  \otimes \mbf{\sigma}_{2}) \mbf{H}_{L, L} (\mbf{V}  \otimes \mbf{\sigma}_{2})^{\top}
        \end{bmatrix}.
    \end{align*}
    Then, the eigenvalues of $\widetilde{\mbf{H}} \in \mbb{R}^{n^2 L \times n^2 L}$ are the same as those of $\mbf{W} \in \mbb{R}^{n^2 L \times n^2 L}$. $\mbf{W}$ is the Hessian of the deep matrix factorization loss with SVS singular vectors and $\widetilde{\mbf{H}}$ is the Hessian computed for product of diagonal matrices.
\end{customlemma}


\begin{proof}

\ag{I will change the order of L and 1 later, it does not change the proof}.
    For sake of notation, say $\mbf{R_{L}} =  (\mbf{\sigma}_{L} \otimes \mbf{U})$, $\mbf{R_{L-1}} =  (\mbf{\sigma}_{L-1} \otimes \mbf{\sigma}_{L}) $,..., $ \mbf{R_{l}} = (\mbf{\sigma}_{l} \otimes \mbf{\sigma}_{l+1})$ and $\mbf{R}_{1} = (\mbf{V}  \otimes \mbf{\sigma}_{2})$. Then for sake of notation we rewrite $\mbf{W}$ as:

\begin{align*}
    \mbf{W} = \begin{bmatrix}
        \mbf{R}_{L}\mbf{H}_{1,1}\mbf{R}_{L}^{\top} & \mbf{R}_{L}\mbf{H}_{1, 2}\mbf{R}_{L-1}^{\top} & \hdots & \mbf{R}_{L}\mbf{H}_{1, L}\mbf{R}_{1}^{\top}\\
        \mbf{R}_{L-1}\mbf{H}_{2,1}\mbf{R}_{L}^{\top} & \mbf{R}_{L-1}\mbf{H}_{2,2}\mbf{R}_{L-1}^{\top} & \hdots & \mbf{R}_{L-1}\mbf{H}_{2, L}\mbf{R}_{1}^{\top}\\
        \vdots & \vdots & \ddots & \vdots \\
        \mbf{R}_{1}\mbf{H}_{L,1}\mbf{R}_{L}^{\top} & \mbf{R}_{1}\mbf{H}_{L,2}\mbf{R}_{L-1}^{\top} & \hdots & \mbf{R}_{1}\mbf{H}_{L,L}\mbf{R}_{1}^{\top}
    \end{bmatrix}.
\end{align*}

In lemma, we show that $\mbf{R}_{l}$ is an orthogonal matrix. With this, it suffices to show that $\mbf{W}$ and $ \widetilde{\mbf{H}}$ have the same characteristic polynomial. Let us define 

Let us define
    \begin{align*}
        \mbf{W} \coloneqq \begin{bmatrix}
            \mbf{A} & \mbf{B} \\
            \mbf{C} & \mbf{D}
        \end{bmatrix},
    \end{align*}
    where 
    \begin{alignat}{3}
        &\mbf{A} \coloneqq  \mbf{R}_{L}\mbf{H}_{1,1}\mbf{R}_{L}^{\top} \quad\quad\quad &\mbf{B} &\coloneqq \begin{bmatrix}
            \mbf{R}_{L}\mbf{H}_{1, 2}\mbf{R}_{L-1}^{\top} & \hdots & \mbf{R}_{L}\mbf{H}_{1, L}\mbf{R}_{1}^{\top}
        \end{bmatrix} \\
        &\mbf{C} \coloneqq \begin{bmatrix}
            \mbf{R}_{L-1}\mbf{H}_{2,1}\mbf{R}_{L}^{\top} \\
            \vdots \\
           \mbf{R}_{1}\mbf{H}_{L,1}\mbf{R}_{L}^{\top}
        \end{bmatrix}  \quad\quad\quad
        &\mbf{D} &\coloneqq \begin{bmatrix}
           \mbf{R}_{L-1}\mbf{H}_{2,2}\mbf{R}_{L-1}^{\top} & \hdots & \mbf{R}_{L-1}\mbf{H}_{2, L}\mbf{R}_{1}^{\top}\\ \\
            \vdots & \ddots & \vdots \\
           \mbf{R}_{1}\mbf{H}_{L,2}\mbf{R}_{L-1}^{\top} & \hdots & \mbf{R}_{1}\mbf{H}_{L,L}\mbf{R}_{1}^{\top}
        \end{bmatrix}.
    \end{alignat}
    Then, we have
    \begin{align*}
        \det(\mbf{W} - \lambda \mbf{I}) &= \det\left(\begin{bmatrix}
            \mbf{A} - \lambda\mbf{I} & \mbf{B} \\
            \mbf{C} & \mbf{D} - \lambda\mbf{I}
        \end{bmatrix}\right) \\
        &= \det(\mbf{A} - \lambda \mbf{I}) \cdot \det((\mbf{D} - \lambda \mbf{I}) - \mbf{C}(\mbf{A} - \lambda \mbf{I})^{-1}\mbf{B}),
    \end{align*}
    where the second equality is by the Schur complement. Notice that
    \begin{align*}
        (\mbf{A} - \lambda \mbf{I})^{-1} = (\mbf{R}_{L}\mbf{H}_{1,1}\mbf{R}_{L}^\top  - \lambda \mbf{I})^{-1} = (\mbf{R}_{L}\mbf{H}_{1,1}\mbf{R}_{L}^\top  - \lambda \mbf{\mbf{R}_{L}\mbf{R}_{L}}^\top)^{-1} = \mbf{R}_{L} \cdot (\mbf{H}_{1,1} - \lambda\mbf{I})^{-1} \cdot \mbf{R}_{L}^\top.
    \end{align*}
    Then, we also see that, 
    \begin{align*}
        \mbf{C}(\mbf{A} - \lambda \mbf{I})^{-1}\mbf{B} = \underbrace{\begin{bmatrix}
            \mbf{R}_{L-1} & & \\
            & \ddots & \\
            & & \mbf{R}_{1}
        \end{bmatrix}}_{\eqqcolon \widehat{\mbf{V}}}\cdot\, 
        \mbf{E}\cdot
        \underbrace{\begin{bmatrix}
            \mbf{R}_{L-1}^\top & & \\
            & \ddots & \\
            & & \mbf{R}_{1}^\top
        \end{bmatrix}}_{\eqqcolon \widehat{\mbf{V}}^\top}.
    \end{align*}
    where
    \begin{align*}
        \mbf{E}\coloneqq
        \begin{bmatrix}
            \mbf{H}_{2, 1} \cdot (\mbf{H}_{1,1} - \lambda \mbf{I})^{-1} \cdot \mbf{H}_{1,2} & \hdots & \mbf{H}_{2,1}\cdot (\mbf{H}_{1,1} - \lambda \mbf{I})^{-1} \cdot \mbf{H}_{1, L} \\
            \vdots & \ddots & \vdots \\
            \mbf{H}_{L, 1}\cdot (\mbf{H}_{1,1} - \lambda \mbf{I})^{-1} \cdot \mbf{H}_{1, 2} & \hdots & \mbf{H}_{L, 1}\cdot (\mbf{H}_{1, 1} - \lambda \mbf{I})^{-1} \cdot \mbf{H}_{1, L}
        \end{bmatrix}.
    \end{align*}
    Similarly, we can write $\mbf{D}$ as 
    \begin{align*}
        \mbf{D} = \widehat{\mbf{V}}
        \underbrace{\begin{bmatrix}
            \mbf{H}_{2,2} & \hdots & \mbf{H}_{2, L} \\
            \vdots & \ddots & \vdots \\
            \mbf{H}_{L, 2} & \hdots & \mbf{H}_{L, L}
        \end{bmatrix}}_{\eqqcolon \mbf{F}}
        \widehat{\mbf{V}}^\top.
    \end{align*}
    Then, we have
    \begin{align*}
        \det(\mbf{W} - \lambda \mbf{I}) &= \det(\mbf{R}_{L}\cdot (\mbf{H}_{1,1} - \lambda \mbf{I})\cdot\mbf{R}_{L}^\top) \cdot \det\left(\widehat{\mbf{V}} \cdot (\mbf{E} - \mbf{F})\cdot \widehat{\mbf{V}}^\top \right) \\
       &= \det(\mbf{H}_{1,1} - \lambda \mbf{I}) \cdot \det(\mbf{E} - \mbf{F}),
    \end{align*}
    which is not a function of $\mbf{U}, \mbf{V}, [\mbf{\sigma}_{l}]_{l=2}^L$. In lemma, we proved that $\mbf{R}_{L}$ and $\widehat{\mbf{V}}$ are orthogonal matrices which do not change the value of determinant.
    
    By doing the same for $\widetilde{\mbf{H}}$, we can show that both $\widetilde{\mbf{H}}$ and $\mbf{W}$ have the same characteristic polynomials, and hence the same eigenvalues. This completes the proof. This shows that the singular vector of the target matrix does not affect the eigenvalues of the Hessian. 
 
\end{proof}


\begin{lemma}
    If $\mbf{R}_{L}$, $\mbf{R}_{L-1}$,.., $\mbf{R}_{1}$ are orthogonal matrices then $ \mbf{R}_{l-1} \otimes \mbf{R}_{l}$ for $l=1,..,L$ is an orthogonal matrix and the block matrix  $\begin{bmatrix}
            \mbf{R}_{L-1} & & \\
            & \ddots & \\
            & & \mbf{R}_{1}
        \end{bmatrix}$ is also an orthogonal matrix. 
\end{lemma}

\begin{proof}

\begin{align*}
   &  (\mbf{R}_{l-1} \otimes \mbf{R}_{l})^{T} (\mbf{R}_{l-1} \otimes \mbf{R}_{l}) \\ 
   & = (\mbf{R}_{l-1}^{T}\mbf{R}_{l-1} ) \otimes (\mbf{R}_{l}^{T}\mbf{R}_{l} ) = \mathbf{I}_{d} \otimes \mathbf{I}_{d} \\
   & = \mathbf{I}_{d^2} 
\end{align*}
    It similarly holds that $ (\mbf{R}_{l-1} \otimes \mbf{R}_{l}) (\mbf{R}_{l-1} \otimes \mbf{R}_{l})^{T} =\mathbf{I}_{d^2} $. 
So, $\mbf{R}_{l-1} \otimes \mbf{R}_{l}$ is orthogonal if  $\mbf{R}_{L}$, $\mbf{R}_{L-1}$,.., $\mbf{R}_{1}$ are orthogonal matrices. 

Similarly, 

$\begin{bmatrix}
            \mbf{R}_{L-1} & & \\
            & \ddots & \\
            & & \mbf{R}_{1}
        \end{bmatrix}^{T} \begin{bmatrix}
            \mbf{R}_{L-1} & & \\
            & \ddots & \\
            & & \mbf{R}_{1}
        \end{bmatrix} = \begin{bmatrix}
            \mbf{R}^{T}_{L-1}\mbf{R}_{L-1}  & & \\
            & \ddots & \\
            & & \mbf{R}^{T}_{1}\mbf{R}_{1} 
        \end{bmatrix} = \mathbf{I}_{d^2} 
    $
    So, the block matrix $\begin{bmatrix}
            \mbf{R}_{L-1} & & \\
            & \ddots & \\
            & & \mbf{R}_{1}
        \end{bmatrix}$ is orthogonal. 
\end{proof}

\end{comment}




\clearpage

\subsection{Deferred Proofs for Singular Vector Invariance}


\begin{manualpropositioninner}
    
\label{prop:one_zero_svs_set}
    Let $\mbf{M}_\star = \mbf{U}_\star\mbf{\Sigma}_\star \mbf{V}_\star^\top$ denote the SVD of the target matrix. The initialization in Equation~(\ref{eqn:init}) is a member of the singular vector stationary set in Proposition~\ref{prop:svs_set}, where $\mbf{Q}_L = \ldots = \mbf{Q}_2 = \mbf{V}_\star$.
\end{manualpropositioninner}
\begin{proof}
Recall that the initialization is given by
    \begin{align*}
        \mbf{W}_L(0) = 0 \quad \text{and} \quad \mbf{W}_\ell(0) = \alpha\mbf{I}_d \quad \forall \ell \in [L-1].
    \end{align*}
    We will show that under this initialization, each weight matrix admits the following decomposition for all $t \geq 1$:
    \begin{align}
        \mbf{W}_L(t) = \mbf{U}_\star \begin{bmatrix}
            \widetilde{\mbf{\Sigma}}_L(t) & \mbf{0} \\
            \mbf{0} & \mbf{0}
        \end{bmatrix} \mbf{V}_\star^\top,
        \quad\quad
        \mbf{W}_{\ell}(t) = \mbf{V}_\star \begin{bmatrix}
            \widetilde{\mbf{\Sigma}}(t) & \mbf{0} \\
            \mbf{0} & \alpha\mbf{I}_{d-r}
        \end{bmatrix} \mbf{V}_\star^\top,
        \quad \forall \ell \in [L-1],
    \end{align}
where
\begin{align*}
    \widetilde{\mbf{\Sigma}}_L(t) &= \widetilde{\mbf{\Sigma}}_L(t-1) - \eta \cdot\left(\widetilde{\mbf{\Sigma}}_L(t-1) \cdot \widetilde{\mbf{\Sigma}}^{L-1}(t-1) - \mbf{\Sigma}_{\star,r}\right)\cdot \widetilde{\mbf{\Sigma}}^{L-1}(t-1) \\
    \widetilde{\mbf{\Sigma}}(t) &= \widetilde{\mbf{\Sigma}}(t-1)\cdot  \left(\mbf{I}_r- \eta\cdot\widetilde{\mbf{\Sigma}}_L(t-1)\cdot\left(\widetilde{\mbf{\Sigma}}_L(t-1) \cdot \widetilde{\mbf{\Sigma}}^{L-1}(t-1) - \mbf{\Sigma}_{\star,r}\right)\cdot \widetilde{\mbf{\Sigma}}^{L-3}(t-1)\right),
\end{align*}
where $\widetilde{\mbf{\Sigma}}_L(t), \widetilde{\mbf{\Sigma}}(t) \in \mbb{R}^{r\times r}$ is a diagonal matrix with $\widetilde{\mbf{\Sigma}}_L(1) = \eta \alpha^{L-1}\cdot \mbf{\Sigma}_{r,\star}$ and $\widetilde{\mbf{\Sigma}}(1) = \alpha \mbf{I}_r$. 

This will prove that the singular vectors are stationary with $\mbf{\Sigma}_L = \ldots =\mbf{\Sigma}_2 = \mbf{V}_\star$. We proceed with mathematical induction. 

\paragraph{Base Case.} For the base case, we will show that the decomposition holds for each weight matrix at $t=1$. The gradient of $f(\mbf{\Theta})$ with respect to $\mbf{W}_{\ell}$ is
\begin{align*}
    \nabla_{\mbf{W}_{\ell}} f(\mbf{\Theta}) = \mbf{W}^{\top}_{L:\ell+1} \cdot \left(\mbf{W}_{L:1} - \mbf{M}_\star \right) \cdot \mbf{W}^{\top}_{\ell-1:1}. 
\end{align*}
For $\mbf{W}_L(1)$, we have
\begin{align*}
    \mbf{W}_L(1) &= \mbf{W}_L(0) - \eta \cdot \nabla_{\mbf{W}_{L}} f(\mbf{\Theta}(0)) \\
    &= \mbf{W}_L(0) - \eta \cdot \left(\mbf{W}_{L:1}(0) - \mbf{M}_\star \right) \cdot \mbf{W}^{\top}_{L-1:1}(0)\\
    &= \eta \alpha^{L-1}\mbf{\Sigma}_\star \\
    &= \mbf{U}_\star \cdot \left( \eta \alpha^{L-1} \cdot \mbf{\Sigma}_\star \right) \cdot \mbf{V}_\star^\top \\
    &= \mbf{U}_\star
    \begin{bmatrix}
        \widetilde{\mbf{\Sigma}}_L(1) & \mbf{0} \\
        \mbf{0} & \mbf{0}
    \end{bmatrix}
    \mbf{V}_\star^\top.
\end{align*}
Then, for each $\mbf{W}_{\ell}(1)$ in $\ell \in [L-1]$, we have
\begin{align*}
\mbf{W}_{\ell}(1)&= \mbf{W}_{\ell}(0) - \eta \cdot \nabla_{\mbf{W}_{\ell}}f(\mbf{\Theta}(0)) \\
&= \alpha\mbf{I}_d,
\end{align*}
where the last equality follows from the fact that $\mbf{W}_L(0) = \mbf{0}$. Finally, we have
\begin{align*}
    \mbf{W}_{\ell}(1) = \alpha \mbf{V}_\star \mbf{V}_\star^\top = \mbf{V}_\star \begin{bmatrix}
        \widetilde{\mbf{\Sigma}}(1) & \mbf{0} \\
        \mbf{0} & \alpha\mbf{I}_{d-r}
     \end{bmatrix}\mbf{V}_\star^\top, \quad \forall \ell \in [L-1].
\end{align*}

\paragraph{Inductive Step.} By the inductive hypothesis, suppose that the decomposition holds. Then, notice that we can simplify the end-to-end weight matrix to
\begin{align*}
    \mbf{W}_{L:1}(t) = \mbf{U}_\star
    \begin{bmatrix}
        \widetilde{\mbf{\Sigma}}_L(t) \cdot \widetilde{\mbf{\Sigma}}^{L-1}(t) & \mbf{0} \\
        \mbf{0} & \mbf{0}
    \end{bmatrix}
    \mbf{V}_\star^\top,
\end{align*}
for which we can simplify the gradients to
\begin{align*}
    \nabla_{\mbf{W}_{L}} f(\mbf{\Theta}(t)) &= \left(\mbf{U}_\star \begin{bmatrix}
        \widetilde{\mbf{\Sigma}}_L(t) \cdot \widetilde{\mbf{\Sigma}}^{L-1}(t) - \mbf{\Sigma}_{\star,r} & \mbf{0} \\
        \mbf{0} & \mbf{0}
    \end{bmatrix} \mbf{V}_\star^\top\right) \cdot  \mbf{V}_\star \begin{bmatrix}
        \widetilde{\mbf{\Sigma}}^{L-1}(t) & \mbf{0} \\
        \mbf{0} & \mbf{0}
    \end{bmatrix}\mbf{V}_\star^\top \\
    &= \mbf{U}_\star \begin{bmatrix}
        \left(\widetilde{\mbf{\Sigma}}_L(t) \cdot \widetilde{\mbf{\Sigma}}^{L-1}(t) - \mbf{\Sigma}_{\star,r}\right)\cdot \widetilde{\mbf{\Sigma}}^{L-1}(t) & \mbf{0} \\
        \mbf{0} & \mbf{0}
    \end{bmatrix} \mbf{V}_\star^\top,
\end{align*}
for the last layer matrix, and similarly,
\begin{align*}
     \nabla_{\mbf{W}_{\ell}} f(\mbf{\Theta}(t)) &= \mbf{V}_\star \begin{bmatrix}
        \widetilde{\mbf{\Sigma}}_L(t)\cdot\left(\widetilde{\mbf{\Sigma}}_L(t) \cdot \widetilde{\mbf{\Sigma}}^{L-1}(t) - \mbf{\Sigma}_{\star,r}\right)\cdot \widetilde{\mbf{\Sigma}}^{L-2}(t)  & \mbf{0} \\
        \mbf{0} & \mbf{0}
    \end{bmatrix} \mbf{V}_\star^\top, \quad \ell \in [L-1],
\end{align*}
for all other layer matrices. Thus, for the next GD iteration, we have
\begin{align*}
    \mbf{W}_L(t+1) &= \mbf{W}_{L}(t) - \eta \cdot \nabla_{\mbf{W}_L}(\mbf{\Theta}(t)) \\
    &= \mbf{U}_\star \begin{bmatrix}
        \widetilde{\mbf{\Sigma}}_L(t) - \eta \cdot\left(\widetilde{\mbf{\Sigma}}_L(t) \cdot \widetilde{\mbf{\Sigma}}^{L-1}(t) - \mbf{\Sigma}_{\star,r}\right)\cdot \widetilde{\mbf{\Sigma}}^{L-1}(t) & \mbf{0} \\
        \mbf{0} & \mbf{0}
    \end{bmatrix} \mbf{V}_\star^\top \\
    &= \mbf{U}_\star \begin{bmatrix}
        \widetilde{\mbf{\Sigma}}_L(t+1) & \mbf{0} \\
        \mbf{0} & \mbf{0}
    \end{bmatrix} \mbf{V}_\star^\top.
\end{align*}
Similarly, we have
\begin{align*}
    \mbf{W}_\ell(t+1) &= \mbf{W}_{\ell}(t) - \eta \cdot \nabla_{\mbf{W}_\ell}(\mbf{\Theta}(t)) \\
    &= \mbf{V}_\star \begin{bmatrix}
        \widetilde{\mbf{\Sigma}}(t) - \eta\cdot\widetilde{\mbf{\Sigma}}_L(t)\cdot\left(\widetilde{\mbf{\Sigma}}_L(t) \cdot \widetilde{\mbf{\Sigma}}^{L-1}(t) - \mbf{\Sigma}_{\star,r}\right)\cdot \widetilde{\mbf{\Sigma}}^{L-2}(t)  & \mbf{0} \\
        \mbf{0} & \alpha \mbf{I}_{d-r}
    \end{bmatrix} \mbf{V}_\star^\top \\
     &= \mbf{V}_\star \begin{bmatrix}
        \widetilde{\mbf{\Sigma}}(t)\cdot  \left(\mbf{I}_r- \eta\cdot\widetilde{\mbf{\Sigma}}_L(t)\cdot\left(\widetilde{\mbf{\Sigma}}_L(t) \cdot \widetilde{\mbf{\Sigma}}^{L-1}(t) - \mbf{\Sigma}_{\star,r}\right)\cdot \widetilde{\mbf{\Sigma}}^{L-3}(t)\right)  & \mbf{0} \\
        \mbf{0} & \alpha \mbf{I}_{d-r}
    \end{bmatrix} \mbf{V}_\star^\top \\
    &= \mbf{V}_\star \begin{bmatrix}
        \widetilde{\mbf{\Sigma}}(t+1) & \mbf{0} \\
        \mbf{0} & \alpha \mbf{I}_{d-r}
    \end{bmatrix} \mbf{V}_\star^\top,
\end{align*}
for all $\ell \in [L-1]$. This completes the proof.
\end{proof}




\begin{manualpropositioninner}
\label{prop:balanced_svs_set}

 Let $\mbf{M}_\star = \mbf{V}_\star\mbf{\Sigma}_\star \mbf{V}_\star^\top \in \mbb{R}^{d\times d}$ denote the SVD of the target matrix. The balanced initialization in Equation~(\ref{eqn:init}) is a member of the singular vector stationary set in Proposition~\ref{prop:svs_set}, where  $\mbf{U}_L = \mbf{Q}_L = \ldots = \mbf{Q}_2 = \mbf{V}_1 = \mbf{V}_\star$.
 
\end{manualpropositioninner}

\begin{proof}
    
Using mathematical induction, we will show that with the balanced initialization in Equation~(\ref{eqn:init}), each weight matrix admits a decomposition of the form
\begin{align}
    \mbf{W}_\ell(t) = \mbf{V}_\star \mbf{\Sigma}_\ell(t) \mbf{V}_\star^\top,
\end{align}
which implies that the singular vectors are stationary for all $t$ such that $\mbf{U}_L = \mbf{Q}_L = \ldots = \mbf{Q}_2 = \mbf{V}_1 = \mbf{V}_\star$.

\paragraph{Base Case.} Consider the weights at iteration $t=0$. By the initialization scheme, we can write each weight matrix as
\begin{align*}
    \mbf{W}_\ell(0) = \alpha \mbf{I}_d \implies  \mbf{W}_\ell(0) = \alpha \mbf{V}_\star \mbf{V}_\star^\top,
\end{align*}
which implies that $\mbf{W}_\ell(0) = \mbf{V}_\star \mbf{\Sigma}_\ell(0)\mbf{V}_\star^\top$ with $\mbf{\Sigma}_\ell(0) = \alpha \mbf{I}_d$.

\paragraph{Inductive Step.} By the inductive hypothesis, assume that the decomposition holds for all $t \geq 0$. We will show that it holds for all iterations $t+1$. Recall that the gradient of $f(\mbf{\Theta})$ with respect to $\mbf{W}_{\ell}$ is
\begin{align*}
    \nabla_{\mbf{W}_{\ell}} f(\mbf{\Theta}) = \mbf{W}^{\top}_{L:\ell+1} \cdot \left(\mbf{W}_{L:1} - \mbf{M}_\star \right) \cdot \mbf{W}^{\top}_{\ell-1:1}. 
\end{align*}
Then, for $\mbf{W}_\ell(t+1)$, we have
\begin{align*}
    \mbf{W}_\ell(t+1) &= \mbf{W}_\ell(t) - \eta \cdot \nabla_{\mbf{W}_{L}} f(\mbf{\Theta}(t)) \\
    &=  \mbf{V}_\star \mbf{\Sigma}_\ell(t)\mbf{V}_\star^\top - \eta \mbf{W}^\top_{L:\ell+1}(t) \cdot \left(\mbf{W}_{L:1}(t) - \mbf{M}_\star \right) \cdot \mbf{W}^{\top}_{\ell-1:1}(t)\\
    &=  \mbf{V}_\star \mbf{\Sigma}_\ell(t)\mbf{V}_\star^\top - \eta \mbf{V}_\star\cdot \left(  \mbf{\Sigma}^{L-\ell}_\ell(t)\cdot \left(\mbf{\Sigma}_\ell^{L}(t) - \mbf{\Sigma}_\star \right)\cdot \mbf{\Sigma}_\ell^{\ell-1}(t) \right) \cdot\mbf{V}^{\top}_{\star}\\
    &=  \mbf{V}_\star\cdot \left(\mbf{\Sigma}_\ell(t) - \eta\cdot  \mbf{\Sigma}^{L-\ell}_\ell(t)\cdot \left(\mbf{\Sigma}_\ell^{L}(t) - \mbf{\Sigma}_\star \right)\cdot \mbf{\Sigma}_\ell^{\ell-1}(t) \right) \cdot\mbf{V}^{\top}_{\star}\\
    &= \mbf{V}_\star
   \mbf{\Sigma}(t)
    \mbf{V}_\star^\top,
\end{align*}
where $\mbf{\Sigma}(t) = \mbf{\Sigma}_\ell(t) - \eta\cdot  \mbf{\Sigma}^{L-\ell}_\ell(t)\cdot \left(\mbf{\Sigma}_\ell^{L}(t) - \mbf{\Sigma}_\star \right)\cdot \mbf{\Sigma}_\ell^{\ell-1}(t)$. This completes the proof.
\end{proof}



\subsection{Auxiliary Results}


\begin{manuallemmainner}
\label{lem:relationship_lemma} 
    Let $\{\mbf{R}_{\ell}\}_{\ell=1}^L \in \mathbb{R}^{n\times n}$ be orthogonal matrices and $\mbf{H}_{i, j} \in \mathbb{R}^{n^2 \times n^2}$ be diagonal matrices. Consider the two following block matrices:
    \begin{align*}
       \mbf{H} &= \begin{bmatrix}
            \mbf{H}_{1,1} & \mbf{H}_{1, 2} & \hdots &\mbf{H}_{L, 1}\\
            \mbf{H}_{2,1} & \mbf{H}_{2,2} & \hdots & \mbf{H}_{L, 2} \\
            \vdots & \vdots & \ddots & \vdots \\
            \mbf{H}_{1, L} & \mbf{H}_{2, L} & \hdots &\mbf{H}_{L, L}
        \end{bmatrix} \\  \widetilde{\mbf{H}} &=
      \begin{bmatrix}
        \mbf{R}_{L}\mbf{H}_{1,1}\mbf{R}_{L}^{\top} & \mbf{R}_{L}\mbf{H}_{1, 2}\mbf{R}_{L-1}^{\top} & \hdots & \mbf{R}_{L}\mbf{H}_{1, L}\mbf{R}_{1}^{\top}\\
        \mbf{R}_{L-1}\mbf{H}_{2,1}\mbf{R}_{L}^{\top} & \mbf{R}_{L-1}\mbf{H}_{2,2}\mbf{R}_{L-1}^{\top} & \hdots & \mbf{R}_{L-1}\mbf{H}_{2, L}\mbf{R}_{1}^{\top}\\
        \vdots & \vdots & \ddots & \vdots \\
        \mbf{R}_{1}\mbf{H}_{L,1}\mbf{R}_{L}^{\top} & \mbf{R}_{1}\mbf{H}_{L,2}\mbf{R}_{L-1}^{\top} & \hdots & \mbf{R}_{1}\mbf{H}_{L,L}\mbf{R}_{1}^{\top}
    \end{bmatrix}.
    \end{align*}
    Then, the two matrices $\mbf{H}$ and $\widetilde{\mbf{H}}$ are similar, in the sense that they have the same eigenvalues.
\end{manuallemmainner}


\begin{proof}
It suffices to show that $\mbf{H}$ and $ \widetilde{\mbf{H}}$ have the same characteristic polynomials. Let us define 
    \begin{align*}
        \widetilde{\mbf{H}} \coloneqq \begin{bmatrix}
            \mbf{A} & \mbf{B} \\
            \mbf{C} & \mbf{D}
        \end{bmatrix},
    \end{align*}
    where 
    \begin{alignat}{3}
        &\mbf{A} \coloneqq  \mbf{R}_{L}\mbf{H}_{1,1}\mbf{R}_{L}^{\top} \quad\quad\quad &\mbf{B} &\coloneqq \begin{bmatrix}
            \mbf{R}_{L}\mbf{H}_{1, 2}\mbf{R}_{L-1}^{\top} & \hdots & \mbf{R}_{L}\mbf{H}_{1, L}\mbf{R}_{1}^{\top}
        \end{bmatrix} \\
        &\mbf{C} \coloneqq \begin{bmatrix}
            \mbf{R}_{L-1}\mbf{H}_{2,1}\mbf{R}_{L}^{\top} \\
            \vdots \\
           \mbf{R}_{1}\mbf{H}_{L,1}\mbf{R}_{L}^{\top}
        \end{bmatrix}  \quad\quad\quad
        &\mbf{D} &\coloneqq \begin{bmatrix}
           \mbf{R}_{L-1}\mbf{H}_{2,2}\mbf{R}_{L-1}^{\top} & \hdots & \mbf{R}_{L-1}\mbf{H}_{2, L}\mbf{R}_{1}^{\top}\\ \\
            \vdots & \ddots & \vdots \\
           \mbf{R}_{1}\mbf{H}_{L,2}\mbf{R}_{L-1}^{\top} & \hdots & \mbf{R}_{1}\mbf{H}_{L,L}\mbf{R}_{1}^{\top}
        \end{bmatrix}.
    \end{alignat}
    Then, we have
    \begin{align*}
        \det(\widetilde{\mbf{H}} - \lambda \mbf{I}) &= \det\left(\begin{bmatrix}
            \mbf{A} - \lambda\mbf{I} & \mbf{B} \\
            \mbf{C} & \mbf{D} - \lambda\mbf{I}
        \end{bmatrix}\right) \\
        &= \det(\mbf{A} - \lambda \mbf{I}) \cdot \det((\mbf{D} - \lambda \mbf{I}) - \mbf{C}(\mbf{A} - \lambda \mbf{I})^{-1}\mbf{B}),
    \end{align*}
    where the second equality is by the Schur complement. Notice that
    \begin{align*}
        (\mbf{A} - \lambda \mbf{I})^{-1} = (\mbf{R}_{L}\mbf{H}_{1,1}\mbf{R}_{L}^\top  - \lambda \mbf{I})^{-1} &= (\mbf{R}_{L}\mbf{H}_{1,1}\mbf{R}_{L}^\top  - \lambda \mbf{\mbf{R}_{L}\mbf{R}_{L}}^\top)^{-1} \\&= \mbf{R}_{L} \cdot (\mbf{H}_{1,1} - \lambda\mbf{I})^{-1} \cdot \mbf{R}_{L}^\top.
    \end{align*}
    Then, we also see that, 
    \begin{align*}
        \mbf{C}(\mbf{A} - \lambda \mbf{I})^{-1}\mbf{B} = \underbrace{\begin{bmatrix}
            \mbf{R}_{L-1} & & \\
            & \ddots & \\
            & & \mbf{R}_{1}
        \end{bmatrix}}_{\eqqcolon \widehat{\mbf{V}}}\cdot\, 
        \mbf{E}\cdot
        \underbrace{\begin{bmatrix}
            \mbf{R}_{L-1}^\top & & \\
            & \ddots & \\
            & & \mbf{R}_{1}^\top
        \end{bmatrix}}_{\eqqcolon \widehat{\mbf{V}}^\top}.
    \end{align*}
    where
    \begin{align*}
        \mbf{E}\coloneqq
        \begin{bmatrix}
            \mbf{H}_{2, 1} \cdot (\mbf{H}_{1,1} - \lambda \mbf{I})^{-1} \cdot \mbf{H}_{1,2} & \hdots & \mbf{H}_{2,1}\cdot (\mbf{H}_{1,1} - \lambda \mbf{I})^{-1} \cdot \mbf{H}_{1, L} \\
            \vdots & \ddots & \vdots \\
            \mbf{H}_{L, 1}\cdot (\mbf{H}_{1,1} - \lambda \mbf{I})^{-1} \cdot \mbf{H}_{1, 2} & \hdots & \mbf{H}_{L, 1}\cdot (\mbf{H}_{1, 1} - \lambda \mbf{I})^{-1} \cdot \mbf{H}_{1, L}
        \end{bmatrix}.
    \end{align*}
    Similarly, we can write $\mbf{D}$ as 
    \begin{align*}
        \mbf{D} = \widehat{\mbf{V}}
        \underbrace{\begin{bmatrix}
            \mbf{H}_{2,2} & \hdots & \mbf{H}_{2, L} \\
            \vdots & \ddots & \vdots \\
            \mbf{H}_{L, 2} & \hdots & \mbf{H}_{L, L}
        \end{bmatrix}}_{\eqqcolon \mbf{F}}
        \widehat{\mbf{V}}^\top.
    \end{align*}
    Then, we have
    \begin{align*}
        \det(\widetilde{\mbf{H}} - \lambda \mbf{I}) &= \det(\mbf{R}_{L}\cdot (\mbf{H}_{1,1} - \lambda \mbf{I})\cdot\mbf{R}_{L}^\top) \cdot \det\left(\widehat{\mbf{V}} \cdot (\mbf{E} - \mbf{F})\cdot \widehat{\mbf{V}}^\top \right) \\
       &= \det(\mbf{H}_{1,1} - \lambda \mbf{I}) \cdot \det(\mbf{E} - \mbf{F}),
    \end{align*}
    which is not a function of $\mbf{U}, \mbf{V},\{\mbf{R}_{\ell}\}_{\ell=1}^L$. By doing the same for $\mbf{H}$, we can show that both $\widetilde{\mbf{H}}$ and $\mbf{H}$ have the same characteristic polynomials, and hence the same eigenvalues. This completes the proof.


\end{proof}


\begin{manuallemmainner}
\label{lemma:kronecker_ortho}
   Let $\mbf{A}, \mbf{B} \in \mbb{R}^{d\times d}$ be two orthogonal matrices. Then, the Kronecker product of $\mbf{A}$ and $\mbf{B}$ is also an orthogonal matrix:
   \begin{align*}
       (\mbf{A} \otimes \mbf{B})^\top (\mbf{A} \otimes \mbf{B}) = (\mbf{A} \otimes \mbf{B})(\mbf{A} \otimes \mbf{B})^\top = \mbf{I}_{d^2}.
   \end{align*}
\end{manuallemmainner}

\begin{proof}
We prove this directly by using properties of Kronecker products:
\begin{align*}
    (\mbf{A} \otimes \mbf{B})^\top (\mbf{A} \otimes \mbf{B}) &= \mbf{A}^\top \mbf{A} \otimes \mbf{B}^\top \mbf{B} \\
    &= \mbf{I}_d \otimes \mbf{I}_d = \mbf{I}_{d^2}.
\end{align*}
Similarly, we have
\begin{align*}
    (\mbf{A} \otimes \mbf{B}) (\mbf{A} \otimes \mbf{B})^\top &= \mbf{A} \mbf{A}^\top \otimes \mbf{B} \mbf{B}^\top \\
    &= \mbf{I}_d \otimes \mbf{I}_d = \mbf{I}_{d^2}.
\end{align*}
This completes the proof.
\end{proof}

\begin{manuallemmainner}
\label{lemm:seq_converge}
    Let $\{a(t)\}_{t=1}^N$ be a sequence such that $a(t) \geq 0$ for all $t$. 
    If there exists a constant $c \in (0,1)$ such that $a(t+1) < c \cdot a(t)$ for all $t$, 
    then $\lim_{t \to \infty} a(t) = 0$.

\end{manuallemmainner}

\begin{proof}
   We prove this by direct reasoning. 
    From the assumption $a(t+1) < c \cdot a(t)$ for some $c \in (0,1)$, we can iteratively expand this inequality:
    \[
    a(t+1) < c \cdot a(t), \quad a(t+2) < c \cdot a(t+1) < c^2 \cdot a(t),
    \]
    and, more generally, by induction:
    \[
    a(t+k) < c^k \cdot a(t), \quad \text{for all } k \geq 0.
    \]
    Since $c \in (0,1)$, the sequence $\{c^k\}_{k=0}^\infty$ converges to $0$ as $k \to \infty$. Hence:
    \[
    0\leq \lim_{k \to \infty} a(t+k) \leq \lim_{k \to \infty} c^k \cdot a(t) = 0.
    \]
    Therefore, by the squeeze theorem, the sequence $\{a(t)\}$ converges to $0$ as $t \to \infty$.
\end{proof}





\begin{manuallemmainner}
[\cite{chen2023edge}]
\label{lemma:chen-bruna}
Consider any 1-D differentiable function $f(x)$ around a local minima $\bar{x}$, satisfying (i) $f^{(3)}(\bar{x}) \neq 0$, and (ii) $3[f^{(3)}]^2 - f'' f^{(4)} > 0$ at $\bar{x}$. Then, there exists $\epsilon$ with sufficiently small $|\epsilon|$ and $\epsilon \cdot f^{(3)} > 0$ such that: for any point $x_0$ between $\bar{x}$ and $\bar{x} - \epsilon$, there exists a learning rate $\eta$ such that $F_{\eta}^2(x_0) = x_0$, and
\end{manuallemmainner}

\[
\frac{2}{f''(\bar{x})} < \eta < \frac{2}{f''(\bar{x}) - \epsilon \cdot f^{(3)}(\bar{x})}.
\]

\clearpage

\begin{manualtheoreminner}
    Let $\eta \geq \frac{2}{K}$, where $K = L\sigma_{\star}^{2- 2/L}$. If we run GD on the singular value loss with learning rate $\eta$, then there exists $\delta_1 \in (0, 1)$ and $\delta_2 \in (1, 2)$ such that if $\sigma_{\ell}(t) \in \left((\delta_1 \sigma_\star)^{1/L}, \sigma_\star^{1/L}\right)$, then for some $t \geq 0$,
    \begin{align*}
    \sigma_{\ell}(t+1) \in \left(\sigma_\star^{1/L}, (\delta_2 \sigma_\star)^{1/L} \right)
    \quad \text{and}
    \quad \sigma_{\ell}(t+2) \in \left((\delta_1 \sigma_\star)^{1/L}, \sigma_\star^{1/L} \right), \quad \forall \ell \in [L].
    \end{align*}

    \noindent Moreover, if $\sigma_{\ell}(t)$ are balanced for all $\ell \in [L]$, then the singular values oscillates in a $2$-period orbit ($j \in \{1,2\}$) around the balanced minimum and admits the following decomposition:
\begin{align}
    \mbf{W}_{L:1} = \underbrace{\sum_{i=1}^p\rho_{i, j}^L \cdot \mbf{u}_{\star, i}\mbf{v}_{\star, i}^{\top} }_{\text{oscillation subspace}}+ \underbrace{\sum_{k=p+1}^d \sigma_{\star, k}\cdot \mbf{u}_{\star, k}\mbf{v}_{\star, k}^{\top}}_{\text{stationary subspace}}, \quad j \in \{1,2\}, \quad \forall\ell \in [L-1],
\end{align}
where $\rho_{i, 1} \in \left(0, \sigma_{\star, i}^{1/L}\right)$ and $\rho_{i, 2} \in \left(\sigma_{\star, i}^{1/L}, (2\sigma_{\star, i})^{1/L}\right)$ are the two real roots of the polynomial $g(\rho_i)=0$ and
\begin{align*}
    g(\rho_i) = \rho_i^L\cdot\frac{1+\left(1 + \eta L(\sigma_{\star, i} - \rho_i^L)\cdot \rho_i^{L-2} \right)^{2L-1}}{1+\left(1 + \eta L(\sigma_{\star, i} - \rho_i^L)\cdot \rho_i^{L-2} \right)^{L-1}} - \sigma_{\star, i}.
\end{align*}
\end{manualtheoreminner}

\begin{proof}
    Suppose that for all $\ell \in [L]$,  $\sigma_{\ell}(t) \in \left((\delta_1 \sigma_\star)^{1/L}, \sigma_\star^{1/L}\right)$ for some $\delta_1 \in (0, 1)$. Then, for any $a_\ell \in (0, 1)$, we can write $\sigma_\ell(t) = (a_\ell \sigma_\star)^{1/L}$. First, we will show that 
    \begin{align}
    \label{eqn:sval_gd}\sigma_\ell(t+1) = \sigma_\ell(t) - \eta \cdot \left(\sigma_L(t)\cdot \ldots \cdot \sigma_1(t) - \sigma_\star\right) \cdot \prod_{i\neq \ell} \sigma_i(t),
    \end{align}
    for $\sigma_\ell(t+1) \in \left(\sigma_\star^{1/L}, (2\sigma_\star)^{1/L} \right)$. It suffices to show that $\sigma_\ell(t+1) = (b_\ell \sigma_\star)^{1/L}$ for some $b_\ell \in (1,2)$ for all $\ell \in [L]$.

    By plugging into Equation~(\ref{eqn:sval_gd}), we have
    \begin{align*}
        (b_\ell \sigma_\star)^{1/L} &= (a_\ell \sigma_\star)^{1/L} - \eta \left(\sigma_\star\cdot \prod_{k=1}^L a_k^{1/L} - \sigma_\star\right) \cdot \prod_{i\neq \ell} (a_i \sigma_\star)^{1/L} \\
        &= (a_\ell \sigma_\star)^{1/L} + \eta \sigma_\star \cdot \left(1- \prod_{k=1}^L a_k^{1/L}\right) \cdot \sigma_\star^{(L-1)/ L}\cdot \prod_{i\neq \ell} a_i ^{1/L} \\
        &= \sigma_\star^{1/L} \cdot \left( a_\ell^{1/L} + \eta \sigma_\star^{(L-2)/ L} \cdot\left(1- \prod_{k=1}^L a_k^{1/L}\right) \cdot  \prod_{i\neq \ell} a_i ^{1/L} \right) \\
        \implies b_\ell^{1/L} &= a_\ell^{1/L} + \eta \sigma_\star^{(L-2)/ L} \cdot\left(1- \prod_{k=1}^L a_k^{1/L}\right) \cdot  \prod_{i\neq \ell} a_i ^{1/L} \\
        &\geq  a_\ell^{1/L} + \frac{2}{L} \cdot\left(1- \prod_{k=1}^L a_k^{1/L}\right) \cdot  \prod_{i\neq \ell} a_i ^{1/L} \tag{$\eta \geq \frac{2}{K}$} \\
        \implies b_\ell &\geq \left(a_\ell^{1/L} + \frac{2}{L} \cdot\left(1- \prod_{k=1}^L a_k^{1/L}\right) \cdot  \prod_{i\neq \ell} a_i ^{1/L}  \right)^L.
    \end{align*}
    
    
\end{proof}


\begin{manuallemmainner}
    
    Let $S_i \coloneqq \sigma_{\star, i}^{2 - 2/L}$. Suppose we run GD with learning rate $\eta = \frac{2}{LK}$, where $\mathrm{max}\{S_{i+1}, \frac{S_i}{\sqrt{2}}\}<K\leq S_i$ on the simplified loss in~(\ref{eqn:simplified_loss}). Suppose that the singular values are oscillating such that if $\sigma_\ell(t) \in (0, \sigma_\star^{1/L})$, we have
    \begin{align*}
        \sigma_\ell(t+1) \in (\sigma_\star^{1/L}, (2\sigma_\star)^{1/L}) \quad \text{and} \quad \sigma_\ell(t+2) \in (0, \sigma_\star^{1/L}). 
    \end{align*}
    Then, the balancing gap defined as $|b_{i, j}(t)| \coloneqq |\sigma_i^2(t) - \sigma_j^2(t)|$ decreases as follows:
    \begin{align*}
        |b_{i, j}(t+1)| = c\cdot |b_{i, j}(t)|,
    \end{align*}
    for some constant $c \in (0, 1)$.    
\end{manuallemmainner}
\begin{proof}
    Let us define $\pi(t) \coloneqq \sigma_L(t) \cdot \ldots \cdot \sigma_1(t)$. The balancing dynamics can be simplified to
    \begin{align*}
        b_{i, j}(t+1) =  b_{i, j}(t) \cdot \underbrace{\left| 1 - \eta^2 (\pi(t) - \sigma_\star)^2 \cdot \frac{\pi^2(t)}{\sigma^2_i(t) \sigma^2_j(t)} \right|}_{\eqqcolon c(t)}.
    \end{align*}
    We need to show that $c(t) \in (0, 1)$ for all $t$. Suppose that $\sigma_\ell(t) \in (0, \sigma_\star^{1/L})$ for all $\ell \in [L]$. That is, let $\sigma_\ell = (a_\ell \sigma_\star)^{1/L})$ for any constant $a_\ell \in (0, 1)$. Then, $c(t)$ is given as 
    \begin{align*}
        c(t) &=  \left| 1 - \eta^2 (\pi(t) - \sigma_\star)^2 \cdot \frac{\pi^2(t)}{\sigma^2_i(t) \sigma^2_j(t)} \right| \\
        &= \left| 1 - \eta^2 (\sigma_\star\prod_\ell a_\ell^{1/L} - \sigma_\star)^2 \cdot \frac{\sigma_\star^2 \cdot \prod_\ell a_\ell^{2/L}}{((a_i a_j)^{2/L})\cdot \sigma_\star^{4/L}}\right| \\
        &= \left| 1 - \eta^2 \sigma_\star^2( a_\ell^{1/L} - 1)^2 \cdot \frac{\sigma_\star^2 \cdot \prod_\ell a_\ell^{2/L}}{((a_i a_j)^{2/L})\cdot \sigma_\star^{4/L}}\right| \\
        &= \left|1- \eta^2 \frac{( a_\ell^{1/L} - 1)^2\cdot \prod_\ell a_\ell^{2/L}}{((a_i a_j)^{2/L})} \cdot \sigma_\star^{\frac{4L -4}{L}} \right|.
    \end{align*}
    Now, notice that since each $a_\ell < 1$, it follows that the quantity
    \begin{align*}
        \frac{( a_\ell^{1/L} - 1)^2\cdot \prod_\ell a_\ell^{2/L}}{((a_i a_j)^{2/L})} < 1 \implies \frac{( a_\ell^{1/L} - 1)^2\cdot \prod_\ell a_\ell^{2/L}}{((a_i a_j)^{2/L})} \cdot \frac{4}{L^2} < 1,
    \end{align*}
    \smk{need to verify the fraction / denominator}
    where the $\frac{4}{L^2}$ term comes from $\eta$ and holds since $L\geq 2$.
    Since the above quantity is less than 1, that means that we need to guarantee that 
    \begin{align*}
        \frac{\sigma_\star^{\frac{4L-4}{L}}}{K^2} < 2,
    \end{align*}
    which is satisfied as long as $K > \sqrt{\frac{\sigma_\star^{\frac{4L-4}{L}}}{2} } = \frac{\sigma_\star^{\frac{2L-2}{L}}}{\sqrt{2}}$.

Similarly, consider $a_\ell \in (1, 2)$. This boils down to showing that 
\begin{align*}
    \frac{( a_\ell^{1/L} - 1)^2\cdot \prod_\ell a_\ell^{2/L}}{((a_i a_j)^{2/L})} \cdot \frac{4}{L^2} < 1.
\end{align*}

\end{proof}


\begin{comment}
    
Let $\mbf{U} \in \mbb{R}^{d\times r}$ represent an $r$-dimensional basis and $\mbf{U}_\perp \in \mbb{R}^{d\times d-r}$ be its orthogonal complement. Define $\beta_{\text{task}} \sim f_{\text{task}} \coloneqq \mathcal{N}(0, \mbf{UU}^\top)$ and $\beta_{\text{ood}} \sim f_{\text{ood}} \coloneqq \mathcal{N}(0, \mbf{U}_\perp \mbf{U}_\perp^\top)$. Given feature vectors $\mbf{x} \sim \mathcal{N}(0, \mbf{I}_d)$, suppose we pretrain a GPT2 model with $y = \beta_{\text{task}}^\top \mbf{x}$. Given a query say $\mbf{x}_{n+1}$, based on the literature, ICL should be able to ``complete'' the prompt for any $\alpha_{\text{task}} \in f_{\text{task}}$. That is, even if we train using $\beta_{\text{task}}$, ICL should be able to perform well on the in-context prompt
\begin{align*}
    \mbf{Z} = \begin{bmatrix}
        \mbf{x}_1 & \ldots & \mbf{x}_n & \mbf{x}_{n+1} \\
        \alpha_{\text{task}}^\top\mbf{x}_1 & \ldots & \alpha_{\text{task}}^\top\mbf{x}_n & 0
    \end{bmatrix},
\end{align*}
since $\beta_{\text{task}}$ and $\alpha_{\text{task}}$ are drawn from the same distribution.

If ICL can truly do out-of-distribution generalization, that means that based on this framework, we can construct a query say
\begin{align*}
    \mbf{Z} = \begin{bmatrix}
        \mbf{x}_1 & \ldots & \mbf{x}_n & \mbf{x}_{n+1} \\
        \beta_{\text{ood}}^\top\mbf{x}_1 & \ldots & \beta_{\text{ood}}^\top\mbf{x}_n & 0
    \end{bmatrix},
\end{align*}
and it should perform well on this prompt. Though, there exists a few work in the literature that states that ICL does not perform well on out-of-distribution tasks (e.g., the ICLR paper I sent). In fact, they state that even when you increase the number of pre-training tasks, ICL cannot generalize. I wonder if we can demonstrate this using this framework. For example, we can increase $r \to d$ and observe if ICL can ``increasingly'' do better on ood tasks as $r$ gets closer to $d$, as that would be analagous to ``increasing the number of training tasks'' (I think).
\end{comment}


==> ICLR/text/experiments.tex <==

\section{Experimental Results}


%Section~\ref{sec:oscillations_exp} presents experiments that corroborate our theory. Section~\ref{sec:unexplained_exp} discusses \edit{(i) phenomena in non-linear networks currently unexplained in the literature and how our theory can account for them in deep linear networks} \edit{and (ii) how landscape in DLNs behave at EOS compared to more complicated non-convex landscapes.} 



\begin{comment}

\begin{figure}[t]
    \centering
    \hfill
    \raisebox{1.4cm}{\rotatebox{90}{\footnotesize DLN}}
    \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \caption*{\footnotesize Stable Region}
\includegraphics[width=\textwidth]{figures/oscillation/eos_sval_none.pdf}
        
     \end{subfigure}
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
        \caption*{\footnotesize 1-D Oscillation Region}
        \includegraphics[width=\textwidth]{figures/oscillation/eos_sval_1.pdf}
     \end{subfigure}
         \begin{subfigure}[b]{0.32\textwidth}
         \centering
        \caption*{\footnotesize 2-D Oscillation Region}\includegraphics[width=\textwidth]{figures/oscillation/eos_sval_2.pdf} 
     \end{subfigure}
     \hfill
        \newline
        \hfill
        \raisebox{1.5cm}{\rotatebox{90}{\footnotesize	 Diagonal LN}}
        \hfill
      \begin{subfigure}[b]{0.32\textwidth}
         \centering
        \includegraphics[width=\textwidth]{figures/oscillation/eos_sval_diag_none.pdf}
         \caption*{$K > \lambda_1$}
     \end{subfigure}
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
        \includegraphics[width=\textwidth]{figures/oscillation/eos_sval_diag_1.pdf}
         \caption*{ $\lambda_1>K>\lambda_2$}
     \end{subfigure}
         \begin{subfigure}[b]{0.32\textwidth}
         \centering
        \includegraphics[width=\textwidth]{figures/oscillation/eos_sval_diag_2.pdf} 
         \caption*{$\lambda_1 > \lambda_2 > K$}
     \end{subfigure}   
     \hfill
    \caption{
    Dynamics of the singular values of the end-to-end DLN (top) and diagonal linear network (bottom) trained using a learning rate $\eta = 2/K$. $\lambda_1 = L\sigma_{\star, 1}^{2 - 2/L}$ and $\lambda_2 = \sum_{\ell=0}^{L-1} \left(\sigma_{\star, 1}^{1-\frac{1}{L} - \frac{1}{L}\ell} \cdot \sigma_{\star, 2}^{\frac{1}{L}\ell}\right)^2$ are the top two eigenvalues of the Hessian of the training loss at convergence for the DLN. By Theorem~\ref{thm:align_thm}, the DLN has corresponding oscillations for these two regimes, while the diagonal linear network does not due to the difference in the curvature of the landscape.}
    \label{fig:diff_dln_diag}
\end{figure}
\end{comment}


\subsection{Subspace Oscillations in Deep Networks}
\label{sec:oscillations_exp}


Firstly, we provide experimental results corroborating Theorem~\ref{thm:align_thm}. 
We let the target matrix be $\mbf{M}_\star \in \mbb{R}^{50 \times 50}$ with rank 3, with dominant singular values $\sigma_{\star} = {10, 9.5, 9}$.
For the DLN, we consider a 3-layer network, with each layer as $\mbf{W}_\ell \in \mbb{R}^{50\times 50}$ and use an initialization scale of $\alpha = 0.01$.
%For the diagonal linear network, we consider a similar setup, with initialization scale $\alpha = 0.01$ and the top-3 elements of $\mbf{s}_\star \in \mbb{R}^{50}$ to be $10, 9, 6$. 
\begin{wrapfigure}{r}{0.35\textwidth}
  \begin{center}
    \includegraphics[width=0.35\textwidth]{figures/eos_osc_range.pdf}
  \end{center}
  \caption{Oscillation range as a function of the learning rate.}
\label{fig:osc_range}
\end{wrapfigure}
In Figure~\ref{fig:thm2_osc}, we present the behaviors of the singular values of the end-to-end network under different learning rate regimes. Recall that by Theorem~\ref{thm:align_thm}, the $i$-th singular value undergoes periodic oscillations when $K$ is set to be $S_i < K < S_{i+1}$, where $S_i = L\sigma_{\star, i}^{2-2/L}$. Figure~\ref{fig:thm2_osc} illustrates this clearly -- we only observe oscillations in the $i$-th coordinate depending on the learning rate. Interestingly, notice that $\sigma_2$ also begins to oscillate in the rank-$1$ oscillation region before settling at a minimum. This occurs because, while the learning rate is large enough to catapult out of a minimum, it is not sufficiently large to induce periodic oscillations.




%However, the difference in the loss landscape plays a role in oscillations for the second component.
%When $\eta > 2/\lambda_2$, where $\lambda_2$ is the second largest eigenvalue of the DLN, the diagonal linear network does not experience oscillations in the second component, as its second largest eigenvalue is much smaller. 
%This highlights a distinction between the two networks and how the landscape changes between them. 

In Figure~\ref{fig:osc_range}, we present an experiment demonstrating the relationship between the oscillation range and the learning rate by plotting the amplitude of the singular value oscillations in the end-to-end network. The oscillations begin to occur starting from each region $\eta = 2/S_i$, and the oscillation range (or amplitude) increases as the learning rate increases. This can also be observed in Figure~\ref{fig:thm2_osc}; the amplitude of $\sigma_1$ increases as we move from the rank-$1$ to the rank-$3$ oscillation region.

%\edit{In Figure~\ref{fig:osc_range} (right), we present an experiment showing that deeper networks require a smaller $\eta$ to enter the EOS regime, as predicted by the eigenvalue computation in Lemma~\ref{lemma:hessian_eigvals}. Here, we consider the same setup as above, but with a leading target singular value of $\sigma_{\star, 1} = 0.5$.}









\subsection{\edit{Similarities and Differences Between Linear and Nonlinear Nets at EOS}}
\label{sec:unexplained_exp}

%In this section, we draw parallels between observations made in deep nonlinear networks and our theory on DLNs.



\paragraph{Mild Sharpening.} \edit{``Mild'' sharpening refers to the sharpness not rising to $2/\eta$ throughout learning, and generally occurs in tasks with low complexity as discussed in Caveat 2 of \citep{cohen2021gradient}.} We illustrate mild sharpening in Figure~\ref{fig:combined_figures}, 
where we plot sharpness in two settings: (i) regression with simple images and (ii) classification with an MLP using a subset of the CIFAR-10 dataset. 
\begin{wrapfigure}{l}{0.35\textwidth}
  \begin{center}
    \includegraphics[width=0.35\textwidth]{figures/intro/eos_nuance.pdf}
    \end{center}
    \caption{DLNs do not enter EOS regime if $L\sigma^{2-\frac{2}{L}}_{1}< 2/\eta$.}
    \label{fig:dln_mild_sharpening}
\end{wrapfigure}
For the regression task, we minimize the loss $\mathcal{L}(\Theta) = \|G(\Theta) - \mbf{y}_{\mathrm{image}}\|_2^2$, where $G(\Theta)$ is a UNet parameterized by $\Theta$, and $\mbf{y}_{\mathrm{image}}$ denotes one of the images in Figure~\ref{fig:img_used}. 
We observe that when $\mbf{y}_{\mathrm{image}}$ is a smooth, low-frequency image, the sharpness of the loss generally remains low. However, when $\mbf{y}_{\mathrm{image}}$ has higher frequency content, the sharpness increases and enters the EOS regime (Figure~\ref{fig:eos-dip}). Similarly, for the classification task, we train a 2-layer fully connected neural network on $N$ labeled training images from the CIFAR-10 dataset using MSE loss and plot the sharpness in Figure \ref{fig:small_Sharp}. The sharpness links to $N$, the number of data points used for training. For small $N$ values, such as 100 or 200, the network learns only a limited set of latent features, resulting in mild sharpening, and it does not reach the EOS threshold. However, when $N$ exceeds 1000, the sharpness increases and reaches the EOS threshold. \edit{The intrinsic dimension update in neural networks for such low complexity tasks is usually smaller \citep{li2018measuring} which could cause the sharpness to be small.}
\edit{Similar} observations can also be seen in DLNs. In Figure~\ref{fig:dln_mild_sharpening}, we show that the sharpness reaches $L\sigma_{\star, 1}^{2-\frac{2}{L}}$, where $\sigma_{\star, 1}$ is the singular value of the target matrix. Whenever $L\sigma_{\star, 1}^{2-\frac{2}{L}} < 2/\eta$, the network will not enter the EOS regime. This can be viewed as low-complexity learning, as $\sigma_{\star, 1}$ corresponds to the magnitude of the strongest feature of the target matrix. Hence, when $\sigma_{\star, 1}$ is not large enough, the sharpness will not rise to $2/\eta$. \edit{While these observations do not fully explain mild sharpening, our experiments demonstrate that interpreting sharpness as a measure of complexity, combined with our findings from DLNs, marks an important first step toward fully understanding this phenomenon.}


\paragraph{\edit{Difference in Oscillation Behaviors}.}

Here, we discuss the differences in oscillations that arise in DLNs compared to catapults that occur in practical deep nonlinear networks. 
The main difference lies in the loss landscape—at convergence, the Hessian for DLNs is positive semi-definite, as shown in Lemma~\ref{lemma:hessian_eigvals}, meaning there are only directions of positive curvature and flat directions (in the null space of the Hessian). 
In this landscape, oscillations occur because the basin walls bounce off, without
the direction of escape. 
However, in deep nonlinear networks, it has been frequently observed that the Hessian at the minima has negative eigenvalues \citep{ghorbani2019investigation, sagun2016eigenvalues}. This enables an escape direction along the negative curvature, preventing sustained oscillations. 
\begin{wrapfigure}{r}{0.57\textwidth}
    \centering
     \begin{subfigure}[t]{0.3\textwidth}
         \centering
        \includegraphics[width=\textwidth]{figures/holder1.png}
     \end{subfigure}
     \begin{subfigure}[t]{0.25\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/dln.png}
         %\caption*{Deep Linear Network}
     \end{subfigure}
     
    \caption{Loss landscape of the Holder table function and DLNs, respectively (left--right). The Holder table function is non-convex which allows catapulting to other minima, whereas DLNs do not have spurious local minima.}
    \label{fig:landscape}
\end{wrapfigure}
\edit{In Figure~\ref{fig:landscape}, we demonstrate these two differences by visualizing the loss landscapes and the iterates throughout GD marked in red. The Holder table function Figure~\ref{fig:landscape} (left) exhibits numerous local minima, causing the loss to exhibit a sharp ``catapult'' when a large learning rate is used. In contrast, for DLNs (shown in the right) the loss oscillates in a periodic orbit around the minima since there are no spurious local minima \citep{ge2016matrix,kawaguchi2016deep,lu2017depth,zhang2019depth,yun2018small}. 
%In Appendix~\ref{sec:extra_details}, we provide experimental details.
}


Lastly,~\cite{damian2023selfstabilization} studies self-stabilization, where sharpness decreases below $2/\eta$ after initially exceeding $2/\eta$. \edit{Their analysis requires assumptions such as  $\nabla L(\theta) \cdot u(\theta) = 0$ and $\nabla S(\theta)$ lies in the null space of the Hessian, where $S(\theta)$ and $u(\theta)$ denotes the sharpness and its corresponding eigenvector respectively. These assumptions do not hold exactly in DLNs. Rather, the sharpness oscillates about $2/\eta$ as shown in Figure~\ref{fig:ps_eos} as the condition for stable oscillation holds along each eigenvector of the Hessian.}


\begin{comment}
\subsection{Explaining Sharpening Phenomenon in Deep Nonlinear Network}
\label{sec:unexplained_exp}

Based on our analysis, we draw parallels to two common observation in deep non-linear networks:\\

1) \textbf{Mild Sharpening in low complexity tasks:} The extent of sharpening in deep neural networks is often related to the complexity of the learning task. To illustrate this, we consider two commonly used tasks: regression and classification.\\
\textit{Regression Task}: In Figure \ref{fig:eos-dip}, we minimize the loss function $L(\boldsymbol{\theta})= \| G(\boldsymbol{\theta}) - \mbf{y}_{im} \|_{2}^2$, fitting an image $\mbf{y}_{im}$ using a deep image generator network like Unet $G(\boldsymbol{\theta})$, with Gradient Descent. We observe that the degree of sharpening in this network depends on the target image $\mbf{y}_{im}$. For example, when $\mbf{y}_{im}$ is a smooth, low-frequency image, the sharpness of the loss $ \| \nabla^2 L(\boldsymbol{\theta}) \|_{2}$ remains low. In contrast, when fitting a detailed image, such as white noise with high-frequency content, the sharpness increases and enters the EOS regime $\frac{2}{\eta}$. In particular,we observe a steady correlation between the sharpness rise (Figure-\ref{fig:eos-dip}) and the high frequency content of the fitting image (Figure-\ref{fig:img_used}). \\
\textit{Classification task}:  In Figure \ref{fig:small_Sharp}, we train a 2-layer fully connected neural network on $N$ pairs of labeled training images from the CIFAR-10 dataset using MSE loss. The sharpness of the loss is linked to $N$, the number of data points used for training. For small $N$ values, such as 100 or 200, the network learns only a limited set of latent features, resulting in mild sharpening, and the network does not reach the EOS threshold. However, when $N$ exceeds 1000, the sharpness increases and reaches the EOS threshold $\frac{2}{\eta}$. Furthermore, Figure-16 in \cite{cohen2021gradient} reported that sharpness also increases with depth of the network. So, the sharpness limit correlates both with network depth and complexity of the learning problem. \\
These two occurences in non-linear network is partially addressed by our analysis of deep matrix factorization at EOS. We show that sharpness rises to $L\sigma^{2-\frac{2}{L}}_{1}$, where $\sigma_{1}$ is the top singular value of the target matrix and $L$ is the depth. In deep matrix factorization problem, $\sigma_{1}$ corresponds to the magnitude of the strongest feature in the data and is related to the complexity of learning. Whenever, $L\sigma^{2-\frac{2}{L}}_{1}<\frac{2}{\eta}$, the network do not enter the EOS regime (Figure-\ref{fig:dln_mild_sharpening}). Similarly, in both regression and classification experiments in Figure \ref{fig:combined_figures}, whenever data has low complexity, sharpness do not rises and network fails to reach EOS. Furthermore, sharpness $L\sigma^{2-\frac{2}{L}}_{1}$ scales with depth of the network $L$, supporting the observation by \cite{cohen2021gradient}.

2) \textbf{Oscillation range in strong feature direction:}
\end{comment}

\begin{figure}[t!]    
\centering
    \begin{subfigure}[t]{0.32\textwidth} % Subfigure (a) - increased size
        \centering
        \includegraphics[width=\textwidth]{figures/dip_eos/eos.pdf}
        \caption{Sharpness plots for training image generator networks using SGD with learning rate $\eta = 2\times 10^{-4}$.}
        \label{fig:eos-dip}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.32\textwidth} % Subfigure (b) - increased size
        \centering
        \includegraphics[width=\textwidth]{figures/dip_eos/img_used.pdf}
        \caption{Target images (denoted as $\mbf{y}_{\mathrm{image}}$) with different frequencies used for training.}
        \label{fig:img_used}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.32\textwidth} % Subfigure (c) - increased size
        \centering
        \includegraphics[width=\textwidth]{figures/small_sharpness.png}
        \caption{2-layer FC network trained with small number $N$ of CIFAR-10 dataset with $\eta=10^{-2}$}
        \label{fig:small_Sharp}
    \end{subfigure}
    \caption{Illustration of Caveat 2 by~\cite{cohen2021gradient} on how mild sharpening occurs on simple datasets and network. (a) Regression task showing the evolution of the sharpness when an UNet (with fixed initialization) is trained to fit a single image shown in (b). (c) Evolution of the minimal progressive sharpening on a classification task of a 2-layer MLP trained on a  subset of CIFAR-10.}
    \label{fig:combined_figures}
\end{figure}

\begin{comment}

\subsection{Difference of EOS dynamics in non-linear networks and deep matrix factorization }

Although mild sharpening and strong directional oscillation phenomenon is partially explained from analyzing deep matrix factorization, we highlight some critical differences between EOS dynamics in non-linear networks and liner networks:

\begin{itemize}
    \item \textbf{Sustained oscillation in DMFs vs catapaults in non-linear networks}: In deep matrix factorization (DMF) loss whenever $\eta > \frac{2}{L \sigma_{1}^{2-\frac{2}{L}}}$, we observe free oscillation in 2-period orbit \footnote{At higher learning rate, iterates enter higher period orbit oscillations, chaos and divergence}. However, in nonlinear networks we observe catapaults or sudden spikes. This is primarily because of difference in loss landscape. At global minima, Hessian of the loss in DMF is provably Positive Semi-Definite (PSD)\footnote{we explicitly derived all positive eigenvalues}. So there are only directions of positive curvature and flat directions (in null space of the Hessian). In this landscape,\textit{ oscillations occur due to bouncing of the basin of the wall with no direction of escape.} But in deep non-linear networks, it is has been frequently observed that the Hessian at the minima has negative eigenvalues \cite{ghorbani2019investigation,sagun2016eigenvalues}. This enables an escape direction in the direction of the negative curvature preventing sustained/free oscillation. We believe understanding the role of non-linear activation layers in changing this loss landscape is the key to address this difference.
    \item \textbf{Absence of self-stabilization effect \cite{damian2023selfstabilization} in deep matrix factorization}
    Damian et al. studied self-stabilization, where sharpness decreases below $\frac{2}{\eta}$ after exceeding $\frac{2}{\eta}$. They assume that $\nabla L(\theta) \cdot u(\theta) = 0$ and $\nabla S(\theta)$ lie in the null-space of the Hessian. However, in deep linear networks, \textit{these assumptions are not satisfied}. Due to singular vector alignment and balancing, the dynamics reduce to a one-dimensional oscillating trajectory, where both $\nabla L(\theta)$ and $\nabla S(\theta)$ lie in the range space of the Hessian. Letting $\pi(\theta)$ represent the scalar product, $\nabla L(\theta) \cdot u(\theta) = (\pi(\theta) - s)\pi(\theta)|w^{-1}|$, which isn't zero unless the loss is zero (not the case in EoS). Hence, in deep linear networks, self-stabilization does not occur, and the iterates and sharpness oscillate above $\frac{2}{\eta}$.

\end{itemize}
\end{comment}
\section{Conclusion, Limitations and Future Work}

In this paper, we presented a fine-grained analysis of the learning dynamics of deep matrix factorization with the aim of understanding unexplained phenomena in deep nonlinear networks within the EOS regime. Our analysis revealed that within EOS, DLNs exhibit periodic oscillations in small subspaces, where the subspace dimension is exactly characterized by the learning rate. 
%This allowed us to explain phenomena such as mild sharpening, oscillations occurring only within the top singular values, and to distinguish the differences between the behaviors of DLNs and diagonal linear networks. 
There are two limitations to our work:  we require (i) the dynamics converge to the singular vector stationary set, and (ii) strict balancing of the singular values. 
However, we provide thorough empirical evidence validating the use of these assumptions, along with more results in Appendix~\ref{sec:additional_exp}.
For the balancing assumption, we leave for future work on alleviating the assumption of strict balancing, and rigorously show that this holds before entering the EOS regime.


%there may exist cases where oscillations begin before strict balance is achieved. We leave it to future work to find subspace oscillations without assuming strict balancing before oscillation starts.


==> ICLR/text/intro.tex <==
\section{Introduction}

Understanding generalization in deep neural networks requires an understanding of the optimization process in gradient descent (GD).
In the literature, it has been empirically observed that the learning rate $\eta$ plays a key role in driving generalization~\citep{hayou2024lora,lewkowycz2020large}. The ``descent lemma'' from classical optimization theory says that for a $\beta$-smooth loss $\mathcal{L}(\mathbf{\Theta})$ parameterized by $\mathbf{\Theta}$, gradient descent (GD) iterates satisfy
\begin{align*}
    \mathcal{L}(\mathbf{\Theta}(t+1)) \leq \mathcal{L}(\mathbf{\Theta}(t)) - \frac{\eta(2-\eta \beta)}{2} \|  \nabla \mathcal{L}(\mathbf{\Theta}(t)) \|_{2}^2,
\end{align*}
and so the learning rate should be chosen as $\eta < 2/\beta$ to monotonically decrease the loss.
%However, classical optimization theory on GD restricts itself to small infinitesimal learning rate and unrealistic convergence assumptions which barely holds for training deep networks in practice. Traditional analysis of GD show that for $L$-smooth loss, only if the step-size $\eta$ is selected to be less than $\frac{2}{L}$, the training is stable and the loss decreases monotonically.
However, many recent works have shown that the training loss decreases even for $\eta > 2/\beta$, albeit non-monotonically.
Surprisingly, it has been observed that choosing such a learning rate often provides better generalization over smaller ones that lie within the stability threshold. This observation has led to a series of works analyzing the behavior of GD within a regime dubbed ``the edge of stability'' (EOS). By letting $\mbf{\Theta}$ be a deep network, we formally define EOS as follows:
%Consider GD is run with learning rate $\eta$ to minimize a loss $l(\mbf{\theta})$ with a deep network. \cite{cohen2021gradient} observed a surprising and a commonly occuring phenomenon in deep networks coined "Edge of Stability" which is formally defined:
\begin{definition}[Edge of Stability~\citep{cohen2021gradient}]
During training, the sharpness of the loss, defined as $S(\mbf{\Theta}):= \| \nabla^2 \mathcal{L}(\mbf{\Theta})\|_{2}$, continues to grow until it reaches $2/\eta$ (progressive sharpening), after which it stabilizes around $2/\eta$. During this process, the training loss behaves non-monotonically over short timescales but consistently decreases over long timescales.
\end{definition}

Using a large learning rate to operate within the EOS regime is hypothesized to give better generalization performance by inducing ``catapults'' in the training loss~\citep{zhu2023catapults}. Intuitively, whenever the sharpness $S(\mbf{\Theta})$ exceeds the local stability limit $2/\eta$, the GD iterates momentarily diverge (or catapults) out of a sharp region and self-stabilizes~\citep{damian2023selfstabilization} to settle for a flatter region where the sharpness is below $2/\eta$, which has shown to correlate with better generalization~\citep{keskar2017on, izmailov2019averaging, petzka2021relative, foret2021sharpnessaware, gatmiry2023inductive}. Of course, the dynamics within EOS differ based on the loss landscape. 
%For example, as illustrated in Figure~\ref{fig:catapults_vs_osc}, 
When the loss landscape is highly non-convex with many local valleys, catapults may occur, whereas sustained oscillations may exist for other landscapes. It is of great interest to understand these behaviors within different network architectures to further our understanding of EOS.
%and how these behaviors can lead to better generalization.

From a theoretical perspective, there have been many recent efforts to understand EOS. These works generally focus on analyzing ``simple'' functions, examples including scalar losses \citep{minimal_eos,wang2023good,kreisler2023gradient}, quadratic regression models \citep{agarwala2022second}, diagonal linear networks \citep{even2024s} and two-layer matrix factorization \citep{chen2023edge}. 
However, the simplicity of these functions cannot fully capture the behaviors of deep neural networks within the EOS regime. Specifically, the following observations remain unexplained by existing analyses: (i) mild (or no) sharpening occurs when either networks are shallow or ``simple'' datasets are used for training~(Caveat 2 from~\citep{cohen2021gradient}); and (ii) \edit{the oscillations and catapults in the training loss occur in the span of the top eigenvectors of the NTK}~\citep{zhu2023catapults}.
%(i) mild (or no) sharpening occurs when deep networks are trained using ``simple'' datasets~(Caveat 2 from~\citep{cohen2021gradient}); (ii) the oscillations and catapults in the weights occur within a low-rank subspace or within the top singular values of each weight matrix~\citep{zhu2024catapultssgdspikestraining}; and (iii) the oscillations are stronger within weight subspaces that generate more prominent features in the output fitting the data. For example, \cite{zhu2024catapultssgdspikestraining} observed that large catapults occurred within the top eigenspace of the NTK, followed by mild (or no) catapults in the complementary space, and \cite{rosenfeld2024outliers} showed that network inputs with large-magnitude features and strong opposing signals oscillate with larger spikes for those particular inputs.%
%\qq{need to discuss the limitation of previous results, especially for the last part} \smk{actually the limitation is that they cannot explain the phenomena}


\begin{comment}
    
These works developed our understanding of EOS but are far from capturing EOS dynamics occuring in deep neural networks. The formulation of deep neural networks is very close to deep matrix factorization problem which only exempts the use of non-linear activations and with a practical assumption that the underlying data is low rank. However, existing literature in deep matrix factorization focused on gradient flow dynamics \cite{arora2019implicit,saxe2014exact} or GD operating in the stable regime \cite{chou2024gradient,gidel} where training loss decreases monotoncally. We enlist important observations made while training deep network in the EOS regime which are currently unexplained by existing analysis in the literature:

\begin{enumerate}
\item  (Obs-1:) \textbf{Mild-sharpening} or no sharpening occurs 1) when deep networks are trained to fit \textit{simple} datasets (Caveat-2 \cite{cohen2021gradient}) (refer Figure) or 2) when the depth of the network is small.  % 
\item (Obs-2:) \textbf{Subspace Oscillation}: Oscillation/catapaults in the weight space occurs in a low rank subspace or within the top few sinuglar values of weight matrix in each layer \cite{zhu2024catapultssgdspikestraining}, hence preserving \textit{structure amidst chaos}.%
\item (Obs-3:) \textbf{Stronger oscillations} occur along weight subspace that generates prominent features in the output fitting the data. \cite{zhu2024catapultssgdspikestraining} observed that large catapaults occured in the top eigenspace of the NTK followed by mild/no catapaults in complementary space. \cite{rosenfeld2024outliers} showed that network inputs with large magnitude features and strong opposing signals oscillate with larger spikes for that particular input. %
\end{enumerate}

Our analysis of EOS on deep matrix factorization aims at explaining these 3 key observations and thereby attempting to bridge the gap between theory and practice. But before understanding EOS dynamics, it is important to understand gradient flow dynamics in deep matrix factorization. 

\begin{figure}[t!]
    \centering
     \begin{subfigure}[b]{0.2475\textwidth}
         \centering
        \includegraphics[width=\textwidth]{figures/intro/dln_train_loss.pdf}
        \caption{Linear Networks}
     \end{subfigure}
     \begin{subfigure}[b]{0.2475\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/intro/mlp_train_loss.pdf}
         \caption{ReLU Networks}
     \end{subfigure}
        \begin{subfigure}[b]{0.475\textwidth}
         \centering
         \includegraphics[width=0.95\textwidth]{figures/intro/lora_osc.pdf}
         \caption{BERT using LoRA}
     \end{subfigure}
     \vspace{-0.1in}
    \caption{Illustration of instability in the training loss for different network architectures. When the loss landscape is more complex with many local valleys (b, c), catapults occur, whereas free/sustained oscillation occur in (a). Parts with oscillations/catapults are zoomed in.}
    
    \label{fig:catapults_vs_osc}
\end{figure}

\end{comment}

\begin{figure}[t!]
    \centering
     \begin{subfigure}[t!]{0.49\textwidth}
         \centering
        \includegraphics[width=\textwidth]{figures/sval_bifur.pdf}
     \caption*{Singular Values of Weights}
     \end{subfigure}
     \begin{subfigure}[t!]{0.49\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/hess_bifur.pdf}
         \caption*{Eigenvalues of Hessian}
     \end{subfigure}
    \caption{Bifurcation plot of the oscillations in the singular values (left) and the eigenvalues of the Hessian (right) of a 3-layer end-to-end DLN. The bifurcation plots indicate the existence of a period-doubling route to chaos in DLNs, which we analyze by examining the two-period orbit. %\edit{Here, $\beta =L \sigma^{2-\frac{2}{L}}_{1}(\mbf{M}_\star) $ and $\eta > 2/\beta$ corresponds to the EOS regime where $\sigma_{1}(\mbf{M}_\star)$ denotes the largest singular value of target matrix $\mbf{M}_\star$.}
    Here, $\eta > 2/\beta$ corresponds to the EOS regime, where $\beta = L\sigma_{\star, 1}^{2 - 2/L}$ is the sharpness at the minima, $L$ is the depth of the network and $\sigma_{\star, 1}$ is the first singular value of the target matrix $\mbf{M}_\star$.
    }
    
    \label{fig:bifurcation}
\end{figure}

%In this work, we attempt to bridge the gap between theory and practice by providing a fine-grained analysis of the learning dynamics of deep linear networks (DLNs) within the EOS regime. DLNs share many characteristics with their nonlinear counterparts, making them a useful surrogate for analyzing behaviors in deep neural networks~\citep{wang2024understandingdeeprepresentationlearning, zhang2024when}. For example,~\cite{zhang2024when} has provably shown that bias-free ReLU networks behave similarly to linear networks.
%Generally, existing works on DLNs focus on analyzing the effect of depth and the initialization scale, and how they implicitly bias the trajectory of gradient flow towards low-rank solutions when the learning rate is chosen to be stable~\citep{saxe2014exact, arora2018optimization, implicit_dmf, zhang2024structure, pesme2023saddle, jacot2022saddletosaddle}.
In this work, we present a fine-grained analysis of the learning dynamics of deep linear networks (DLNs) within the EOS regime, demonstrating that these phenomena can be replicated and effectively explained using DLNs. Generally, there are two lines of work for DLNs: (i) those that analyze the effects of depth and initialization scale, and how they implicitly bias the trajectory of gradient flow towards low-rank solutions when the learning rate is chosen to be stable~\citep{saxe2014exact, arora2018optimization, implicit_dmf, you2020robust, liu2022robust, zhang2024structure, pesme2023saddle, jacot2022saddletosaddle}, and (ii) those that analyze the similarities in behavior between linear and nonlinear networks~\citep{wang2024understandingdeeprepresentationlearning, zhang2024when,yaras2023law}.
Our analysis builds upon these works to show that DLNs exhibit intricate and interesting behaviors outside the stability regime and to demonstrate how factors such as depth and initialization scale contribute to the EOS regime. Our main contributions can be summarized as follows: \qq{the bolded sentences below do not capture the key contributions. It needs to be rephrased.}
%particularly periodic oscillations within a small subspace, where the subspace dimension is precisely characterized by the step size. 
%\qq{need a short title for each bullet point}

\begin{itemize}
\item \textbf{Oscillations in Top Subspaces.} We show that there exist periodic oscillations within $r$-dimensional subspaces in DLNs, where $r$ is precisely characterized by the learning rate. For DLNs, a period-doubling route to chaos~\citep{Ott_2002} exists in both the singular values of the DLN and the eigenvalues of the Hessian, as shown in Figure~\ref{fig:bifurcation}. We rigorously characterize the case of the two-period orbit, aiming to contribute to explaining the empirical observations by~\cite{zhu2023catapults} and~\cite{cohen2021gradient}. We also prove that the learning rate needed to enter EOS is a function of the network depth, further revealing its role in deep networks.
\item \textbf{DLNs vs. Diagonal Linear Networks.} 
\edit{We prove that while DLNs and diagonal linear networks have different curvatures about the global minimum, they exhibit similar behaviors within the EOS regime.
We show that the additional eigendirections present in DLNs are not explored during training, making the behavior of the two networks synonymous.}
\end{itemize}

\begin{comment}
    
\subsection{Implicit regularization in deep linear models with gradient flow}
Over the past few years, several works have analyzed the effect of depth and initialization in deep linear networks \cite{saxe2014exact, arora2018optimization, implicit_dmf, zhang2024structure}. It has been observed that small initialization and larger depth make the trajectory of gradient flow implicitly biased towards low-rank solutions. Similar observations have been made in diagonal linear networks \cite{woodworth2020kernel, pesme2021implicit}, where the scale of initialization determines whether the dynamics of the iterates are in the rich regime or the kernel regime. Smaller initialization promotes rich regime dynamics, where features are learned incrementally through saddle-to-saddle dynamics \cite{pesme2023saddle, jacot2022saddletosaddle}. Larger depth increases the duration of these saddle points and has a stronger implicit bias towards exact low-rank solutions by suppressing the residual singular values through the depth factor \cite{arora2018optimization}. In deep matrix factorization gradient flow aligns the singular vectors of successive layer factors \cite{du2018algorithmic}. 

Due to this alignment, the flow dynamics in deep matrix factorization are the same as those in deep linear networks, but act on the singular values of the matrices.

Our analysis and experiments reveal certain surprising (yet explainable) phenoemons that is critical to understand Edge of Stability:

\begin{itemize}
    \item  The dynamics in deep matrix factorization and diagonal linear networks (or even tensor factorization) differ in the EOS regime, unlike in gradient flow (GF). These dynamics depend on the dimensionality of the layers (whether vector in diagonal linear networks, matrix in deep matrix factorization, or tensor in tensor factorization), which is not the case in GF.
    \item  We prove that in deep linear networks, only the depth and the largest singular value of the target matrix determine whether the network will operate in the EOS regime.
    \item The condition to enter the EOS regime is independent of the initialization scale and the dimensionality of the layers, dimension the rank of the target matrix. 
\end{itemize}


\ag{I am unsure whether it is better to state it after notations otherwise it will be a reptitition. Probably we should state this in the contribution section?}


\end{comment}





%\paragraph{Related Works.} We briefly survey a few related works to highlight their differences, and provide a detailed discussion in \Cref{app:related}. 
%    DLNs are often used as prototypes to study the behaviors of nonlinear networks~\citep{benign, saxe2014exact, wang2024understanding, nc}. The most relevant literature on DLNs are those by Yaras et al.~\citep{yaras2023law, yaras2024compressible} and Kwon et al.~\citep{kwon}, who reveal that the weight updates of deep networks occur within an invariant subspace. Our work differs from that of Yaras et al.~\citep{yaras2023law} in that we fully capture the learning dynamics of DLNs throughout the entire GD process. While Kwon et al.~\citep{kwon} observe invariant weight updates, they use this observation for model compression and do not study the learning dynamics with large learning rates. Regarding the edge of stability, the most relevant works are those that analyze scalar functions to demonstrate that the edge of stability occurs on such functions, which have a non-zero third-order derivative and satisfy certain regularity conditions~\citep{chen2023edge,wang2023good,minimal_eos}. However, as mentioned previously, these works do not capture the more complicated models that we consider in this work.


\section{Notation and Problem Setup}

%\qq{we need to be consistent, some place we call it deep linear networks, other places we call it deep matrix factorization. Let us call it "deep linear network", and training loss for DLN}

\paragraph{Notation.}
We denote vectors with bold lower-case letters (e.g., $\mbf{x}$)
and matrices with bold upper-case letters (e.g., $\mbf{X}$).
%Given any $n \in \N$,
We use $\mbf{I}_n$ to denote an identity matrix of size $n \in \N$.
We use $[L]$ to denote the set $\{1, 2, \ldots, L\}$. 
We use the notation $\sigma_i(\mbf{A})$ to denote the $i$-th singular value of the matrix $\mbf{A}$. We also use the notation $\sigma_{\ell, i}$ to denote the $i$-th singular value of the matrix $\mbf{W}_\ell$.

\begin{comment}
\paragraph{Deep linear model}
Consider the problem of least squares fitting problem with multidimensional output. We want to learn a mapping $f(.):\mbb{R}^{d}\rightarrow \mbb{R}^{d}  $ given $d$ number of input vectors $\mbf{x}_{i} \in \mbb{R}^{d}$ to same number of target vector $\mbf{y}_{i} \in \mbb{R}^{d}$. Considering $f(.)$ to be deep linear model with set of parameters  $\mbf{\Theta} = \left(\mbf{W}_1, \mbf{W}_2, \ldots, \mbf{W}_L \right)$, then the fitting regression problem can be formulated as minimizing the loss wrt $\frac{1}{2} \|\mbf{Y} - \mbf{X} \mbf{W}_L \cdot \ldots \cdot \mbf{W}_1\|^2_{F} $ where $\mbf{X}$ and $\mbf{Y}$ are column stacking of the input  $\left\{\mathbf{x}_{i}\right\}_{i=1}^d$ and target $ \left\{\mathbf{y}_{i}\right\}_{i=1}^d$. Assuming the data matrix $\mbf{X}$ to be whitened matrix with dominant features such that $\mbf{X}^T \mbf{Y} = \mbf{M}$ (say) is low rank, then the optimization can be formulated as a low rank recovery problem. Throughout the paper, we will restrict ourselves to analyze the deep matrix factorization problem, which we introduce next.
\end{comment}


 \paragraph{Deep Matrix Factorization Loss.} \qq{needs to explain why we choose to study based upon deep matrix factorization. We also need to be consistent when we refer to deep matrix factorization, or DLNs.}
The objective in deep matrix factorization is to model a low-rank matrix $\mbf{M}_\star \in \mbb{R}^{d\times d}$ with $\rank(\mbf{M}_\star) = r$ via a DLN parameterized by a set of parameters $\mbf{\Theta} = \left(\mbf{W}_1, \mbf{W}_2, \ldots, \mbf{W}_L \right)$, which can be estimated by solving
\begin{align}\label{eqn:deep_mf}
    \underset{\mbf{\Theta}}{\rm{arg min}} \, f(\mbf{\Theta}) \coloneqq \frac{1}{2}\|\underbrace{\mbf{W}_L \cdot \ldots \cdot \mbf{W}_1}_{\eqqcolon \mbf{W}_{L:1}} - \mbf{M}_\star\|^2_{\mathsf{F}},
\end{align}
where we adopt the abbreviation $\mbf{W}_{j:i} = \mbf{W}_{j}\cdot \ldots \cdot \mbf{W}_i$ to denote the end-to-end DLN and is identity when $j < i$. We assume that each weight matrix has dimensions $\mbf{W}_\ell \in \mbb{R}^{d\times d}$ to observe the effects of overparameterization. We also assume that the singular values of $\mbf{M}_\star$ are distinct.
%such that $\sigma_{\star, 1} > \ldots > \sigma_{\star, r}$.





\paragraph{Optimization.}
We update each weight matrix $\mbf W_\ell \in \mbb{R}^{d\times d}$ using GD with iterations given by
\begin{align}\label{eqn:gd}
    \mbf{W}_\ell(t) = \mbf{W}_\ell(t-1) - \eta\cdot \nabla_{\mbf{W}_\ell}f(\mbf{\Theta}(t-1)), \quad \forall \ell \in [L],
\end{align}
where $\eta > 0$ is the learning rate and $\nabla_{\mbf{W}_\ell}f(\mbf{\Theta}(t))$ is the gradient of $f(\mbf{\Theta})$ with respect to the $\ell$-th weight matrix at the $t$-th GD iterate. 



\begin{figure}[t!]
    \centering
    \includegraphics[width=\textwidth]{figures/dln_ps_eos_lr172_new.pdf}
    \caption{Depiction of the two phases of learning in the deep matrix factorization problem for a network of depth $3$. It appears that upon escaping the first saddle point, the GD iterates enter the EOS regime, where the sharpness hovers just above $2/\eta$. \qq{add two subcaptions}
    }
    \label{fig:ps_eos}
\end{figure}



\paragraph{Initialization.}

In this work, we consider both balanced and unbalanced initializations, respectively:
\begin{align}\label{eqn:init}
 \mbf{W}_\ell(0) = \alpha \mbf{I}_d, \quad \forall \ell \in [L], \quad \text{and} \quad\mbf{W}_L(0) = \mbf{0},  \quad \mbf{W}_\ell(0) = \alpha \mbf{I}_d, \quad \forall \ell \in [L-1],
\end{align}
where $\alpha > 0$ is a small constant. We assume $\alpha$ is chosen small enough such that $\alpha \in (0, \sigma_{\star, r})$, where $\sigma_{\star, r}$ is the $r$-th singular value of $\mbf{M}_\star$. Generally, many existing works on both shallow and deep linear networks assume a zero-balanced initialization (i.e., $\mbf{W}_i^\top(0)\mbf{W}_i(0) = \mbf{W}_j(0)\mbf{W}^\top_j(0)$ for $i \neq j$). This introduces the invariant $\mbf{W}_i^\top(t)\mbf{W}_i(t) = \mbf{W}_j(t)\mbf{W}^\top_j(t)$ for all $t > 0$, ensuring two (degenerate) conditions throughout the training trajectory: (i) the singular vectors of each of the layers remain aligned and (ii) the singular values stay balanced.
For the unbalanced initialization, the zero weight layer can be viewed as the limiting case of initializing the weights with a (very) small constant $\alpha' \ll \alpha$, and has been similarly explored by~\cite{two_layer_bias,xu2024provable}, albeit for two-layer networks. 
The zero weight layer relieves the balancing condition of the singular values.
Rather than staying balanced, we show that the singular values become increasingly balanced (see Lemma~\ref{lemma:balancing}). This allows us to jointly analyze the singular values of the weights for either case.

Nevertheless, we also show that our analysis is not limited to either initialization but applies to \emph{any initialization} that converges to a set we call the singular vector stationary set (see Proposition~\ref{prop:svs_set}).To the best of our knowledge, it is common to assume that the singular vectors remain aligned, as many existing works make the same assumption~\citep{two_layer_bias, implicit_dmf, saxe2014exact, gidel,chou2024gradient, kwon}. 



%In the following section (as well as Appendix~\ref{sec:additional_exp}), we provide examples of such initializations, which we adopt for our analyses as well.



%\smk{I am pretty adamant that we should have this section like this; it has clear motivation.} \ag{Slightly debatable, but let's hear opinions of others. }
%\ag{@Qing: would it be better if we specify the general class of initialization instead of the zero-one initilaization in the main text?}\smk{Note that we never prove that any initialization belongs in the SVS set! And we need to then change all of our proofs to be $\mbf{Q}$ orthogonal matrices rather than the target matrix $\mbf{V}$ like we have now.}
 % For deep linear networks, it is common to use an orthogonal-type initialization rather than a random one~\citep{kwon, kwon2024on, yaras2023law}, as it has been provably shown that random initialization slows down convergence~\citep{Hu2020Provable}.

==> ICLR/text/theory.tex <==
 \section{Deep Matrix Factorization Beyond the Edge of Stability}



When using a large learning rate, the learning dynamics can typically be separated into two distinct stages: (i) progressive sharpening and (ii) the edge of stability. Within the progressive sharpening stage, the sharpness lies below $2/\eta$ and tends to continually rise.  Our goal is to analyze the EOS stage under the deep matrix factorization formulation. Here, we observe that the training loss fluctuates due to layerwise singular value oscillations, as illustrated in Figure~\ref{fig:ps_eos}.

%Here, we observe that the training loss oscillates in a two-period orbit rather than decreasing over iterations, as illustrated in Figure~\ref{fig:ps_eos} and rigorously shown in the following sections.


\begin{figure}[t!]
    \centering
    \includegraphics[width=\textwidth]{figures/svector_alignment_diff_lr.png}
    \caption{Illustrations of the singular vector and value evolution of the end-to-end DLN. The singular vectors of the network remain static across all iterations, as suggested by the singular vector stationary set, regardless of the learning rate. The angle between the true singular vectors and those of the network remains aligned throughout. The first singular values undergo oscillations in the large $\eta$ regime, whereas they remain constant in the small $\eta$ regime.}
    \label{fig:svec_alignment}
\end{figure}

\subsection{Main Results}


Before we present our main results, we provide a definition of what we refer to as a strict balanced state of the singular values of the weight matrices. The parameters are said to be in a strict balanced state if the singular values of each weight matrix take the same values across all layers.

\begin{definition}[Strict Balanced State]
The parameters $\mbf{\Theta}$ of the DLN from Equation~(\ref{eqn:deep_mf}) are said to be in a strict balanced state if for some $t\geq 0$
    \begin{align*}
        \sigma_i(\mbf{W}_\ell(t)) = \sigma_i(\mbf{W}_k(t)), \quad  \forall i \in [r], \quad \forall \ell, k \in [L],
    \end{align*}
    where $\sigma_{i}(\mbf{W}_{\ell})$ denotes the $i$-th singular value of the $\ell$-th layer and $r$ is the rank of the matrix $\mbf{M}_\star$.
\end{definition}

It is straightforward to show that the parameters are in a strictly balanced state for all $t\geq 0$ if we initialize the singular values to be the same across all weight matrices $\mbf{W}_\ell$. Hence, it immediately holds that the balanced initialization is in a strictly balanced state. However, the one-zero initialization in Equation~(\ref{eqn:init}) sets the singular values of $\mbf{W}_L$ to zero, meaning the parameters are not initially in a strictly balanced state.
However, in Lemma~\ref{lemma:balancing} of Section~\ref{sec:used_tools}, we prove that the balancing increasingly occurs throughout GD iterations within the EOS regime. Consequently, we assume a strictly balanced state for the remainder of this paper and analyze the EOS regime in relation to the balanced minimum.
Next, we derive the eigenvalues of the Hessian at convergence, such that we can identify the learning rate needed to enter the EOS regime for DLNs.

\begin{lemma}[Eigenvalues of Hessian at the Balanced Minimum]
\label{lemma:hessian_eigvals}
    Consider running GD on the deep matrix factorization loss $f(\mbf{\Theta})$ defined in Equation~(\ref{eqn:deep_mf}). The \edit{set of all} non-zero eigenvalues of the training loss Hessian \emph{at the balanced minimum} is given by
    \begin{align*}
       \lambda_{\mbf{\Theta}} = \underbrace{\left\{L \sigma_{\star, i}^{2 - \frac{2}{L}}, \sigma_{\star, i}^{2 - \frac{2}{L}}\right\}_{i=1}^r }_{\text{self-interaction}} \, \bigcup \, \underbrace{\left\{\sum_{\ell=0}^{L-1} \left(\sigma_{\star, i}^{1-\frac{1}{L} - \frac{1}{L}\ell} \cdot \sigma_{\star, j}^{\frac{1}{L}\ell}\right)^2\right\}_{i\neq j}^{r}}_{\text{interaction with other singular values}} \,\bigcup \, \underbrace{\left\{\sum_{\ell=0}^{L-1} \left(\sigma_{\star, k}^{1-\frac{1}{L} - \frac{1}{L}\ell} \cdot \alpha^{\ell}\right)^2\right\}_{k = 1}^{r}}_{\text{interaction with initialization}} 
    \end{align*}
    where $\sigma_{\star, i}$ is the $i$-th singular value of the target matrix $\mbf{M}_\star \in \mbb{R}^{d\times d}$,  $\alpha \in \mbb{R}$ is the initialization scale, $L$ is the depth of the network, and the second element of the set under ``self-interaction'' has a multiplicity of $d-r$.
\end{lemma}


We defer all of the proofs to Appendix~\ref{sec:proofs}.
Let $\lambda_i$ denote the $i$-th largest eigenvalue of the Hessian. 
By Lemma~\ref{lemma:hessian_eigvals}, we observe that the sharpness is equal to $\lambda_1 = \|\nabla^2 f(\mbf{\Theta})\|_2 = L\sigma_{\star, 1}^{2- \frac{2}{L}}$ at the balanced minimum. \edit{In Lemma~\ref{lemma:flattest}, we show that the sharpness at the balanced minimum is the flattest, and hence $L\sigma_{\star, 1}^{2 - \frac{2}{L}}$ represents the smallest sharpness value among all global minima.
Thus, if $\eta$ is set such that $\eta > 2/\lambda_1$, oscillations in the loss will occur, as the step size is large enough to induce oscillations even in the flattest region.}   Interestingly, notice that all non-zero eigenvalues are a function of network depth. For a deeper network, the sharpness will be larger, implying that a smaller learning rate can be used to drive the DLN into EOS. This provides a unique perspective on how the learning rate should be chosen as networks become deeper and explains the observation made by~\cite{cohen2021gradient}, who observed that sharpness scales with the depth of the network.
Equipped with the eigenvalues, we show in the following result that oscillations occur in a two-period orbit along the $i$-th eigenvector direction, given that the learning rate is set to be greater than $2/\lambda_i$.

\begin{theorem}[Stable Subspace Oscillations]
\label{thm:stable_oscillations}
Let $\alpha' \coloneqq \left( \ln\left( \frac{2\sqrt{2}}{\eta \lambda_1} \right) \cdot \frac{ \sigma_{\star, 1}^{4/L}}{L^2 \cdot 2^{\frac{2L-3}{L}}} \right)^{1/4}$.
Consider running GD on the loss in~(\ref{eqn:deep_mf}) with initialization scale $0<\alpha < \alpha'$.
    If $\eta = \frac{2}{K}$ with $\lambda_i \leq K< \lambda_{i+1}$, then $2$-period orbit oscillation occurs in the direction of $\Delta_i$, where $\lambda_i$ and $\Delta_i$ denote the $i$-th largest eigenvalue and  eigenvector of the Hessian at the balanced minimum, respectively.
\end{theorem}


The complete proof is provided in Appendix~\ref{sec:proofs_oscillations}, where we derive all eigenvectors at the balanced minimum and demonstrate that the necessary conditions from Lemma~\ref{lemma:chen-bruna} (restated from~\cite{chen2023edge}) are satisfied for a two-period orbit. The condition on the initialization scale is chosen to ensure balanced behavior, as demonstrated in Lemma~\ref{lemm:balancing}. \qq{fix}
To understand Theorem~\ref{thm:stable_oscillations} more clearly, consider the first eigenvector of the Hessian, which is
\begin{align*}
        \Delta_1 = \frac{1}{\sqrt{L}}\cdot \mathrm{vec}\left(\mbf{u}_{\star, 1} \mbf{v}_{\star, 1}^\top, \mbf{v}_{\star, 1}  \mbf{v}_{\star, 1}^\top, \ldots, \mbf{v}_{\star, 1}  \mbf{v}_{\star, 1}^\top \right),
\end{align*}
where $\mbf{u}_{\star, 1}, \mbf{v}_{\star, 1} \in \mbb{R}^d$ are the first left and right singular vectors of $\mbf{M}_\star$, respectively. By Proposition~\ref{prop:one_zero_svs_set}, we know that the each weight layer takes the form  $\mbf{W}_\ell = \mbf{V}_\star \mbf{\Sigma}_\ell \mbf{V}_\star$ \qq{transpose?} for all $\ell \in [L-1]$ and $\mbf{W}_L = \mbf{U}_\star \mbf{\Sigma}_L \mbf{V}_\star$ at convergence, starting from the unbalanced initialization. By stacking and flattening these weights, consider the direction
\begin{align*}
    \widetilde{\Delta} \coloneqq \sum_{i=1}^d \mathrm{vec}\left(\sigma_{L, i}\cdot\mbf{u}_{\star, i} \mbf{v}_{\star, i}^\top,\sigma_{L-1, i}\cdot \mbf{v}_{\star, i}  \mbf{v}_{\star, i}^\top, \ldots, \sigma_{1, i}\cdot\mbf{v}_{\star, i}  \mbf{v}_{\star, i}^\top \right).
\end{align*}
Since $\widetilde{\Delta}^\top \Delta_1$ is only non-zero in the rank-$1$ components of $\widetilde{\Delta}$, this implies that if $\lambda_1 \leq K < \lambda_2$ from Theorem~\ref{thm:stable_oscillations},
the oscillations only occur in the rank-$1$ components of the weights. The following result substantiates this claim by demonstrating that, with an appropriately chosen learning rate, oscillations occur in the singular values in the top-$r$ directions.

\begin{theorem}[\edit{Rank-$p$} Oscillations]
\label{thm:align_thm}
\edit{Let $\mbf{M}_\star = \mbf{U}_\star \mbf{\Sigma}_\star \mbf{V}_\star^\top$ denote the SVD of the target matrix and define $S_p\coloneqq L \sigma^{2-\frac{2}{L}}_{\star,p}$ and $K'_p \coloneqq \mathrm{max} \left\{ S_{p+1},\frac{S_p}{2\sqrt{2}}\right\}$.
If we run GD on the deep matrix factorization loss with initialization scale $\alpha < \alpha'$ from Theorem~\ref{thm:stable_oscillations} and learning rate $\eta = \frac{2}{K}$, where $K'_p < K< S_p$, then under strict balancing, each weight matrix $\mbf{W}_{\ell} \in \mbb{R}^{d\times d}$ oscillates around the balanced minimum in a $2$-period fixed orbit ($j \in \{1,2\}$) as follows:
\begin{align*}
    \mbf{W}_L &= \sum_{i=1}^p\rho_{i, j} \cdot \mbf{u}_{\star, i}\mbf{v}_{\star, i}^{\top} + \sum_{k=p+1}^d \sigma_{\star, k}^{1/L} \cdot \mbf{u}_{\star, k}\mbf{v}_{\star, k}^{\top}, \\
    \mbf{W}_\ell &=\underbrace{\sum_{i=1}^p\rho_{i, j} \cdot \mbf{v}_{\star, i}\mbf{v}_{\star, i}^{\top} }_{\text{oscillation subspace}}+ \underbrace{\sum_{k=p+1}^r \sigma_{\star, k}^{1/L}\cdot \mbf{u}_{\star, k}\mbf{v}_{\star, k}^{\top} + \sum_{m=r+1}^d \alpha\cdot \mbf{u}_{\star, m}\mbf{v}_{\star, m}^{\top}}_{\text{stationary subspace}}, \quad \forall\ell \in [L-1],
\end{align*}
where $\rho_{i, 1} \in \left(0, \sigma_{\star, i}^{1/L}\right)$ and $\rho_{i, 2} \in \left(\sigma_{\star, i}^{1/L}, (2\sigma_{\star, i})^{1/L}\right)$} are the two real roots of the polynomial $g(\rho_i)=0$, where
\begin{align*}
    g(\rho_i) = \rho_i^L\cdot\frac{1+\left(1 + \eta L(\sigma_{\star, i} - \rho_i^L)\cdot \rho_i^{L-2} \right)^{2L-1}}{1+\left(1 + \eta L(\sigma_{\star, i} - \rho_i^L)\cdot \rho_i^{L-2} \right)^{L-1}} - \sigma_{\star, i}.
\end{align*}
\end{theorem}

%\ag{Should we have the general oscillation as a lemma?
%Also where are we having the digoanl liner network oscillation?}
%\paragraph{Remarks.}
In contrast to Theorem~\ref{thm:stable_oscillations}, Theorem~\ref{thm:align_thm} explicitly identifies the subspaces that exhibit a two-period orbit based on the range of the learning rate. It also provides a rough characterization of the oscillation amplitude, which is determined by $\rho_{i, 1}$ and $\rho_{i, 2}$—values below and above the balanced minimum, respectively. 
%Hence, the oscillations occur around the minima.
Since there is no closed-form solution for an arbitrary higher-order polynomial, $\rho_{i, 1}$ and $\rho_{i, 2}$ are defined as solutions to the polynomial $g(\rho_i)$.
Overall, this aims to theoretically explain why (i) oscillations occur primarily within the top subspaces of the network, as observed by~\cite{zhu2023catapults}, and (ii) oscillations are more pronounced in the directions of stronger features, as measured by the magnitudes of their singular values.


\begin{figure}[t!]
    \centering
     \begin{subfigure}[t!]{0.495\textwidth}
         \centering
        \includegraphics[width=0.85\textwidth]{figures/eos_balanced_contour_1.pdf}
        \caption*{$\eta < 0.2$}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t!]{0.495\textwidth}
         \centering
         \includegraphics[width=0.85\textwidth]{figures/eos_balanced_contour_2.pdf}
         \caption*{$\eta > 0.2$}
     \end{subfigure}
    \caption{Illustration of the GD trajectories for two different learning rates for minimizing the function $f(\sigma_1, \sigma_2) = \frac{1}{2}(\sigma_2 \cdot \sigma_1 - 5)^2$, starting from an unbalanced initial point. The sharpness at the balanced minimum is $10$, and so the learning rate needed to enter EOS is $\eta = 0.2$. These plots show that while GD initially arrives at an unbalanced solution in both cases, the iterates oscillate about the other minima to arrive at the balanced solution within the EOS regime.
    }
    
    \label{fig:contour}
\end{figure}



Notice that Theorem~\ref{thm:align_thm} demonstrates the existence of a two-period orbit only around the balanced minimum. While this assumption was initially made for ease of analysis, we empirically observe that the two-period orbit actually \emph{only} occurs around the balanced solution.
To illustrate this claim, in Figure~\ref{fig:contour}, we provide a plot of the GD trajectory for minimizing a two-layer scalar loss $f(\sigma_1, \sigma_2) = \frac{1}{2}(\sigma_2 \cdot \sigma_1 - 5)^2$, starting from an unbalanced initial point $(\sigma_1, \sigma_2) = (1.5, 2.25)$. Notice that, by Lemma~\ref{lemma:hessian_eigvals}, the sharpness around the balanced minimum is $L\sigma_{\star,1}^{2-2/L} = 10$, and thus the necessary learning rate to enter the EOS regime is $\eta = 0.2$.
We plot the GD trajectory under two cases for the learning rate: (i) slightly below the EOS learning rate, $\eta = 0.1999$, and (ii) slightly above it, $\eta = 0.2010$. When $\eta = 0.2010$, GD first arrives at an unbalanced solution, then oscillates until it reaches the balanced minimum, where it sustains a two-period orbit around the balanced solution. The other minima are too narrow to sustain the oscillations induced by the large learning rate, causing the GD iterates to bounce out of those minima and settle at the flattest, balanced solution.
When the learning rate is slightly below $\eta = 0.2$, it remains large enough to induce oscillations around other unbalanced minima, but ultimately GD converges to the balanced solution, where it exhibits no oscillations, as predicted by Theorem~\ref{thm:align_thm}. This empirical observation suggests that two-period oscillations and balancing occur simultaneously, which we leave for future investigation.

Finally, we conclude by remarking that our result also aims to generalize the recent theoretical findings of~\cite{chen2023edge}, where they proved the existence of a certain class of scalar functions \( f(x) \) for which GD does not diverge even when operating beyond the stability threshold.
%\( \eta > \frac{2}{f^{''}(\hat{x})} \), where \( \hat{x} \) is a local minimum of \( f(x) \). Specifically, they showed that for a function dependent $\epsilon > 0$, there exists a range \( \eta \in \left( \frac{2}{f^{''}(\hat{x})}, \frac{2}{f^{''}(\hat{x})}(1+\epsilon) \right) \), 
They demonstrated that there exists a range in which the loss oscillates around the local minima with a certain periodicity. These oscillations gradually progress into higher periodic orbits (e.g., 2, 4, 8 periods), transition into chaotic behavior, and ultimately result in divergence. In our work, we prove that this oscillatory behavior beyond the stability threshold also occurs in DLNs.



% For the initialization scale, we require an upper bound on $\alpha$ to satisfy the balancing condition in Lemma~\ref{lemma:balancing}.


\subsection{Assumptions and Analytical Tools}
\label{sec:used_tools}

This section presents the two main tools used in our analyses: the singular vector stationary set and
singular value balancedness. First, we present the singular vector stationary set, which allows us to
encompass a wider range of initialization schemes. This set defines a broad class of initialization for
which singular vector alignment occurs, simplifying the dynamics to only singular values.


\begin{proposition}[Singular Vector Stationary Set]
\label{prop:svs_set}
Consider the deep matrix factorization loss in Equation~(\ref{eqn:deep_mf}). Let $\mbf{M}_\star = \mbf{U}_\star \mbf{\Sigma}_\star \mbf{V}_\star^\top$ and 
$\mbf{W}_\ell(t) = \mbf{U}_\ell(t) \mbf{\Sigma}_\ell(t) \mbf{V}_\ell^\top(t)$ denote the compact SVD for the target matrix and the $\ell$-th layer weight matrix at time $t$, respectively. For any time $t\geq 0$, if $\dot{\mbf{U}}_\ell(t) = \dot{\mbf{V}}_\ell(t) = 0$ for all $\ell \in [L]$, then the singular vector stationary points for each weight matrix are given by
\begin{align*}
\mathrm{SVS}(f(\mbf{\Theta})) = 
\begin{cases}
    (\mbf{U}_L, \mbf{V}_L) &= (\mbf{U}_\star, \mbf{Q}_L), \\
    (\mbf{U}_\ell, \mbf{V}_\ell) &= (\mbf{Q}_{\ell+1}, \mbf{Q}_\ell), \quad\forall \ell \in [2, L-1], \\
    (\mbf{U}_1, \mbf{V}_1) &= (\mbf{Q}_2, \mbf{V}_\star),
\end{cases}
\end{align*}
where \(\{\mbf{Q}_\ell\}_{\ell=2}^{L}\) are any set of orthogonal matrices. 
\end{proposition}


The singular vector stationary set states that for any set of weights where the gradients with respect to the singular vectors become zero, the singular vectors become fixed points for subsequent iterations. Once the singular vectors become stationary, running GD further isolates the dynamics on the singular values. Hence, throughout our analysis, we re-write and consider the loss 
\begin{align}\label{eqn:simplified_loss}
    \frac{1}{2} \left\|\mbf{W}_{L:1}(t) - \mbf{M}^\star\right\|^2_{\mathsf{F}} = \frac{1}{2} \|\mbf{\Sigma}_{L:1} - \mbf{\Sigma}^\star\|^2_{\mathsf{F}} = \frac{1}{2} \sum_{i=1}^r \left(\sigma_i(\mbf{\Sigma}_{L:1}(t)) - \sigma_{\star, i}\right)^2,
\end{align}
where $\mbf{\Sigma}_{L:1}$ are the singular values of $\mbf{W}_{L:1}$. This allows us to decouple the dynamics of the singular vectors and singular values, focusing on the periodicity that occurs in the singular values within the EOS regime. \edit{In Propositions~\ref{prop:one_zero_svs_set} and~\ref{prop:balanced_svs_set}, we prove that both the unbalanced and balanced initializations belong to this set respectively,
with an illustration in Figure~\ref{fig:svec_alignment}.
Specifically, we show that the singular vectors belongs to the singular vector stationary set after GD iteration $t=1$ (far before entering the EOS regime) with $\mbf{Q}_\ell = \mbf{V}_\star$,
allowing us to consider the loss in Equation~(\ref{eqn:simplified_loss}).}
Next, we present a result to validate our use of the strictly balanced assumption \edit{on the unbalanced initialization case} by showing that the singular values become increasingly balanced throughout the GD iterations.

\begin{lemma}[Balancing]
\label{lemma:balancing}
   Let $\sigma_{\star, i}$ and $\sigma_{\ell, i}(t)$ denote the $i$-th singular value of $\mbf{M}_\star \in \mbb{R}^{d\times d}$ and $\mbf{W}_\ell(t)$, respectively and define $S_i \coloneqq L \sigma^{2-\frac{2}{L}}_{\star,i}$.
    Consider GD on the $i$-th index of the simplified loss in~(\ref{eqn:simplified_loss}) with unbalanced initialization in  (\ref{eqn:init}) and learning rate $\frac{2}{S_i} < \eta < \frac{2\sqrt{2}}{S_i}$. If the initialization scale $\alpha$ satisfies
    $0 < \alpha < \left( \ln\left( \frac{2\sqrt{2}}{\eta S_i} \right) \cdot \frac{ \sigma_{\star, i}^{4/L}}{L^2 \cdot 2^{\frac{2L-3}{L}}} \right)^{1/4}$, \edit{then there exists a constant $c \in (0, 1]$ such that} for all $\ell \in [L-1]$, we have $\left| \sigma^2_{L, i}(t+1) - \sigma^2_{\ell, i}(t+1)\right| < \edit{c}\left| \sigma^2_{L, i}(t) - \sigma^2_{\ell, i}(t)\right|$.
\end{lemma}

\begin{wrapfigure}{r}{0.385\textwidth}
  \begin{center}
    \includegraphics[width=\linewidth]{figures/balancing_gap.pdf}
    
  \end{center}
  \caption{Plot of $| \sigma^2_{L, i}(t) - \sigma^2_{\ell, i}(t)|$ 
 showing strict balancing.}
\label{fig:balancing}
\end{wrapfigure}
This result has been shown to hold similarly for two-layer matrix factorization~\citep{wang2021large,ye2021global,chen2023edge}, and our analysis extends it to the deep case.
Lemma~\ref{lemm:balancing} considers the scalar loss for a single singular value index and states that, as long as $\alpha$ is chosen below a threshold dependent on $\sigma_{\star, i}$, the $i$-th singular value will become increasingly balanced. To ensure that balancing occurs for all singular values of the loss in~(\ref{eqn:simplified_loss}), we can select the learning rate to induce oscillations in all singular values (assuming they remain below the divergence limit) and choose $\alpha$ with $\sigma_{\star, 1}$ such that it is the smallest $\alpha$ that satisfies the condition for all singular values $\sigma_{\star, i}$.


If the constant were $c < 1$, note that the balancing gap would approach zero infinitesimally. However, our analysis currently only shows that 
$c<1$ when the product of singular values across all layers $\sigma_i(\mbf{\Sigma}_{L:1}) < \sigma_{\star, i}$ and but $c=1$ when $\sigma_i(\mbf{\Sigma}_{L:1}) > \sigma_{\star, i}$.
Since we start from a small initialization scale, we generally mostly operate within the regime $\sigma_i(\mbf{\Sigma}_{L:1}) < \sigma_{\star, i}$,
and only transition to the latter regime when oscillations occur.
Note that $\sigma_i(\mbf{\Sigma}_{L:1}) = \sigma_{\star, i}$ cannot occur since the learning rate is chosen to be within the EOS regime -- equality
can only arise in the stable regime, where balancing does not occur. 
%\edit{To summarize, Lemma~\ref{lemm:balancing} states that, provided $\alphay$ is chosen below a certain threshold, the top-$r$ singular values of the weights across all layers become increasingly balanced during GD, even if they are unbalanced as in the initialization of Equation~(\ref{eqn:init}).  Our result is an extension of these analyses, but to the deep matrix factorization case. Our analysis shows that the constant $c$ changes for two different cases\footnote{We exclude the case  $\sigma_i(\mbf{\Sigma}_{L:1}) = \sigma_{\star, i}$, as this occurs with probability 0 in the presence of oscillations in the EOS regime.}: (i) $0<c<1$ when the product of singular values across all layers $\sigma_i(\mbf{\Sigma}_{L:1}) < \sigma_{\star, i}$ and (ii) $c=1$ when $\sigma_i(\mbf{\Sigma}_{L:1}) > \sigma_{\star, i}$. In the literature, it has been widely shown that the dynamics of DLNs (along with diagonal linear networks) exhibit an incremental learning phenomenon, where the singular values $\sigma_i(\mbf{W}_\ell)$ start from $\alpha$ and increase to the target singular value one-by-one~\citep{gissin2020the, inclearndiag, kwon, jacot2021saddle}. Empirically, this implies that we often operate in the regime of $\sigma_i(\mbf{\Sigma}_{L:1}) < \sigma_{\star, i}$, as the oscillations begin to occur once we reach and about the minima. Hence, throughout most of the learning trajectory, $0<c<1$ holds, and the balancing gap becomes infinitesimally small.}
In Figure~\ref{fig:balancing},
we plot the balancing gap between the top-3 singular values of a weight matrix initialized to zero and those initialized to $\alpha$ for a rank-3 matrix.
 This plot shows that the gap decreases and goes to zero empirically, and this is consistently the case across all of our experiments, with additional results provided in Appendix~\ref{sec:additional_exp}.
 This provides empirical evidence that our analysis can be further improved such that $c<1$ for both cases. 
 To this end, we use this insights to assume that strict balancing holds for both initializations in Equation~(\ref{eqn:init}). This allows us to write the loss of the singular values into the form $\sigma_i(\mbf{\Sigma}_{L:1}(t)) = \sigma^L_{i}(t)$, which allows us to focus on the dynamics in the singular values.





%Also in Appendix~\ref{sec:additional_exp}, we show that even for a slightly larger initialization scale, the balancing still holds in practice. Furthermore, we note that very similar results for imbalanced initialization have been proven by~\cite{wang2021large}, where our result can be viewed as an extension to multiple variables.
%Finally, by assuming strict balancing, we can simplify the loss even further, particularly in the form $\sigma_i(\mbf{\Sigma}_{L:1}(t)) = \sigma^L_{i}(t)$, which allows us to solely analyze the dynamics of the singular values within the EOS regime. 

%Recall that by our initialization scheme, we initialize to $\sigma_{L, i}(0) = 0$ and $\sigma_{\ell, i}(0) = \alpha$ for all $\ell \in [L-1]$. By considering the singular value scalar loss in Equation~(\ref{eqn:simplified_loss}), the gradient with respect to each $\sigma_{\ell, i}(t)$ are all the same. Thus, except for $\sigma_{L, i}(t)$, all of the other singular values across all weight matrices remain balanced throughout all iterations of GD. Lemma~\ref{lemma:balancing} states that throughout the course of GD, as long as $\alpha$ is below a certain threshold, $\sigma_{L, i}(t)$ becomes increasingly balanced to the rest of the singular values regardless of the learning rate. Since the balancing gap strictly decreases and $| \sigma^2_{i,L} - \sigma^2_{i,\ell} |$ is lower bounded by zero, it converges to 0 as $t \to \infty$. 


%However, it is worth noting that (i)~Lemma~\ref{lemma:balancing} does not state that the difference goes to zero, but rather that it becomes increasingly balanced and (ii) the bound on $\alpha$ may be too conservative and is an artifact of our analysis. 








\begin{comment}
    
\begin{figure}[htbp]
    \centering
    \begin{minipage}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/deep_martix_figs/oscillation_ranges.png}
        \caption{Figure 1}
        \label{fig:figure1}
    \end{minipage}%
    \hfill
    \begin{minipage}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/deep_martix_figs/layer_1_singular_values_0.01546.png}
        \caption{$\eta=\frac{1}{L\sigma^{2-\frac{2}{L}}_{\star,1}}$}
        \label{fig:figure2}
    \end{minipage}%
    
    \vspace{0.5cm} % Adds some vertical space between rows

    \begin{minipage}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/deep_martix_figs/layer_1_singular_values_0.0167.png}
        \caption{$\eta=\frac{1}{\sum_{\ell=0}^{L-1} \left(\sigma_{\star, 1}^{1-\frac{1}{L} - \frac{1}{L}\ell} \cdot \sigma_{\star, 2}^{\frac{1}{L}\ell}\right)^2}$}
        \label{fig:figure3}
    \end{minipage}%
    \hfill
    \begin{minipage}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/deep_martix_figs/layer_1_singular_values_0.02.png}
        \caption{$\eta>\frac{1}{L\sigma^{2-\frac{2}{L}}_{\star,2}}$}
        \label{fig:figure4}
    \end{minipage}
    \caption{}
\end{figure}





\end{comment}




%it is possible to have $r$-dimensional oscillations as long as the learning rate is chosen correctly. 



%\paragraph{Remarks.} By adopting this proof technique, we show that both conditions are true in each eigenvector direction considered in Theorem~\ref{thm:stable_oscillations}. Hence, Theorem~\ref{thm:stable_oscillations} that it is possible to have $r$-dimensional oscillations as long as the learning rate is chosen correctly. 












\subsection{Relation to Diagonal Linear Networks}

\label{sec:diagonal}

%Due to singular vector stationarity and balancing, DLNs may appear equivalent to diagonal linear networks at first glance. In this section, we characterize an explicit distinction between the two networks by deriving the eigenvalues of diagonal linear networks from the Hessian at convergence and explaining how they contribute to periodic oscillations in the EOS regime.

In this section, we derive the necessary conditions and characteristics of two-period oscillations in diagonal linear networks to establish their similarities with DLNs.

\begin{theorem}[Subspace Oscillation for Diagonal Linear Networks]
\label{thm:diag_lin_thm}
\edit{Consider an $L$-layer diagonal linear network on the loss 
\begin{align}
\label{eqn:diag_lin_loss}
        \mathcal{L}\left(\{\mbf{s}_\ell\}_{\ell=1}^L \right) \coloneqq \frac{1}{2} \|\mbf{s}_1 \odot \ldots \odot \mbf{s}_{L} - \mbf{s}_{\star}\|_2^2, 
 \end{align}
where $\mbf{s}_\star \in \mbb{R}^{d}$ be an $r$-sparse vector with ordered coordinates such that $s_{\star,1} >\ldots>s_{\star,d}$ and define $S_p \coloneqq L s_{\star,p}^{2-\frac{2}{L}}$ and $\alpha' \coloneqq \left( \ln\left( \frac{2\sqrt{2}}{\eta L s_{\star, 1}^{2 - \frac{2}{L}}} \right) \cdot \frac{ s_{\star, 1}^{\frac{4}{L}}}{L^2 \cdot 2^{\frac{2L-3}{L}}} \right)^{\frac{1}{4}}$.
For any $p < r-1$ and $\alpha < \alpha'$, suppose we run GD on Equation~(\ref{eqn:diag_lin_loss}) with learning rate $\eta = \frac{2}{K}$, where $S_{p}\geq K> S_{p+1}$ with initialization 
$\mbf{s}_\ell = \alpha  \mbf{1}_d$ for all $\ell \in [L-1]$ and $\mbf{s}_{L}=\mbf{0}_d$.} Then, under strict balancing, the top-$p$ coordinates of $\mbf{s}_\ell$ oscillate within a $2$-period fixed orbit around the minima in the form
 \begin{align*}
     s_{\ell, i}(t) = \rho_{i, j}(t), \quad \forall i < p,  \, \forall \ell \in [L],
 \end{align*}
where $\rho_{i, j}(t) \in\{\rho_{i, 1}, \rho_{i, 2}\}$, $\rho_{i, 1} \in \left(0, s_{\star, i}^{1/L} \right)$ and $\rho_{i, 2} \in \left(s_{\star, i}^{1/L}, (2s_{\star, i})^{1/L} \right)$ are two real roots of the polynomial $h(\rho)=0$:
\begin{align*}
    h(\rho) = \rho^L\cdot \frac{1+\left(1 + \eta L(s_{\star,i}  - \rho^L)\cdot \rho^{L-2} \right)^{2L-1}}{1+\left(1 + \eta L(s_{\star,i}  - \rho^L)\cdot \rho^{L-2} \right)^{L-1}}- s_{\star,i}.
\end{align*}

\end{theorem}

\begin{figure}[t!]
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \caption*{\footnotesize Rank-$1$ Oscillation}
\includegraphics[width=\textwidth]{figures/eos_osc_region_1.pdf}
\caption*{$S_1 >K>S_2$}
\end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \caption*{\footnotesize Rank-$2$ Oscillation}
\includegraphics[width=\textwidth]{figures/eos_osc_region_2.pdf}
\caption*{$S_2 >K>S_3$}
\end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \caption*{\footnotesize Rank-$3$ Oscillation}
         \includegraphics[width=\textwidth]{figures/eos_osc_region_3.pdf}
         \caption*{$S_3 >K>S_4$}
\end{subfigure}
\caption{Evolution of the singular values of the end-to-end $3$-layer network for fitting a rank-3 target matrix with singular values $10$, $9.5$, and $9$. We use a learning rate of $\eta = 2/S_i$ with $S_i \coloneqq L\sigma_{\star, i}^{2 - 2/L}$. The oscillations occur exactly with learning rate ranges specified in Theorem~\ref{thm:align_thm}.}
\label{fig:thm2_osc}
\end{figure}


From Lemma~\ref{lemma:hessian_eigvals}, we observe that DLNs exhibit additional dominant curvature directions that are not present in diagonal linear networks—specifically, the eigenvalues corresponding to the ``interaction with other singular values'' are absent in diagonal linear networks. These eigenvalues arise due to the zero off-diagonal elements of the singular value diagonal matrix in~(\ref{eqn:simplified_loss}).
However, despite these extra directions, Theorem~\ref{thm:diag_lin_thm} demonstrates that the behavior of diagonal linear networks and DLNs is essentially the same. This can be understood using the argument from Theorem~\ref{thm:stable_oscillations}: the eigenvectors corresponding to these directions are always orthogonal to the flattened weights $\widetilde{\Delta}$, thereby making the behaviors of the two network types synonymous, even in the EOS regime.


%Similar to Theorem~\ref{thm:align_thm}, each coordinate of the diagonal linear network undergoes periodic oscillations with an appropriately chosen learning rate. However, as shown in the proof of Theorem~\ref{thm:diag_lin_thm}, the main difference lies in the eigenvalues themselves -- the number non-zero eigenvalues for diagonal linear networks are much smaller than those of the DLN. The set of eigenvalues corresponding to the interaction with other singular values in Lemma~\ref{lemma:hessian_eigvals} are missing for diagonal linear networks. Therefore, the top two eigenvalues of the diagonal linear network are $L s_{\star, 1}^{2 - \frac{2}{L}}$ and $L s_{\star, 2}^{2 - \frac{2}{L}}$, whereas the top two eigenvalues of the DLN are  $L s_{\star, 1}^{2 - \frac{2}{L}}$ and $\sum_{\ell=0}^{L-1} \left(s_{\star, 1}^{1-\frac{1}{L} - \frac{1}{L}\ell} \cdot s_{\star, 2}^{\frac{1}{L}\ell}\right)^2$. Hence, the dynamics in the EOS regime between the two networks differ significantly (see Figure~\ref{fig:diff_dln_diag}). \edit{The primary difference in the landscape arises from the zero off-diagonal elements of the singular value diagonal matrix of the DLN which introduces additional curvature directions despite singular vector invariance.}


% In the DLN, some eigenvalues are a function of a ``mixture'' of singular values, which arise from the off-diagonal elements in the decoupled loss in Equation~(\ref{eqn:simplified_loss}). In the diagonal linear network, they depend only on a single coordinate (i.e., $s_{\star,i}$) or the initialization scale $\alpha$. Hence, in the diagonal linear network, a much larger learning rate is required to observe oscillations in two or more coordinates compared to the DLN. 



==> ICLR/text_after_sub/experiments.tex <==
\section{Experimental Results}
In this section, we present experimental results to supplement our theory along with experiments on nonlinear networks within the EOS regime. Section~\ref{sec:oscillations_exp} presents experiments that corroborate our theory. Section~\ref{sec:lora_exp} shows experiments where oscillations occur when using low-rank adaptors and their relation to generalization. Finally, Section~\ref{sec:unexplained_exp} discusses phenomena currently unexplained in the literature and how our theory can account for them.



\begin{figure}[t!]
    \centering
     \begin{subfigure}[b]{0.325\textwidth}
         \centering
        \includegraphics[width=\textwidth]{figures/oscillation/eos_sval_none.pdf}
     \end{subfigure}
     \begin{subfigure}[b]{0.325\textwidth}
         \centering
        \includegraphics[width=\textwidth]{figures/oscillation/eos_sval_1.pdf}
     \end{subfigure}
         \begin{subfigure}[b]{0.325\textwidth}
         \centering
        \includegraphics[width=\textwidth]{figures/oscillation/eos_sval_2.pdf} 
     \end{subfigure}
        \newline
      \begin{subfigure}[b]{0.325\textwidth}
         \centering
        \includegraphics[width=\textwidth]{figures/oscillation/eos_sval_diag_none.pdf}
         \caption*{$\eta < 2/\lambda_1$}
     \end{subfigure}
     \begin{subfigure}[b]{0.325\textwidth}
         \centering
        \includegraphics[width=\textwidth]{figures/oscillation/eos_sval_diag_1.pdf}
         \caption*{$2/\lambda_1 <\eta < 2/\lambda_2$}
     \end{subfigure}
         \begin{subfigure}[b]{0.325\textwidth}
         \centering
        \includegraphics[width=\textwidth]{figures/oscillation/eos_sval_diag_2.pdf} 
         \caption*{$\eta > 2/\lambda_2 > 2/\lambda_1$}
     \end{subfigure}   
    \caption{Top: Plots of the singular values of the end-to-end DLN; Bottom: plots of the end-to-end diagonal linear network, where $\lambda_i$ denotes the $i$-th largest eigenvalue of the Hessian. While the largest eigenvalue for both networks are the same $\lambda_1 = L\sigma_{\star,1}^{2- \frac{2}{L}}$, the second largest eigenvalue is different, and we use
    $\lambda_2 = \sum_{\ell=0}^{L-1} \left(\sigma_{\star, 1}^{1-\frac{1}{L} - \frac{1}{L}\ell} \cdot \sigma_{\star, 2}^{\frac{1}{L}\ell}\right)^2$, which is the second largest eigenvalue of the DLN. While the DLN undergoes oscillations in the top-2 components, the diagonal linear network only shows oscillations in 1.}
    \label{fig:diff_dln_diag}
\end{figure}

\subsection{Subspace Oscillations in Deep Networks}
\label{sec:oscillations_exp}

\begin{wrapfigure}{r}{0.35\textwidth}
  \begin{center}
    \includegraphics[width=0.35\textwidth]{figures/oscillation_range.pdf}
  \end{center}
  \caption{Oscillation range as a function of the learning rate.}
\label{fig:osc_range}
\end{wrapfigure}
Firstly, we provide experimental results corroborating Theorem~\ref{thm:align_thm} and Theorem~\ref{thm:diag_lin_thm} to highlight their differences. We let the target matrix be $\mbf{M}_\star \in \mbb{R}^{50 \times 50}$ with rank 3, with dominant singular values $\sigma_{\star} = {10, 9, 6}$.
For the DLN, we consider a 3-layer network, with each layer as $\mbf{W}_\ell \in \mbb{R}^{50\times 50}$ and use an initialization scale of $\alpha = 0.01$. For the diagonal linear network, we consider a similar setup, with initialization scale $\alpha = 0.01$ and the top-3 elements of $\mbf{s}_\star \in \mbb{R}^{50}$ to be $10, 9, 6$. 
In Figure~\ref{fig:diff_dln_diag}, we present the behaviors of both end-to-end networks under different learning rate regimes. By Theorem~\ref{thm:align_thm} and Theorem~\ref{thm:diag_lin_thm}, the largest eigenvalue $\lambda_1$ is the same for both networks, and thus both undergo oscillations in the largest component when $\eta > 2/\lambda_1$. 
However, the difference in the loss landscape plays a role in oscillations for the second component.
When $\eta > 2/\lambda_2$, where $\lambda_2$ is the second largest eigenvalue of the DLN, the diagonal linear network does not experience oscillations in the second component, as its second largest eigenvalue is much smaller. 
This highlights a distinction between the two networks and how the landscape changes between them. In Figure~\ref{fig:osc_range}, we present an experiment demonstrating the relationship between the range of oscillations and the learning rate by plotting the amplitude of the singular value oscillations in the end-to-end network.
We can clearly see that there exists no oscillations when $\eta < 2/\lambda_1$, but begins to occur as soon as $\eta > 2/\lambda_1 $. As the learning rate increases, the amplitude also increases, which can similarly be observed in Figure~\ref{fig:diff_dln_diag}. 






\subsection{Oscillations in Low-Rank Adaptors}
\label{sec:lora_exp}


Low-rank adaptation (LoRA)~\citep{lora} has arguably become one of the most popular methods for fine-tuning deep neural networks. The main idea behind LoRA is that rather than training from scratch, we can update two low-rank factor matrices to ``append'' onto an existing weight matrix.
That is, give a pre-trained weight matrix $\mathbf{W}_0 \in \mathbb{R}^{d_1 \times d_2}$, LoRA involves updating two low-rank factors commonly referred to as ``adaptors'':
\begin{align*}
    \underbrace{\mathbf{W}_\star}_{\text{new weight}} = \underbrace{\mathbf{W}_0}_{\text{pre-trained weight}} + \underbrace{\mathbf{AB}^\top}_{\text{adaptors}}.
\end{align*}
Upon training only $\mathbf{A} \in \mbb{R}^{d_1 \times r}$ and $\mathbf{B} \in \mbb{R}^{d_2 \times r}$, $\mathbf{W}_\star \in \mbb{R}^{d_1 \times d_2}$ is used for inference. By viewing the adaptations as individual low-rank matrix factorization problems, then this formulation closely aligns with our theoretical setup with a depth of $2$. Hence, we investigate (i) how oscillations may appear in such a setup and (ii) what these oscillations may imply in terms of generalization.


To this end, we follow the setup used by~\cite{yaras2024compressible} and consider a pre-trained BERT~\citep{wang2018glue} base model and apply
adaptation on all attention and feedforward weights in the transformer, resulting in 72 adapted
layers in total. 
We choose an initialization scale of $\alpha = 10^{-3}$ for the adaptors and randomly sample $512$ examples from the STS-B~\citep{wang2018glue} dataset for fine-tuning.  We choose a batch size of 64  with a maximum sequence length of 128 tokens. 
First, we experiment how large the rank of the adaptors must be to drive the entire network to EOS. Using a learning rate of $\eta = 10^{-4}$, Figure~\ref{fig:rank_vs_correlation} shows oscillatory behavior across all ranks. However, this behavior may also be an artifact of the stochasticity induced by updating with only a batch of samples. Notably, for ranks $r = 4$ and $r = 8$, there are catapults (or jumps) that occur very early in the iterations, which do not occur for $r = 1$ or $r = 2$. Then, using a rank of $r=8$, we experiment what the oscillations and catapults might imply in terms of generalization.
\begin{wrapfigure}{l}{0.375\textwidth}
  \begin{center}
    \includegraphics[width=0.375\textwidth]{figures/bert/train_loss_ranks.pdf}
  \end{center}
  \caption{Catapults in the training loss for different ranks for LoRA.}
\label{fig:rank_vs_correlation}
\end{wrapfigure}
 In Figure~\ref{fig:lr_vs_correlation}, we present the training loss and Pearson correlation for different learning rates.
 When the learning rate is large enough to induce catapults (as seen for $\eta = 10^{-4}$), we observe that the training loss decreases rapidly, resulting in a very high Pearson correlation. In contrast, when the learning rate is small, convergence takes much longer, as the model seems to bounce around within the same local basin before reaching a low training loss. These results suggest that there may exist a combination of rank and learning rate that can converge to an optimal solution (as measured by Pearson correlation) more quickly and with better generalization by inducing catapults in the loss through EOS, as the learning rate of $10^{-4}$ appears to yield the highest Pearson correlation.
We leave for future work a careful study of this observation, aiming to accurately select the learning rate to maximize the efficiency of LoRA.

 \begin{comment}
    \begin{figure}[h!]
    \centering
     \begin{subfigure}[t!]{0.495\textwidth}
         \centering
        \includegraphics[width=0.87\textwidth]{figures/bert/train_loss.pdf}
     \end{subfigure}
     \begin{subfigure}[t!]{0.495\textwidth}
         \centering
         \includegraphics[width=0.9\textwidth]{figures/bert/test_loss.pdf}
     \end{subfigure}
    \caption{Illustration of the different behaviors in the training loss for various ranks of the adaptors at a fixed learning rate of $\eta = 10^{-4}$. While each choice of rank exhibits oscillations, higher ranks show more ``catapults'', which appear to be correlated with generalization as measured by Pearson correlation.}
    
    \label{fig:rank_vs_correlation}
\end{figure}
\end{comment}

\begin{figure}[t!]
    \centering
     \begin{subfigure}[t!]{0.495\textwidth}
         \centering
        \includegraphics[width=0.75\textwidth]{figures/bert/train_loss_diff_lr.pdf}
     \end{subfigure}
     \begin{subfigure}[t!]{0.495\textwidth}
         \centering
         \includegraphics[width=0.75\textwidth]{figures/bert/test_loss_diff_lr.pdf}
     \end{subfigure}
    \caption{Illustration of different behaviors in the training loss for various learning rates with a fixed rank of $r=8$ for fine-tuning BERT using LoRA. When the learning rate is large enough to induce catapults in the loss (visible early in the stages for $\eta = 10^{-4}$), the adaptors converge to a point with high Pearson correlation much more rapidly.}
    
    \label{fig:lr_vs_correlation}
\end{figure}

\subsection{Deep Linear Networks to Explain Phenomena in Nonlinear Networks}
\label{sec:unexplained_exp}

%In this section, we draw parallels between observations made in deep nonlinear networks and our theory on DLNs.



\paragraph{Mild Sharpening.} \cite{cohen2021gradient} discussed in Caveat 2 of their work that sharpness does not always rise to $2/\eta$, especially in tasks with low complexity. We re-illustrate this in Figure~\ref{fig:combined_figures}, 
\begin{wrapfigure}{r}{0.375\textwidth}
  \begin{center}
    \includegraphics[width=0.375\textwidth]{figures/intro/eos_nuance.pdf}
    \end{center}
    \caption{DLNs do not enter EOS regime if $L\sigma^{2-\frac{2}{L}}_{1}< 2/\eta$.}
    \label{fig:dln_mild_sharpening}
\end{wrapfigure}
where we plot sharpness in two settings: (i) regression with simple images and (ii) classification with an MLP using a subset of the CIFAR-10 dataset. For the regression task, we minimize the loss $\mathcal{L}(\Theta) = \|G(\Theta) - \mbf{y}_{\mathrm{image}}\|_2^2$, where $G(\Theta)$ is a UNet parameterized by $\Theta$, and $\mbf{y}_{\mathrm{image}}$ denotes one of the images in Figure~\ref{fig:img_used}. We observe that when $\mbf{y}_{\mathrm{image}}$ is a smooth, low-frequency image, the sharpness of the loss generally remains low. However, when $\mbf{y}_{\mathrm{image}}$ has higher frequency content, the sharpness increases and enters the EOS regime (Figure~\ref{fig:eos-dip}). Similarly, for the classification task, we train a 2-layer fully connected neural network on $N$ labeled training images from the CIFAR-10 dataset using MSE loss and plot the sharpness in Figure \ref{fig:small_Sharp}. The sharpness of the loss is linked to $N$, the number of data points used for training. For small $N$ values, such as 100 or 200, the network learns only a limited set of latent features, resulting in mild sharpening, and it does not reach the EOS threshold. However, when $N$ exceeds 1000, the sharpness increases and reaches the EOS threshold.
These observations can also be seen in DLNs. In Figure~\ref{fig:dln_mild_sharpening}, we show that the sharpness reaches $L\sigma_{\star, 1}^{2-\frac{2}{L}}$, where $\sigma_{\star, 1}$ is the singular value of the target matrix. Whenever $L\sigma_{\star, 1}^{2-\frac{2}{L}} < 2/\eta$, the network will not enter the EOS regime. This can be viewed as low-complexity learning, as $\sigma_{\star, 1}$ corresponds to the magnitude of the strongest feature of the target matrix. Hence, when $\sigma_{\star, 1}$ is not large enough, the sharpness will not rise to $2/\eta$. Lastly,~\cite{cohen2021gradient} also observed that sharpness scales with the depth of the network, which is also directly supported by our analysis.




\paragraph{Sustained vs. Free Oscillations.}


Here, we discuss the differences in oscillations between ``simpler'' networks such as DLNs and those studied in the literature, versus oscillations and catapults in practical deep nonlinear networks. The main difference lies in the loss landscape—at convergence, the Hessian for DLNs is positive semi-definite, as shown in Lemma~\ref{lemma:hessian_eigvals}, meaning there are only directions of positive curvature and flat directions (in the null space of the Hessian). In this landscape, oscillations occur due to bouncing off the basin walls, with no direction of escape. However, in deep nonlinear networks, it has been frequently observed that the Hessian at the minima has negative eigenvalues \citep{ghorbani2019investigation, sagun2016eigenvalues}. This enables an escape direction along the negative curvature, preventing sustained or free oscillations. We believe understanding the role of nonlinear activation layers in altering this loss landscape is key to addressing this difference.

Lastly,~\cite{damian2023selfstabilization} studied self-stabilization, where sharpness decreases below $2/\eta$ after initially exceeding $2/\eta$. Let $u(\theta)$ be the top eigenvector direction and $\nabla S(\theta)$ denote the change in sharpness. They assume that $\nabla L(\theta) \cdot u(\theta) = 0$ and that $\nabla S(\theta)$ lies in the null space of the Hessian. However, \emph{these assumptions are not satisfied for DLNs}. Due to Proposition~\ref{prop:svs_set} and Lemma~\ref{lemma:balancing}, the dynamics reduce to a one-dimensional oscillating trajectory, where both $\nabla L(\theta)$ and $\nabla S(\theta)$ lie in the range space of the Hessian. By letting $\pi(\theta)$ represent the scalar product of singular values, $\nabla L(\theta) \cdot u(\theta) = (\pi(\theta) - s)\pi(\theta)\cdot|\theta^{-1}|$, which is not zero unless the loss is zero (which is not the case in EOS). Hence, in DLNs, self-stabilization does not occur, and the iterates and sharpness oscillate above $2/\eta$.


\begin{comment}
\subsection{Explaining Sharpening Phenomenon in Deep Nonlinear Network}
\label{sec:unexplained_exp}

Based on our analysis, we draw parallels to two common observation in deep non-linear networks:\\

1) \textbf{Mild Sharpening in low complexity tasks:} The extent of sharpening in deep neural networks is often related to the complexity of the learning task. To illustrate this, we consider two commonly used tasks: regression and classification.\\
\textit{Regression Task}: In Figure \ref{fig:eos-dip}, we minimize the loss function $L(\boldsymbol{\theta})= \| G(\boldsymbol{\theta}) - \mbf{y}_{im} \|_{2}^2$, fitting an image $\mbf{y}_{im}$ using a deep image generator network like Unet $G(\boldsymbol{\theta})$, with Gradient Descent. We observe that the degree of sharpening in this network depends on the target image $\mbf{y}_{im}$. For example, when $\mbf{y}_{im}$ is a smooth, low-frequency image, the sharpness of the loss $ \| \nabla^2 L(\boldsymbol{\theta}) \|_{2}$ remains low. In contrast, when fitting a detailed image, such as white noise with high-frequency content, the sharpness increases and enters the EOS regime $\frac{2}{\eta}$. In particular,we observe a steady correlation between the sharpness rise (Figure-\ref{fig:eos-dip}) and the high frequency content of the fitting image (Figure-\ref{fig:img_used}). \\
\textit{Classification task}:  In Figure \ref{fig:small_Sharp}, we train a 2-layer fully connected neural network on $N$ pairs of labeled training images from the CIFAR-10 dataset using MSE loss. The sharpness of the loss is linked to $N$, the number of data points used for training. For small $N$ values, such as 100 or 200, the network learns only a limited set of latent features, resulting in mild sharpening, and the network does not reach the EOS threshold. However, when $N$ exceeds 1000, the sharpness increases and reaches the EOS threshold $\frac{2}{\eta}$. Furthermore, Figure-16 in \cite{cohen2021gradient} reported that sharpness also increases with depth of the network. So, the sharpness limit correlates both with network depth and complexity of the learning problem. \\
These two occurences in non-linear network is partially addressed by our analysis of deep matrix factorization at EOS. We show that sharpness rises to $L\sigma^{2-\frac{2}{L}}_{1}$, where $\sigma_{1}$ is the top singular value of the target matrix and $L$ is the depth. In deep matrix factorization problem, $\sigma_{1}$ corresponds to the magnitude of the strongest feature in the data and is related to the complexity of learning. Whenever, $L\sigma^{2-\frac{2}{L}}_{1}<\frac{2}{\eta}$, the network do not enter the EOS regime (Figure-\ref{fig:dln_mild_sharpening}). Similarly, in both regression and classification experiments in Figure \ref{fig:combined_figures}, whenever data has low complexity, sharpness do not rises and network fails to reach EOS. Furthermore, sharpness $L\sigma^{2-\frac{2}{L}}_{1}$ scales with depth of the network $L$, supporting the observation by \cite{cohen2021gradient}.

2) \textbf{Oscillation range in strong feature direction:}
\end{comment}

\begin{figure}[t!]    
\centering
    \begin{subfigure}[t]{0.32\textwidth} % Subfigure (a) - increased size
        \centering
        \includesvg[width=\textwidth]{figures/dip_eos/eos.svg}
        \caption{Sharpness plots for training image generator networks using SGD with learning rate $\eta = 2^{-4}$.}
        \label{fig:eos-dip}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.32\textwidth} % Subfigure (b) - increased size
        \centering
        \includesvg[width=\textwidth]{figures/dip_eos/img_used.svg}
        \caption{Target images (denoted as $\mbf{y}_{\mathrm{image}}$) with different frequencies used for training.}
        \label{fig:img_used}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.32\textwidth} % Subfigure (c) - increased size
        \centering
        \includegraphics[width=\textwidth]{figures/small_sharpness.png}
        \caption{2-layer FC network trained with small number $N$ of CIFAR-10 dataset with $\eta=1e-2$}
        \label{fig:small_Sharp}
    \end{subfigure}
    \caption{Illustration of Caveat 2 by~\cite{cohen2021gradient} on how mild sharpening occurs on simple datasets and network. (a) Regression task showing the evolution of the sharpness when an UNet (with fixed initialization) is trained to fit a single image shown in (b). (c) Evolution of the minimal progressive sharpening on a classification task of a 2-layer MLP trained on a  subset of CIFAR-10.}
    \label{fig:combined_figures}
\end{figure}

\begin{comment}

\subsection{Difference of EOS dynamics in non-linear networks and deep matrix factorization }

Although mild sharpening and strong directional oscillation phenomenon is partially explained from analyzing deep matrix factorization, we highlight some critical differences between EOS dynamics in non-linear networks and liner networks:

\begin{itemize}
    \item \textbf{Sustained oscillation in DMFs vs catapaults in non-linear networks}: In deep matrix factorization (DMF) loss whenever $\eta > \frac{2}{L \sigma_{1}^{2-\frac{2}{L}}}$, we observe free oscillation in 2-period orbit \footnote{At higher learning rate, iterates enter higher period orbit oscillations, chaos and divergence}. However, in nonlinear networks we observe catapaults or sudden spikes. This is primarily because of difference in loss landscape. At global minima, Hessian of the loss in DMF is provably Positive Semi-Definite (PSD)\footnote{we explicitly derived all positive eigenvalues}. So there are only directions of positive curvature and flat directions (in null space of the Hessian). In this landscape,\textit{ oscillations occur due to bouncing of the basin of the wall with no direction of escape.} But in deep non-linear networks, it is has been frequently observed that the Hessian at the minima has negative eigenvalues \cite{ghorbani2019investigation,sagun2016eigenvalues}. This enables an escape direction in the direction of the negative curvature preventing sustained/free oscillation. We believe understanding the role of non-linear activation layers in changing this loss landscape is the key to address this difference.
    \item \textbf{Absence of self-stabilization effect \cite{damian2023selfstabilization} in deep matrix factorization}
    Damian et al. studied self-stabilization, where sharpness decreases below $\frac{2}{\eta}$ after exceeding $\frac{2}{\eta}$. They assume that $\nabla L(\theta) \cdot u(\theta) = 0$ and $\nabla S(\theta)$ lie in the null-space of the Hessian. However, in deep linear networks, \textit{these assumptions are not satisfied}. Due to singular vector alignment and balancing, the dynamics reduce to a one-dimensional oscillating trajectory, where both $\nabla L(\theta)$ and $\nabla S(\theta)$ lie in the range space of the Hessian. Letting $\pi(\theta)$ represent the scalar product, $\nabla L(\theta) \cdot u(\theta) = (\pi(\theta) - s)\pi(\theta)|w^{-1}|$, which isn't zero unless the loss is zero (not the case in EoS). Hence, in deep linear networks, self-stabilization does not occur, and the iterates and sharpness oscillate above $\frac{2}{\eta}$.

\end{itemize}
\end{comment}
\section{Conclusion, Limitations and Future Work}

In this paper, we presented a fine-grained analysis of the learning dynamics of deep matrix factorization with the aim of understanding unexplained phenomena in deep nonlinear networks within the EOS regime. Our analysis revealed that within EOS, DLNs exhibit periodic oscillations in small subspaces, where the subspace dimension is exactly characterized by the learning rate. 
%This allowed us to explain phenomena such as mild sharpening, oscillations occurring only within the top singular values, and to distinguish the differences between the behaviors of DLNs and diagonal linear networks. 

There are two limitations to our work: (i) we require that the dynamics converge to the singular vector stationary set, and (ii) we require strict balancing of the singular values. Regarding the singular vector stationary set, we leave it for future work to analyze cases where initialization occurs outside the singular vector stationary set, which requires jointly analyzing the oscillation in both singular vectors and singular values. It should be noted, however, that the oscillations largely occur due to the singular values, so our results still accurately capture the behavior of DLNs at EOS.
As for balancing, there may exist cases where oscillations begin before strict balance is achieved. We leave it to future work to find subspace oscillations without assuming strict balancing before oscillation starts.


==> ICLR/text_after_sub/intro.tex <==
\section{Introduction}

Understanding generalization in deep neural networks requires an understanding of the optimization process in gradient descent (GD).
In the literature, it has been empirically observed that the learning rate $\eta$ plays a key role in driving generalization~\citep{hayou2024lora,lewkowycz2020large}.%, with larger learning rates often leading to better generalization performance. 
The ``descent lemma'' from classical optimization theory says that for a $\beta$-smooth loss $\mathcal{L}(\mathbf{\Theta})$ parameterized by $\mathbf{\Theta}$, gradient descent (GD) iterates satisfy
\begin{align*}
    \mathcal{L}(\mathbf{\Theta}(t+1)) \leq \mathcal{L}(\mathbf{\Theta}(t)) - \frac{\eta(2-\eta \beta)}{2} \|  \nabla \mathcal{L}(\mathbf{\Theta}(t)) \|_{2}^2,
\end{align*}
and so the learning rate should be chosen as $\eta < 2/\beta$ to monotonically decrease the loss.
%However, classical optimization theory on GD restricts itself to small infinitesimal learning rate and unrealistic convergence assumptions which barely holds for training deep networks in practice. Traditional analysis of GD show that for $L$-smooth loss, only if the step-size $\eta$ is selected to be less than $\frac{2}{L}$, the training is stable and the loss decreases monotonically.
However, many recent works have shown that the training loss decreases even for $\eta > 2/\beta$, albeit non-monotonically.
Surprisingly, it has been observed that choosing such a learning rate often provides better generalization over smaller ones that lie within the stability threshold. This observation has led to a series of works analyzing the behavior of GD within a regime dubbed ``the edge of stability'' (EOS). By letting $\mbf{\Theta}$ be a deep network, we formally define EOS as follows:
%Consider GD is run with learning rate $\eta$ to minimize a loss $l(\mbf{\theta})$ with a deep network. \cite{cohen2021gradient} observed a surprising and a commonly occuring phenomenon in deep networks coined "Edge of Stability" which is formally defined:
\begin{definition}[Edge of Stability~\citep{cohen2021gradient}]
During training, the sharpness of the loss, defined as $S(\mbf{\Theta}):= \| \nabla^2 \mathcal{L}(\mbf{\Theta})\|_{2}$, continues to grow until it reaches $2/\eta$, after which it stabilizes around $2/\eta$. During this process, the training loss behaves non-monotonically over short timescales but consistently decreases over long timescales.
\end{definition}

Using a large learning rate to operate within the EOS regime is hypothesized to give better generalization performance by inducing ``catapults'' in the training loss~\citep{zhu2023catapults}. Intuitively, whenever the sharpness $S(\mbf{\Theta})$ exceeds the local stability limit $2/\eta$, the GD iterates momentarily diverge (or catapults) out of a sharp region and self-stabilizes~\citep{damian2023selfstabilization} to settle for a flatter region where the sharpness is below $2/\eta$, which is known to generalize better~\citep{keskar2017on, izmailov2019averaging, petzka2021relative, foret2021sharpnessaware, gatmiry2023inductive}. Of course, the dynamics within EOS differ based on the loss landscape. For example, as illustrated in Figure~\ref{fig:catapults_vs_osc}, when the loss landscape is highly non-convex with many local valleys, catapults may occur, whereas sustained oscillations may exist for ``nicer'' landscapes. It is of great interest to understand the behaviors of such oscillations (or catapults) within different network architectures to further our understanding of EOS and how these behaviors can lead to better generalization.

From a theoretical perspective, there have been many recent efforts to understand EOS. These works generally focus on analyzing ``simple'' functions, examples including scalar losses \citep{minimal_eos,wang2023good,kreisler2023gradient}, quadratic regression models \citep{agarwala2022second}, diagonal linear networks \citep{even2024s} and two-layer matrix factorization \citep{chen2023edge}. 
However, the simplicity of these functions cannot fully capture the behaviors of deep neural networks within the EOS regime. Specifically, the following observations remain unexplained by existing analyses: (i) mild (or no) sharpening occurs when deep networks are trained using ``simple'' datasets~(Caveat 2 from~\citep{cohen2021gradient}); (ii) the oscillations and catapults in the weights occur within a low-rank subspace or within the top singular values of each weight matrix~\citep{zhu2024catapultssgdspikestraining}; and (iii) the oscillations are stronger within weight subspaces that generate more prominent features in the output fitting the data. For example, \cite{zhu2024catapultssgdspikestraining} observed that large catapults occurred within the top eigenspace of the NTK, followed by mild (or no) catapults in the complementary space, and \cite{rosenfeld2024outliers} showed that network inputs with large-magnitude features and strong opposing signals oscillate with larger spikes for those particular inputs.%
%\qq{need to discuss the limitation of previous results, especially for the last part} \smk{actually the limitation is that they cannot explain the phenomena}


\begin{comment}
    
These works developed our understanding of EOS but are far from capturing EOS dynamics occuring in deep neural networks. The formulation of deep neural networks is very close to deep matrix factorization problem which only exempts the use of non-linear activations and with a practical assumption that the underlying data is low rank. However, existing literature in deep matrix factorization focused on gradient flow dynamics \cite{arora2019implicit,saxe2014exact} or GD operating in the stable regime \cite{chou2024gradient,gidel} where training loss decreases monotoncally. We enlist important observations made while training deep network in the EOS regime which are currently unexplained by existing analysis in the literature:

\begin{enumerate}
\item  (Obs-1:) \textbf{Mild-sharpening} or no sharpening occurs 1) when deep networks are trained to fit \textit{simple} datasets (Caveat-2 \cite{cohen2021gradient}) (refer Figure) or 2) when the depth of the network is small.  % 
\item (Obs-2:) \textbf{Subspace Oscillation}: Oscillation/catapaults in the weight space occurs in a low rank subspace or within the top few sinuglar values of weight matrix in each layer \cite{zhu2024catapultssgdspikestraining}, hence preserving \textit{structure amidst chaos}.%
\item (Obs-3:) \textbf{Stronger oscillations} occur along weight subspace that generates prominent features in the output fitting the data. \cite{zhu2024catapultssgdspikestraining} observed that large catapaults occured in the top eigenspace of the NTK followed by mild/no catapaults in complementary space. \cite{rosenfeld2024outliers} showed that network inputs with large magnitude features and strong opposing signals oscillate with larger spikes for that particular input. %
\end{enumerate}

Our analysis of EOS on deep matrix factorization aims at explaining these 3 key observations and thereby attempting to bridge the gap between theory and practice. But before understanding EOS dynamics, it is important to understand gradient flow dynamics in deep matrix factorization. 
\end{comment}

\begin{figure}[t!]
    \centering
     \begin{subfigure}[b]{0.2475\textwidth}
         \centering
        \includegraphics[width=\textwidth]{figures/intro/dln_train_loss.pdf}
        \caption{Linear Networks}
     \end{subfigure}
     \begin{subfigure}[b]{0.2475\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/intro/mlp_train_loss.pdf}
         \caption{ReLU Networks}
     \end{subfigure}
        \begin{subfigure}[b]{0.475\textwidth}
         \centering
         \includegraphics[width=0.95\textwidth]{figures/intro/lora_osc.pdf}
         \caption{BERT using LoRA}
     \end{subfigure}
     \vspace{-0.1in}
    \caption{Illustration of instability in the training loss for different network architectures. When the loss landscape is more complex with many local valleys (b, c), catapults occur, whereas free/sustained oscillation occur in (a). Parts with oscillations/catapults are zoomed in.}
    
    \label{fig:catapults_vs_osc}
\end{figure}

In this work, we attempt to bridge the gap between theory and practice by providing a fine-grained analysis of the learning dynamics of deep linear networks (DLNs) within the EOS regime. DLNs share many characteristics with their nonlinear counterparts, making them a useful surrogate for analyzing behaviors in deep neural networks~\citep{wang2024understandingdeeprepresentationlearning, zhang2024when}. For example,~\cite{zhang2024when} has provably shown that bias-free ReLU networks behave similarly to linear networks.
Generally, existing works on DLNs focus on analyzing the effect of depth and the initialization scale, and how they implicitly bias the trajectory of gradient flow towards low-rank solutions when the learning rate is chosen to be stable~\citep{saxe2014exact, arora2018optimization, implicit_dmf, zhang2024structure, pesme2023saddle, jacot2022saddletosaddle}.
Our analysis builds upon these works to show that DLNs exhibit intricate and interesting behaviors outside the stability regime. Our main contributions can be summarized as follows: 
%particularly periodic oscillations within a small subspace, where the subspace dimension is precisely characterized by the step size. 
%\qq{need a short title for each bullet point}
\vspace{-0.1in}
\begin{itemize}
\item \textbf{Periodic Subspace Oscillations.} We show that there exist periodic oscillations within $r$-dimensional subspaces in DLNs, where the rank $r$ is precisely characterized by the learning rate. This effectively explains why oscillations occur within top subspaces as observed by~\cite{zhu2023catapults}. We also prove that the learning rate needed to enter EOS is a function of the network depth, further revealing the role of depth in deep networks.
\item \textbf{Difference in DLNs and Diagonal Linear Networks.} We prove that the behavior of DLNs and  diagonal linear networks differ within the EOS regime. This also provides a unique perspective on how the landscape changes between the two networks, despite its similarities.
\item \textbf{Catapults in LoRA.} Lastly, we empirically demonstrate how oscillations and catapults may occur in different network architectures and their effects. We show that, for a sufficiently large learning rate, updating low-rank adaptors (LoRA) \citep{hu2022lora} during the fine-tuning of LLMs can drive the entire network into the EOS regime, where catapults can potentially improve generalization.
    %\item  The dynamics in deep matrix factorization and diagonal linear networks differ in the EOS regime, unlike in gradient flow (GF). These dynamics depend on the dimensionality of the layers (whether vector in diagonal linear networks, matrix in deep matrix factorization, or tensor in tensor factorization), which is not the case in GF.
    %\item  We prove that in deep linear networks, only the depth and the largest singular value of the target matrix determine whether the network will operate in the EOS regime.
    %\item The condition to enter the EOS regime is independent of the initialization scale and the dimensionality of the layers, dimension the rank of the target matrix. 
\end{itemize}

\begin{comment}
    
\subsection{Implicit regularization in deep linear models with gradient flow}
Over the past few years, several works have analyzed the effect of depth and initialization in deep linear networks \cite{saxe2014exact, arora2018optimization, implicit_dmf, zhang2024structure}. It has been observed that small initialization and larger depth make the trajectory of gradient flow implicitly biased towards low-rank solutions. Similar observations have been made in diagonal linear networks \cite{woodworth2020kernel, pesme2021implicit}, where the scale of initialization determines whether the dynamics of the iterates are in the rich regime or the kernel regime. Smaller initialization promotes rich regime dynamics, where features are learned incrementally through saddle-to-saddle dynamics \cite{pesme2023saddle, jacot2022saddletosaddle}. Larger depth increases the duration of these saddle points and has a stronger implicit bias towards exact low-rank solutions by suppressing the residual singular values through the depth factor \cite{arora2018optimization}. In deep matrix factorization gradient flow aligns the singular vectors of successive layer factors \cite{du2018algorithmic}. 

Due to this alignment, the flow dynamics in deep matrix factorization are the same as those in deep linear networks, but act on the singular values of the matrices.

Our analysis and experiments reveal certain surprising (yet explainable) phenoemons that is critical to understand Edge of Stability:

\begin{itemize}
    \item  The dynamics in deep matrix factorization and diagonal linear networks (or even tensor factorization) differ in the EOS regime, unlike in gradient flow (GF). These dynamics depend on the dimensionality of the layers (whether vector in diagonal linear networks, matrix in deep matrix factorization, or tensor in tensor factorization), which is not the case in GF.
    \item  We prove that in deep linear networks, only the depth and the largest singular value of the target matrix determine whether the network will operate in the EOS regime.
    \item The condition to enter the EOS regime is independent of the initialization scale and the dimensionality of the layers, dimension the rank of the target matrix. 
\end{itemize}


\ag{I am unsure whether it is better to state it after notations otherwise it will be a reptitition. Probably we should state this in the contribution section?}


\end{comment}





%\paragraph{Related Works.} We briefly survey a few related works to highlight their differences, and provide a detailed discussion in \Cref{app:related}. 
%    DLNs are often used as prototypes to study the behaviors of nonlinear networks~\citep{benign, saxe2014exact, wang2024understanding, nc}. The most relevant literature on DLNs are those by Yaras et al.~\citep{yaras2023law, yaras2024compressible} and Kwon et al.~\citep{kwon}, who reveal that the weight updates of deep networks occur within an invariant subspace. Our work differs from that of Yaras et al.~\citep{yaras2023law} in that we fully capture the learning dynamics of DLNs throughout the entire GD process. While Kwon et al.~\citep{kwon} observe invariant weight updates, they use this observation for model compression and do not study the learning dynamics with large learning rates. Regarding the edge of stability, the most relevant works are those that analyze scalar functions to demonstrate that the edge of stability occurs on such functions, which have a non-zero third-order derivative and satisfy certain regularity conditions~\citep{chen2023edge,wang2023good,minimal_eos}. However, as mentioned previously, these works do not capture the more complicated models that we consider in this work.


\section{Notation and Problem Setup}

%\qq{we need to be consistent, some place we call it deep linear networks, other places we call it deep matrix factorization. Let us call it "deep linear network", and training loss for DLN}

\paragraph{Notation.}
We denote vectors with bold lower-case letters (e.g., $\mbf{x}$)
and matrices with bold upper-case letters (e.g., $\mbf{X}$).
%Given any $n \in \N$,
We use $\mbf{I}_n$ to denote an identity matrix of size $n \in \N$.
We use $[L]$ to denote the set $\{1, 2, \ldots, L\}$. 
We use the notation $\sigma_i(\mbf{A})$ to denote the $i$-th singular value of the matrix $\mbf{A}$.

\begin{comment}
\paragraph{Deep linear model}
Consider the problem of least squares fitting problem with multidimensional output. We want to learn a mapping $f(.):\mbb{R}^{d}\rightarrow \mbb{R}^{d}  $ given $d$ number of input vectors $\mbf{x}_{i} \in \mbb{R}^{d}$ to same number of target vector $\mbf{y}_{i} \in \mbb{R}^{d}$. Considering $f(.)$ to be deep linear model with set of parameters  $\mbf{\Theta} = \left(\mbf{W}_1, \mbf{W}_2, \ldots, \mbf{W}_L \right)$, then the fitting regression problem can be formulated as minimizing the loss wrt $\frac{1}{2} \|\mbf{Y} - \mbf{X} \mbf{W}_L \cdot \ldots \cdot \mbf{W}_1\|^2_{F} $ where $\mbf{X}$ and $\mbf{Y}$ are column stacking of the input  $\left\{\mathbf{x}_{i}\right\}_{i=1}^d$ and target $ \left\{\mathbf{y}_{i}\right\}_{i=1}^d$. Assuming the data matrix $\mbf{X}$ to be whitened matrix with dominant features such that $\mbf{X}^T \mbf{Y} = \mbf{M}$ (say) is low rank, then the optimization can be formulated as a low rank recovery problem. Throughout the paper, we will restrict ourselves to analyze the deep matrix factorization problem, which we introduce next.
\end{comment}


 \paragraph{Deep Matrix Factorization Loss.}
The objective in deep matrix factorization is to model a low-rank matrix $\mbf{M}_\star \in \mbb{R}^{d\times d}$ with $\rank(\mbf{M}_\star) = r$ via a DLN parameterized by a set of parameters $\mbf{\Theta} = \left(\mbf{W}_1, \mbf{W}_2, \ldots, \mbf{W}_L \right)$, which can be estimated by solving
\begin{align}\label{eqn:deep_mf}
    \underset{\mbf{\Theta}}{\rm{arg min}} \, f(\mbf{\Theta}) \coloneqq \frac{1}{2}\|\underbrace{\mbf{W}_L \cdot \ldots \cdot \mbf{W}_1}_{\eqqcolon \mbf{W}_{L:1}} - \mbf{M}_\star\|^2_{\mathsf{F}},
\end{align}
where we adopt the abbreviation $\mbf{W}_{j:i} = \mbf{W}_{j}\cdot \ldots \cdot \mbf{W}_i$ to denote the end-to-end DLN and is identity when $j < i$. We assume that each weight matrix has dimensions $\mbf{W}_\ell \in \mbb{R}^{d\times d}$ to observe the effects of overparameterization.





\paragraph{Optimization.}
We update each weight matrix $\mbf W_\ell \in \mbb{R}^{d\times d}$ using GD with iterations given by
\begin{align}\label{eqn:gd}
    \mbf{W}_\ell(t) = \mbf{W}_\ell(t-1) - \eta\cdot \nabla_{\mbf{W}_\ell}f(\mbf{\Theta}(t-1)), \quad \forall \ell \in [L],
\end{align}
where $\eta > 0$ is the learning rate and $\nabla_{\mbf{W}_\ell}f(\mbf{\Theta}(t))$ is the gradient of $f(\mbf{\Theta})$ with respect to the $\ell$-th weight matrix at the $t$-th GD iterate. We initialize the network as the following:
\begin{align}\label{eqn:init}
    \mbf{W}_L(0) = \mbf{0}, \quad \quad\quad \mbf{W}_\ell(0) = \alpha \mbf{I}_d, \quad \forall \ell \in [L-1],
\end{align}
where $\alpha > 0$ is a small constant. The zero weight layer can be viewed as the limiting case of initializing the weights with a (very) small constant $\alpha' \ll \alpha$, and has been similarly explored by~\cite{two_layer_bias}, albeit for two-layer networks. 

Previous works on both shallow and deep linear networks assume a zero-balanced initialization (i.e., $\mbf{W}_i^\top(0)\mbf{W}_i(0) = \mbf{W}_j(0)\mbf{W}^\top_j(0)$ for $i \neq j$). This introduces the invariant $\mbf{W}_i^\top(t)\mbf{W}_i(t) = \mbf{W}_j(t)\mbf{W}^\top_j(t)$ for all $t > 0$, ensuring two (degenerate) conditions throughout the training trajectory: (i) the singular vectors of each of the layers remain aligned and (ii) the singular values stay balanced.

Our initialization lifts condition (ii). 
Rather than staying balanced, we show that the singular values become increasingly balanced (see Lemma~\ref{lemma:balancing}).
We also show that our analysis is not limited to this specific initialization but applies to \emph{any initialization} that converges to the singular vector stationary set (see Proposition~\ref{prop:svs_set}). To the best of our knowledge, it is common to assume that the singular vectors remain aligned, as many existing works make the same assumption~\citep{two_layer_bias, implicit_dmf, saxe2014exact, gidel,chou2024gradient, kwon}. 



%In the following section (as well as Appendix~\ref{sec:additional_exp}), we provide examples of such initializations, which we adopt for our analyses as well.



%\smk{I am pretty adamant that we should have this section like this; it has clear motivation.} \ag{Slightly debatable, but let's hear opinions of others. }
%\ag{@Qing: would it be better if we specify the general class of initialization instead of the zero-one initilaization in the main text?}\smk{Note that we never prove that any initialization belongs in the SVS set! And we need to then change all of our proofs to be $\mbf{Q}$ orthogonal matrices rather than the target matrix $\mbf{V}$ like we have now.}
 % For deep linear networks, it is common to use an orthogonal-type initialization rather than a random one~\citep{kwon, kwon2024on, yaras2023law}, as it has been provably shown that random initialization slows down convergence~\citep{Hu2020Provable}.

==> ICLR/text_after_sub/theory.tex <==
 \section{Deep Matrix Factorization Beyond the Edge of Stability}




\begin{figure}[t!]
    \centering
    \includegraphics[width=\textwidth]{figures/dln_ps_eos_lr172.pdf}
    \caption{Depiction of the two phases of learning in the deep matrix factorization problem for a network of depth $3$. It appears that upon escaping the first saddle point, the GD iterates enter the edge of stability regime, where the sharpness hovers just above $2/\eta$ when the learning rate is chosen to be above $2/\|\nabla^2 f(\mbf{\Theta})\|_2$ at convergence.
    }
    \label{fig:ps_eos}
\end{figure}

When using a large learning rate, the learning dynamics can typically be separated into two distinct stages: (i) progressive sharpening and (ii) the edge of stability. Within the progressive sharpening stage, the sharpness lies below $2/\eta$ and tends to continually rise. In the edge of stability regime, the sharpess hovers just above $2/\eta$, and the training loss oscillates
over short timescales, yet consistently decreases over long timescales~\citep{cohen2021gradient}. Our goal is to analyze the EOS stage under the deep matrix factorization formulation, with the aim of understanding phenomena that arise in DLNs. Our result extends the theoritical findings of \cite{chen2023edge}, where the authors proved the existence of a certain class of scalar functions \( f(x) \) for which gradient descent (GD) does not diverge even when operating beyond the stability threshold \( \eta > \frac{2}{f^{''}(\hat{x})} \), where \( \hat{x} \) is a local minimum of \( f(x) \). Specifically, the authors showed that there exists a range \( \eta \in \left( \frac{2}{f^{''}(\hat{x})}, \frac{2}{f^{''}(\hat{x})}(1+\epsilon) \right) \), with a function-dependent \( \epsilon > 0 \), where the loss oscillates around the local minima $(\hat{x})$ with a certain periodicity. As \( \eta \) increases beyond \( \frac{2}{f^{''}(\hat{x})} \), the oscillations gradually enter higher periodic orbits (e.g., 2, 4, 8 periods), then transition into chaotic behavior, and ultimately lead to divergence. In our work, we prove that this oscillatory behaviour beyond the stability threshold occurs even for deep linear networks. Our key observation is that due to two specific implicit bias of GD namely 1) singular vector alignment and 2) balancing, stable oscillations takes place in the top $r$ eigenvectors of the Hessian of the loss, where $r$ is dependent on $\eta$. 
Throughout the analysis, we only limit ourselves to analyzing two periodic orbit oscillation (Figure~\ref{fig:ps_eos}) and show higher period oscillations in the appendix.

%Here, we observe that the training loss oscillates in a two-period orbit rather than decreasing over iterations, as illustrated in Figure~\ref{fig:ps_eos} and rigorously shown in the following sections.


\subsection{Main Results}
In this section, we present our main results rigorously describing the learning dynamics of DLNs in the edge of stability regime. Before doing so, we give a proof brief sketch on how we analyze EOS for deep linear networks:

\begin{itemize}
    \item We state the two implicit biases of GD in deep matrix factorization in Proposition~\ref{prop:svs_set} and Lemma~ \ref{lemma:balancing}. These allows us to find the local minima in the non-convex problem and find the eigenvectors and eigenvalues of the Hessian. 
   \item We prove that oscillation in each eigenvector direction satisfies the stable oscillation condition which we prove in Theorem-\ref{thm:stable_oscillations}. We also show the existence and uniqueness of two point fixed period orbit along each eigenvector direction in Theorem~\ref{thm:align_thm}. 
\end{itemize}


\subsection{Tools used in the Analyses}

This section presents the two main tools used in our analyses: the singular vector stationary set and balancedness. First, we present the singular vector stationary set, which allows us to encompass a wider range of initialization schemes. This set defines a broad class of initialization for which singular vector alignment occurs, simplifying the dynamics to only singular values.

\begin{proposition}[Singular Vector Stationary Set]
\label{prop:svs_set}
Consider the deep matrix factorization loss in Equation~(\ref{eqn:deep_mf}). Let $\mbf{M}_\star = \mbf{U}_\star \mbf{\Sigma}_\star \mbf{V}_\star^\top$ and 
$\mbf{W}_\ell(t) = \mbf{U}_\ell(t) \mbf{\Sigma}_\ell(t) \mbf{V}_\ell(t)^\top$ denote the compact SVD for the target matrix and the $\ell$-th weight matrix at time $t$, respectively. Then the set of all time stationary points $\dot{\mbf{U}}_\ell(t) = \dot{\mbf{V}}_\ell(t) = 0$ for all $\ell \in [L]$ are given by
\begin{align*}
\mathrm{SVS}(f(\mbf{\Theta})) = 
\begin{cases}
    (\mbf{U}_L, \mbf{V}_L) &= (\mbf{U}_\star, \mbf{Q}_L), \\
    (\mbf{U}_\ell, \mbf{V}_\ell) &= (\mbf{Q}_{\ell+1}, \mbf{Q}_\ell), \quad\forall \ell \in [2, L-1], \\
    (\mbf{U}_1, \mbf{V}_1) &= (\mbf{Q}_2, \mbf{V}_\star),
\end{cases}
\end{align*}
where \(\{\mbf{Q}_\ell\}_{\ell=2}^{L}\) are any set of orthogonal matrices. 
\end{proposition}


The singular vector stationary set states that for any set of weights where the gradients with respect to the singular vectors become zero, the singular vectors become fixed points for subsequent iterations. Once the singular vectors become stationary, running GD further isolates the dynamics on the singular values. Hence, throughout our analysis, we re-write and consider the loss 
\begin{align}\label{eqn:simplified_loss}
    \frac{1}{2} \left\|\mbf{W}_{L:1}(t) - \mbf{M}^\star\right\|^2_{\mathsf{F}} = \frac{1}{2} \|\mbf{\Sigma}_{L:1} - \mbf{\Sigma}^\star\|^2_{\mathsf{F}} = \frac{1}{2} \sum_{i=1}^r \left(\sigma_i(\mbf{\Sigma}_{L:1}(t)) - \sigma_{\star, i}\right)^2,
\end{align}
where $\mbf{\Sigma}_{L:1}$ are the singular values of $\mbf{W}_{L:1}$. This allows us to decouple the dynamics of the singular vectors and singular values, focusing on the periodicity that occurs in the singular values within the EOS regime. In Proposition~\ref{prop:one_zero_svs_set}, we prove that the one-zero initialization we consider belongs to the singular vector stationary set with an illustration in Figure~\ref{fig:svec_alignment}.
In Appendix~\ref{sec:additional_exp}, we provide additional examples of initialization that belong to this set. Next, we present a result to validate our use of the strictly balanced assumption by showing that the singular values become increasingly balanced throughout the GD iterations.

\begin{lemma}[Balancing]
\label{lemma:balancing}
    Suppose we run GD on the deep matrix factorization loss in Equation~(\ref{eqn:deep_mf}) with learning rate $\eta < \frac{2\sqrt{2}}{L \sigma^{2-\frac{2}{L}}_{\star,1}}$, where $\sigma_{\star, 1}$ is the first singular value of $\mbf{M}_\star \in \mbb{R}^{d\times d}$. Let $\sigma_{i,\ell}$ denote the $i$-th singular value of the $\ell$-th layer matrix.  If the initialization scale $\alpha$ satisfies
    $0< \alpha < \left( \log\left( \frac{2\sqrt{2}}{\eta L \sigma_{\star, 1}^{2 - \frac{2}{L}}} \right) \cdot 2 \sigma_{\star, 1}^{\frac{4}{L}} \right)^{\frac{1}{4}}$,  we have $| \sigma^2_{i,L}(t+1) - \sigma^2_{i,\ell}(t+1)| < | \sigma^2_{i,L}(t) - \sigma^2_{i,\ell}(t)|$. 
\end{lemma}


\begin{definition}[Strict Balanced State]
    The parameters $\mbf{\Theta}$ in the deep matrix factorization loss are said to be in a strict balanced state if the singular values of the top $r$ indices for each layer are the same. Specifically, for all $1 \leq i \leq r$ and for all layers $\ell, k = 1, 2, \dots, L$, we have $\sigma_{i}(\mbf{W_{\ell}}) = \sigma_{i}(\mbf{W_{k}})$, where $\sigma_{i}(\mbf{W_{\ell}})$ denotes the $i$-th singular value of the $\ell$-th layer.
\end{definition}

\begin{lemma}[Eigenvalues of Hessian at Convergence]
\label{lemma:hessian_eigvals}
    Consider running GD on the deep matrix factorization loss $f(\mbf{\Theta})$ defined in Equation~(\ref{eqn:deep_mf}). Under  strict balancing with any stationary point $\Theta$ with $\nabla_{\mbf{\Theta}} f(\mbf{\Theta}) = 0$, the non-zero eigenvalues of the training loss Hessian are given by
    \begin{align*}
        \lambda_{\mbf{\Theta}} = \left\{\sum_{\ell=0}^{L-1} \left(\sigma_{\star, i}^{1-\frac{1}{L} - \frac{1}{L}\ell} \cdot \sigma_{\star, j}^{\frac{1}{L}\ell}\right)^2\right\}_{i,j = 1}^{r} \,\bigcup \, \,\left\{\sum_{\ell=0}^{L-1} \left(\sigma_{\star, k}^{1-\frac{1}{L} - \frac{1}{L}\ell} \cdot \alpha^{\ell}\right)^2\right\}_{k = 1}^{r} \, \bigcup \, \,\left\{\sigma_{\star, m}^{2-\frac{2}{L}}\right\}_{m=1}^r,
    \end{align*}
    where $\sigma_{\star, i}$ is the $i$-th singular value of the target matrix $\mbf{M}_\star \in \mbb{R}^{d\times d}$,  $\alpha \in \mbb{R}$ is the initialization scale, $L$ is the depth of the network, and the last set of eigenvalues each have a multiplicity of $d-r$.
\end{lemma}

We defer all of the proofs to Appendix~\ref{sec:proofs}. Since we are interested in analyzing the dynamics when the learning rate is $\eta > 2 / \|\nabla^2 f(\mbf{\Theta})\|_2$, we need to exactly quantify the sharpness value $\|\nabla^2 f(\mbf{\Theta})\|_2$. By Lemma~\ref{lemma:hessian_eigvals}, we can see that the sharpness is exactly $\|\nabla^2 f(\mbf{\Theta})\|_2 = L\sigma_{\star, 1}^{2- \frac{2}{L}}$, assuming strict balance. Hence, as long as $\eta$ is set to $\eta > 2 / L\sigma_{\star, 1}^{2- \frac{2}{L}}$, we will observe oscillations in the loss.

Interestingly, notice that all non-zero eigenvalues are a function of network depth. For a deeper network, the sharpness will be larger, implying that a smaller learning rate can be used to drive the DLN into EOS. This provides a unique perspective on how the learning rate should be chosen as networks become deeper. Next, we present our result on the dynamics of DLNs within EOS.

Lastly, notice that the Lemma~\ref{lemma:hessian_eigvals} was established under a strict balancing assumption, meaning the singular values across all weight matrices are the same in the EOS regime. In Lemma~\ref{lemma:balancing}, we show that as long as the initialization scale $\alpha$ satisfies the upper bound, the singular values do indeed become balanced as $t \to \infty$, but not necessarily before oscillation starts.
However, we validate with experimental results that the singular values become balanced even before entering the EOS regime, supporting the use of the strict balancing assumption.



\begin{comment}
    
Interestingly, Lemma~\ref{lemma:hessian_eigvals} also reveals that the loss landscape of DLNs differs from that of the widely studied diagonal linear networks. In diagonal linear networks, each eigenvalue is characterized by a coordinate of the target vector (which is equivalent to the singular values of the target matrix in DLNs), whereas in our case, there is a ``mixture'' of singular values in the eigenvalues that arise primarily from the off-diagonal terms. This presents a unique distinction between our analysis and those on diagonal networks~\citep{even2024s}.
Next, we present our main result on $2$-period subspace oscillations in the singular values of the DLN.
\end{comment}

\begin{theorem}[1-D Subspace Oscillation]
\label{thm:align_thm}
Suppose we run GD on the deep matrix factorization loss with learning rate $\eta = \frac{2}{K}$, where $\mathrm{max} \left\{ \sum_{\ell=0}^{L-1} \left(\sigma_{\star, 1}^{1-\frac{1}{L} - \frac{1}{L}\ell} \cdot \sigma_{\star, 2}^{\frac{1}{L}\ell}\right)^2,L\sigma_{\star, 1}^{2-\frac{2}{L}}/\sqrt{2}\right\}< K< L\sigma_{\star, 1}^{2-\frac{2}{L}}$ and with initialization scale $\alpha < \left( \log\left( \frac{2\sqrt{2}}{\eta L \sigma_{\star, 1}^{2 - \frac{2}{L}}} \right) \cdot 2 \sigma_{\star, 1}^{\frac{4}{L}} \right)^{\frac{1}{4}}$. Then, under strict balancing, each weight matrix $\mbf{W}_{\ell}(t) \in \mbb{R}^{d\times d}$ oscillates around the minima in a $2$-period fixed orbit as follows:
\begin{align*}
    \mbf{W}_L(t) &= \rho_i(t)\cdot \mbf{u}_{\star, 1}\mbf{v}_{\star, 1}^{\top} + \sum_{j=1}^r \sigma_{\star, i}\mbf{u}_{\star, j}\mbf{v}_{\star, j}^{\top}, \quad i = 1, 2, \\
    \mbf{W}_\ell(t) &= \rho_i(t) \cdot\mbf{v}_{\star, 1}\mbf{v}_{\star, 1}^{\top} + \sum_{j=1}^r \sigma_{\star, i}\mbf{v}_{\star, j}\mbf{v}_{\star, j}^{\top}, \quad i = 1, 2, \quad \forall\ell \in [L-1],
\end{align*}
where $\mbf{M}_\star = \mbf{U}_\star \mbf{\Sigma}_\star \mbf{V}_\star^\top$ denotes the SVD of the target matrix , $\rho_i(t) \in \{\rho_1, \rho_2\}$
and $\rho_1 \in \left(0, \sigma_{\star, 1}^{1/L}\right)$ and $\rho_2 \in \left(\sigma_{\star, 1}^{1/L}, (2\sigma_{\star, 1})^{1/L}\right)$ are the two real roots of the polynomial $g(\rho)=0$, where
\begin{align*}
    g(\rho) = \rho^L\frac{1+\left(1 + \eta L(\sigma_{\star, 1} - \rho^L)\cdot \rho^{L-2} \right)^{2L-1}}{1+\left(1 + \eta L(\sigma_{\star, 1} - \rho^L)\cdot \rho^{L-2} \right)^{L-1}} - \sigma_{\star, 1}.
\end{align*}
\end{theorem}

%\ag{Should we have the general oscillation as a lemma?
%Also where are we having the digoanl liner network oscillation?}
\paragraph{Remarks.} Let $\lambda_i$ denote the $i$-th largest eigenvalue of the training loss Hessian. In Theorem~\ref{thm:align_thm}, we showed that if the learning rate is chosen such that $\eta = \frac{2}{K}$ with $\lambda_2 < K< \lambda_1$ (assuming that $\lambda_2 > \lambda_1  / \sqrt{2}$), then the largest singular value of the DLN will undergo periodic oscillations, where the amplitude is governed by $\rho_1$ and $\rho_2$. This theoretically shows why (i) oscillations only occur within top subspaces of the network as observed by~\cite{zhu2023catapults} and (ii) oscillations are more prevalent in the direction of the stronger features (measured by the magnitude of the singular values). 



% For the initialization scale, we require an upper bound on $\alpha$ to satisfy the balancing condition in Lemma~\ref{lemma:balancing}.

To show oscillations in two or more subspaces, we can easily extend Theorem~\ref{thm:align_thm} and set the learning rate such that $\lambda_i \geq K > \lambda_{i+1}$ for $i \geq 2$. For example, to observe oscillations in the top-$2$ subspaces, one needs to set $\lambda_2 \geq K > \lambda_3$, according to the eigenvalues computed in Lemma~\ref{lemma:hessian_eigvals}. Since Theorem~\ref{thm:align_thm} already shows that there must exist real roots for $K < \lambda_1$, a more careful treatment of the range of $\rho_1$ and $\rho_2$ is needed to rigorously extend this to $r$-dimensional oscillations. The upper bound of learning rate $\eta< \frac{2\sqrt{2}}{L\sigma^{2-\frac{2}{L}}_{\star,1}}$ depends only on the top singular value $\sigma_{\star,1}$ for which balancing fails to hold in all scalar singular value losses. 
% Lastly, note that we implicitly assumed the learning rate is chosen below some divergence limit. We leave for future work the task of precisely quantifying the learning rate for divergence, in order to obtain a more accurate bound on which learning rates contribute to the EOS regime.

In the following, we demonstrate that it is indeed possible to observe oscillations in all $r$-dimensional subspaces. From Lemma~\ref{lemma:chen-bruna} (restated from~\cite{chen2023edge}), the necessary condition for stable two-period orbit is that $f_{\Delta_i}^{(3)}(x) \neq 0$ and $3[f_{\Delta_i}^{(3)}(x)]^2 - f_{\Delta_i}^{(2)}(x)f_{\Delta_i}^{(4)}(x) > 0$ around a local minima $x$, where $\Delta_i$ is the $i$-th eigenvector of the Hessian and $f_{\Delta_i}$ is the loss function restricted to the line $\{y: y=x+ t \Delta_i, t\in \mbb{R}\}$.
In Theorem~\ref{thm:stable_oscillations}, we prove that this condition holds for each eigenvector direction.
%it is possible to have $r$-dimensional oscillations as long as the learning rate is chosen correctly. 


\begin{theorem}[Stable Subspace Oscillations]
\label{thm:stable_oscillations}
    Consider running GD on the deep matrix factorization loss in Equation~(\ref{eqn:deep_mf}) and denote the SVD of the target matrix as  $\mbf{M}_\star = \mbf{U}_\star\mbf{\Sigma}_\star\mbf{V}^\top_\star $, with distinct singular values $\sigma_{\star, 1} > \ldots > \sigma_{\star, r}$. Let $\Delta_i$  denote the $i$-th eigenvector of the Hessian with unit norm, $\lambda_{i}$ the corresponding eigenvalue after strict balancing occurs and denote $f_{\Delta_i}$ as the 1-D function at the cross section of the loss landscape and the line
following the direction of $\Delta_i$ passing the minima.
Then, if the minima of $f_{\Delta_i}$ satisfy $f_{\Delta_i}^{(3)}>0$ and $3[f_{\Delta_i}^{(3)}]^2 - f_{\Delta_i}^{(2)}f_{\Delta_i}^{(4)} > 0$, then 2-period orbit oscillation occurs in direction of $\Delta_i$ if $\eta>\frac{2}{\lambda_{i}}$. 
\end{theorem}
%\paragraph{Remarks.} By adopting this proof technique, we show that both conditions are true in each eigenvector direction considered in Theorem~\ref{thm:stable_oscillations}. Hence, Theorem~\ref{thm:stable_oscillations} that it is possible to have $r$-dimensional oscillations as long as the learning rate is chosen correctly. 


\begin{figure}[t!]
    \centering
    \includegraphics[width=\textwidth]{figures/svector_alignment_diff_lr.png}
    \caption{Illustrations of the singular vector and value evolution of the end-to-end DLN. The singular vectors of the network remain static across all iterations, as suggested by the singular vector stationary set, regardless of the learning rate. The angle between the true singular vectors and those of the network remains aligned throughout. The first singular values undergo oscillations in the large $\eta$ regime, whereas they remain constant in the small $\eta$ regime.}
    \label{fig:svec_alignment}
\end{figure}

\vspace{-0.25in}



\begin{wrapfigure}{r}{0.385\textwidth}
  \begin{center}
    \includegraphics[width=\linewidth]{figures/balancing_gap.pdf}
    
  \end{center}
  \caption{Plot of $| \sigma^2_{i,L}(t) - \sigma^2_{i,\ell}(t)|$ for initialization scale $\alpha = 0.01$ showing strict balancing.}
\label{fig:balancing}
\end{wrapfigure}
Recall that by our initialization scheme, we initialize to $\sigma_{L, i}(0) = 0$ and $\sigma_{\ell, i}(0) = \alpha$ for all $\ell \in [L-1]$. By considering the singular value scalar loss in Equation~(\ref{eqn:simplified_loss}), the gradient with respect to each $\sigma_{\ell, i}(t)$ are all the same. Thus, except for $\sigma_{L, i}(t)$, all of the other singular values across all weight matrices remain balanced throughout all iterations of GD. Lemma~\ref{lemma:balancing} states that throughout the course of GD, as long as $\alpha$ is below a certain threshold, $\sigma_{L, i}(t)$ becomes increasingly balanced to the rest of the singular values regardless of the learning rate. Since the balancing gap strictly decreases and $| \sigma^2_{i,L} - \sigma^2_{i,\ell} |$ is lower bounded by zero, it converges to 0 as $t \to \infty$. In Figure~\ref{fig:balancing}, we show that the gap indeed goes to zero empirically, and this is consistently the case across all of our experiments, with additional results provided in Appendix~\ref{sec:additional_exp}. Also in Appendix~\ref{sec:additional_exp}, we show that even for a slightly larger initialization scale, the balancing still holds in practice. Furthermore, we note that very similar results for imbalanced initialization have been proven by~\cite{wang2021large}, where our result can be viewed as an extension to multiple variables.
Finally, by assuming strict balancing, we can simplify the loss even further, particularly in the form $\sigma_i(\mbf{\Sigma}_{L:1}(t)) = \sigma^L_{i}(t)$, which allows us to solely analyze the dynamics of the singular values within the EOS regime. 


%However, it is worth noting that (i)~Lemma~\ref{lemma:balancing} does not state that the difference goes to zero, but rather that it becomes increasingly balanced and (ii) the bound on $\alpha$ may be too conservative and is an artifact of our analysis. 








\begin{comment}
    
\begin{figure}[htbp]
    \centering
    \begin{minipage}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/deep_martix_figs/oscillation_ranges.png}
        \caption{Figure 1}
        \label{fig:figure1}
    \end{minipage}%
    \hfill
    \begin{minipage}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/deep_martix_figs/layer_1_singular_values_0.01546.png}
        \caption{$\eta=\frac{1}{L\sigma^{2-\frac{2}{L}}_{\star,1}}$}
        \label{fig:figure2}
    \end{minipage}%
    
    \vspace{0.5cm} % Adds some vertical space between rows

    \begin{minipage}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/deep_martix_figs/layer_1_singular_values_0.0167.png}
        \caption{$\eta=\frac{1}{\sum_{\ell=0}^{L-1} \left(\sigma_{\star, 1}^{1-\frac{1}{L} - \frac{1}{L}\ell} \cdot \sigma_{\star, 2}^{\frac{1}{L}\ell}\right)^2}$}
        \label{fig:figure3}
    \end{minipage}%
    \hfill
    \begin{minipage}[b]{0.45\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/deep_martix_figs/layer_1_singular_values_0.02.png}
        \caption{$\eta>\frac{1}{L\sigma^{2-\frac{2}{L}}_{\star,2}}$}
        \label{fig:figure4}
    \end{minipage}
    \caption{}
\end{figure}





\end{comment}







\subsection{Relation to Diagonal Linear Networks}
Due to singular vector stationarity and balancing, DLNs may appear equivalent to diagonal linear networks at first glance. In this section, we characterize an explicit distinction between the two networks by deriving the eigenvalues of diagonal linear networks from the Hessian at convergence and explaining how they contribute to periodic oscillations in the EOS regime.

\begin{theorem}[Subspace Oscillation for Diagonal Linear Networks]
\label{thm:diag_lin_thm}
Let $\mbf{s}_\star \in \mbb{R}^{d}$ be an $r$-sparse vector with ordered coordinates such that $s_{\star,1} >\ldots>s_{\star,d}$. 
%Denote $I$ as the support set of $\mbf{s}_\star \in \mbb{R}^d$, $I^{C}$ as its complementary set, and $P$ denote the set containing $p$ largest elements in  $\mbf{s}^\star$. 
Suppose we run GD (\ref{eqn:gd}) with learning rate $\eta = \frac{2}{K}$, where $L s_{\star,p}^{2-\frac{2}{L}}\geq K>L s_{\star,p+1}^{2-\frac{2}{L}}$
for any $p < r$ and $\frac{s_{\star, p}}{s_{\star, 1}}> (\frac{1}{2})^{\frac{1}{4-4/L}} $ on the loss 
\begin{align*}
        \mathcal{L}\left(\{\mbf{s}_\ell\}_{\ell=1}^L \right) \coloneqq \frac{1}{2} \|\mbf{s}_1 \odot \ldots \odot \mbf{s}_{L} - \mbf{s}_{\star}\|_2^2, 
 \end{align*}
 with initialization $\mbf{s}_\ell = \alpha  \mbf{1}_d$ for all $\ell \in [L-1]$ where $\alpha < \left( \log\left( \frac{2\sqrt{2}}{\eta L s_{\star, 1}^{2 - \frac{2}{L}}} \right) \cdot 2 s_{\star, 1}^{\frac{4}{L}} \right)^{\frac{1}{4}}$, and $\mbf{s}_{L}=\mbf{0}_d$. Then, under strict balancing, the top-$p$ coordinates of $\mbf{s}_\ell$ oscillate within a $2$-period fixed orbit around the minima in the form
 \begin{align*}
     s_{\ell, i}(t) = \rho_{i, j}(t), \quad \forall i < p,  \, \forall \ell \in [L],
 \end{align*}
where $\rho_{i, j}(t) \in\{\rho_{i, 1}, \rho_{i, 2}\}$, $\rho_{i, 1} \in \left(0, s_{\star, i}^{1/L} \right)$ and $\rho_{i, 2} \in \left(s_{\star, i}^{1/L}, (2s_{\star, i})^{1/L} \right)$ are two real roots of the polynomial $h(\rho)=0$:
\begin{align*}
    h(\rho) = \rho^L\frac{1+\left(1 + \eta L(s_{\star,i}  - \rho^L)\cdot \rho^{L-2} \right)^{2L-1}}{1+\left(1 + \eta L(s_{\star,i}  - \rho^L)\cdot \rho^{L-2} \right)^{L-1}}- s_{\star,i}.
\end{align*}

\end{theorem}
\paragraph{Remarks.}

Similar to Theorem~\ref{thm:align_thm}, each coordinate of the diagonal linear network undergoes periodic oscillations as long as the learning rate is set to $\eta > 2/\lambda_1$, where $\lambda_1$ is the largest eigenvalue of the training loss Hessian. However, as shown in the proof of Theorem~\ref{thm:diag_lin_thm}, the main difference lies in the eigenvalues themselves -- the non-zero eigenvalue set of the diagonal linear network is much smaller than those of the DLN. For example, the top two eigenvalues of the diagonal linear network are $L s_{\star, 1}^{2 - \frac{2}{L}}$ and $L s_{\star, 2}^{2 - \frac{2}{L}}$, whereas the top two eigenvalues of the DLN are  $L s_{\star, 1}^{2 - \frac{2}{L}}$ and $\sum_{\ell=0}^{L-1} \left(s_{\star, 1}^{1-\frac{1}{L} - \frac{1}{L}\ell} \cdot s_{\star, 2}^{\frac{1}{L}\ell}\right)^2$. Hence, while the dynamics for diagonal linear networks and DLNs both occur in $r$-dimensional subspaces based on our initialization, the two loss landscapes differ significantly (see Figure~\ref{fig:diff_dln_diag}). This implicit bias is absent for gradient flow or GD in the stable regime. 


% In the DLN, some eigenvalues are a function of a ``mixture'' of singular values, which arise from the off-diagonal elements in the decoupled loss in Equation~(\ref{eqn:simplified_loss}). In the diagonal linear network, they depend only on a single coordinate (i.e., $s_{\star,i}$) or the initialization scale $\alpha$. Hence, in the diagonal linear network, a much larger learning rate is required to observe oscillations in two or more coordinates compared to the DLN. 


